Unrolling SGD: Understanding Factors Influencing Machine Unlearning

Machine unlearning is the process through which a deployed machine learning model is made to forget about some of its training data points. While naively retraining the model from scratch is an option, it is almost always associated with large computational overheads for deep learning models. Thus, several approaches to approximately unlearn have been proposed along with corresponding metrics that formalize what it means for a model to forget about a data point. In this work, we first taxonomize approaches and metrics of approximate unlearning. As a result, we identify verification error, i.e., the L2 difference between the weights of an approximately unlearned and a naively retrained model, as an approximate unlearning metric that should be optimized for as it subsumes a large class of other metrics. We theoretically analyze the canonical training algorithm, stochastic gradient descent (SGD), to surface the variables which are relevant to reducing the verification error of approximate unlearning for SGD. From this analysis, we first derive an easy-to-compute proxy for verification error (termed unlearning error). The analysis also informs the design of a new training objective penalty that limits the overall change in weights during SGD and as a result facilitates approximate unlearning with lower verification error. We validate our theoretical work through an empirical evaluation on learning with CIFAR-10, CIFAR-100, and IMDB sentiment analysis.

==> Contents/4_Verification_Error.tex <==
\section{Verification Error Captures All Metrics}
\label{sec:verification}

%leave the below label with the old title so we don't have to change it everywhere
\label{sec: One Metric to Rule Them All}

%when we earlier said that {\bf Def 1} implies {\bf Def 2}, we're talking about the limit as the verification error approaches 0 (what is used for continuity). 

%As can be seen in Figure \ref{fig:unlearning_table} there are many different broad classes of metrics to define unlearning; our question is whether there might be a metric that unifies them. 

%Broadly speaking, it's 

%Nevertheless we'll proceed to show explicitly that MI doesn't correlate with verification error ( the $\ell_2$ distance metric on the weights used for the continuity implication of {\bf Def 1} to {\bf Def 2}), then show that verification error also captures the distribution of weights metric. The result of all this is the conclusion that verification error captures all the metrics on the y-axis of Figure \ref{fig:unlearning_table}, and is the metric we can focus on - the metric to rule them all.

%\varun{you should nail, in the first couple of sentences, why the l2 difference is the only thing we should care about. that's missing.}

%It is clear that {\bf Def 1} implies {\bf Def 2} under continuity (as if the $\ell_2$ difference in weights of $M'$ and $M''$ approaches 0, then so must the outputs), however does the opposite hold? It is well known that it is possible to simply permute the weights of the model, and retain the same outputs \cite{} \anvith{@Nicolas or @Varun or me, need citation}- this violates {\bf Def 1} as the weights are no longer the same in any of the metrics we've considered, so {\bf Def 2} doesn't blindly imply {\bf Def 1}. 

% \varun{@vc: needs a bit more to motivate why we consider verification error}
% \anvith{changed}
%\anvith{I think this 3 point setup misses the point imo it should be reshuffled so that (b) is first (which we say we show in the first paragraph), then state (a) and follow up with (c) (and say we explain (c) more mathematically in the second paragraph}

%\anvith{This should also start with the motivation for the problem that there are many different metrics, each carrying their own intuition, but ideally we'd simply have one that implies all (or almost all). Our first claim is that MI (one of the most popular metrics) isn't this metric (which we empirically shows in the first paragraph), and that verification error does capture all these metrics for the reason that by continuity it implies Def2, and that in the secon paragraph we show that verification error also puts bounds on how different the distribution in weights can be (capturing the general distribution of weights category of metrics)}

%\anvith{I've written what I would }

%\anvith{for me or someone: this is bland I think}
%\varun{re-write} \anvith{alright so it was rewritten yesterday, is it better?}

%From the taxonomy laid out in \S~\ref{sec:overview_unlearning} we observe that there are many different metrics for unlearning, each carrying their own aspect of what unlearning is. In response to this, and which will be the ultimate outcome of this section, we propose the verification error as a metric that unifies all the metrics shown on the y-axis of Figure~\ref{fig:unlearning_table}.

%In the following, we show that verification error (\ie comparing an approximately unlearned model with a naively retrained model) serves as a comprehensive ground truth metric because it can be used to derive all other metrics. % Ideally there would just be one metric which implies all these other metrics. In the first paragraph below 
%Capturing all the other metrics is not the case for all metrics.  For instance, we first show that despite being one of the most popular metrics \cite{}\anvith{@Gabe can you fill the citation using it from Figure 1 here?}\nicolas{cite papers using it} privacy leakage in the outputs (\ie MI) does not capture what is measured by metrics for {\bf Def 1}. %, such as verification error.

One of the main takeaways from the taxonomy laid out in \S~\ref{sec:overview_unlearning} is that there are many different metrics for measuring unlearning. Understanding the relationship between these metrics is paramount to concretely understanding the unlearning guarantees they provide. To this end, we focus on unifying the various metrics proposed earlier. 

% What we'll first show is that the general weights category (and in particular the verification error metric) implies the general outputs category (by a pointwise convergence) but this is implication is not necessarily true in the opposite direction. Then, focusing on just the weights category, we show that the average verification error gives a uniform bound on the difference in distribution of weights between naively retraining and an approximate unlearning method of a particular form. 

% The outcome of this section will be that verification error implies, whether by a bound or in the limit, all the metrics we've discussed.

\subsection{Weight Metrics encompass Output Metrics}
\label{ssec:weights-supersede-outputs}

% \varun{2 norm is written incorrectly; content below needs a header?}
% \paragraph{Continuity:} 
It is intuitive that having similar weights would mean having similar outputs, as clearly if the weights of two models are identical then so are their outputs. We can formalize this by looking specifically at the verification error defined as $v = ||\weights'' - \weights'||_2$ where $\weights''$ are the weights of $M''$ (the unlearned model) and $\weights'$ are the weights of $M'$ (the model unlearned by retraining). With $v$ defined as above, we have for any $\mathbf{x} \in D$ that $\lim_{v \to 0} ||M'(\mathbf{x}) - M''(\mathbf{x})||_{2} = 0$ under continuity of the outputs of the models as functions of the weights. Here by continuity we mean that  fixing the input $\mathbf{x}$ to a model we then have that $M(\mathbf{x})$ is a continuous function of the weights. Thus, $\lim_{v \to 0}$ entails point-wise convergence of the outputs of $M''$ to the outputs of $M'$. Furthermore, note that smooth functions are locally lipschitz. Because DNNs are smooth functions, this relation in the limit sense is thus equivalent to a linear convergence on an upper bound on the $\ell_2$ difference between the two models' outputs. This means changes to the differences in weights lead to proportional changes to an upper bound on the $\ell_2$ difference in the models' outputs for a datapoint. Thus, we observe that the weight space category of metrics ({\bf Def 1}), and specifically the verification error, imply the output space category of metrics ({\bf Def 2}). 

However the opposite does not hold. To see why, consider the following counterexample. If one permutes the weights of a neural network, the model's outputs remain identical~\cite{permutation}. Yet, the verification error would not be $0$ after such a permutation, and so having all the outputs be the same does not entail having the same weights. 

We further illustrate 
how output space metrics are unable to capture weight space metrics by considering a  MI-based metric from \S~\ref{sec:overview_unlearning} for the output space metric and verification error for the weight space metric. We  empirically show how the privacy risk score (PRS)~\cite{song2021systematic} does not imply verification error (in the sense a decrease in PRS does not imply a decrease in verification error). 
% To understand the relation between metrics based on MI and verification error, we thus 
Specifically, we test the correlation between PRS and verification error after applying an approximate  method to unlearn a datapoint $\mathbf{x}^*$. Here, we choose  amnesiac machine learning~\cite{graves2020amnesiac} because it was introduced as an approximate approach to unlearning with a MI-based criterion.\footnote{We reproduced the approach because it was originally evaluated on a MI attack by Yeom \etal~\cite{yeom2018privacy}.}
To this end, we train the original model $M$, the naively retrained model $M'$, and  model $M''$ unlearned using amnesiac unlearning on the CIFAR-10~\cite{krizhevsky2009learning} and CIFAR-100 datasets~\cite{krizhevsky2009learning}, using the ResNet-18 and VGG-19 architectures~\cite{resnet, simonyan2014very}. We obtain 27 triplets of $M$,$M''$,$M'$ by changing the training settings (\ie different amounts of training, batch sizes, learning rates etc.). For each triplet, we measured the PRS of the unlearned point $\mathbf{x}^*$ on $M''$, and the verification error $||\weights'' - \weights'||_{2}$ (obtained from $M''$ and $M'$ respectively). The results are presented in Figure~\ref{fig:amnesiac_prs_vs_ver}. Observe that there is little to {\em no correlation} between PRS (an output space metric) and the verification error (a weight space metric). This illustrates how MI, and in general output space metrics, do not capture weight space definitions ({\bf Def 1}). 


\begin{figure}
    \centering
    \includegraphics[width = 3.2in]{plots/fig2.png}
 \caption{Correlation between privacy risk score and verification error in different training setups for CIFAR-10 and CIFAR-100. The correlations are -0.29 and -0.02, respectively.}
 \label{fig:amnesiac_prs_vs_ver}
\end{figure}


%What this means is that the limit as verification error goes to 0 implies that all the outputs of $M''$ and $M'$ are the same and so we see that verification error implies the general {\bf Def 2} category of metrics (under point-wise convergence).

%\anvith{@here changing subsection title to "$L^p$ distribution metrics" from "all other weight metrics"; note we use capital L for Lebesgue (lower case l is for euclidean)} 
%\varun{1. can't we use the name Lebesgue?; 2. can we have shorter titles that don't spill over to another line?; 3. you've to define with $L^p$ is} \anvith{1. sorry I mispoke earlier, $L^p$ is the definition (not we're doing this, this is a standard math definition); 2. dropped "distribution"; 3. Can I just cite a textbook the first time I mention it? I guess this is slightly complicated cuz the none of the analysis textbooks I learned from have google scholar citations so...}


\subsection{Verification Error implies $L^p$ Weight Metrics}
\label{sec: ver_err_implies_weights}

% \anvith{dunno what this paragraph below is saying; commented out old one gave new one}

We will prove that verification error provides a bound on the supremum norm of the difference of the distribution of weights obtained by (1) naively retraining, and by (2) using an approximate unlearning method (which depends on the initial weights and batch ordering). Note that a bound on the supremum norm implies bounds on all $L^p$ norms on bounded domains in the weight space. Informally, this allows us to motivate that verification error is an unlearning metric which not only supersedes all output space metrics, but also bounds most weight space metrics. Later in the paper, we will thus consider verification error as the primary metric of interest for unlearning.

Recall the $L^p$ norm of a (lebesgue) measurable function $f$ over a space X is $(\int_{X} |f|^p d\mu)^{\frac{1}{p}}$ where $d\mu$ is the lebesgue measure~\cite{browder2012mathematical}. Furthermore, note that by the dominated convergence theorem~\cite{browder2012mathematical} that all probability density functions can be approximated by a function which has bounded support for arbitrary $L^1$ error (see Appendix~\ref{sec: Appendix A: Proofs}). Hence the claim that the bound on the supremum norm implies bounds on {\em all $L^p$ metrics}. 

%\todo{nicolas replaced noisiness with stochasticity but if this is not exact reverse}\anvith{I think stochasticity is good}
Similarly, a bound on the supremum norm also implies guarantees similar to differential privacy (DP) (in particular $\varepsilon=0$ and $\delta = b$ where $b$ is the bound on the supremum norm) by the reverse triangle inequality. The opposite, though, is not true when $\varepsilon \neq 0$ (as the bound now depends on the magnitude of the function and thus is not uniform). 
However, it should be noted that in our subsequent analysis, we make several assumptions about the stochasticity of training which does not allow us to derive strict DP-like guarantees. In particular we will assume: (1) noise is simply added to the final weights (to approximate step-wise noisiness), and (2) that this noise changes negligibly when removing a data point from the dataset. We explain why we made these assumptions later in the section during our derivation.

%\todo{how do we justify these assumptions are reasonable}\anvith{@varun we explain these assumptions more during the section, so I added a statement saying that}


%\anvith{@Nicolas expanded a bit more on this without writing equation, hopefully is a bit better}

%A uniform bound implies guarantees similar to differential privacy (DP) (in particular $\varepsilon=0$ and $\delta$ equals the uniform bound) by the reverse triangle inequality, though the opposite is not true when $\varepsilon \neq 0$ (as the bound now depends on the magnitude of the function and thus isn't uniform).\footnote{It should be noted that in our subsequent analysis we make several assumptions about noise during training which does not allow us derive strict DP gurantees; future work may possibly improve these assumptions. In particular we assume noise is simply added to the final weights, and that this noise changes negligibly when removing a data point from the dataset.}

%We will prove a difference in the distribution of weights by naive retraining and by an approximate unlearning method that is solely a function on the initial weights and batch ordering, and this is uniformly bounded by the verification error. It is easy to see how a uniform bound. A uniform bound is a generally strong condition \varun{for what?}, and it is easy to see how it implies guarantees similar to DP.

In particular, the focus here will be first comparing the probability distributions of final weights obtained by training $m$ epochs starting at a fixed initial weight $\weights_0$ with dataset $D$ and dataset $D'= D \setminus \mathbf{x}^*$ with SGD (and not mini-batch SGD, \ie considering mini-batch sizes of 1). We will represent the density functions respectively as $\mathbb{P}(\weights)$ and $\mathbb{P'}(\weights)$ where both are functions of the weights of the model $\weights$, and note in what follows $\mathbf{x}^*$ is fixed but can be any data point (\ie is a constant).

Let the size of $D$ be $|D|=n$, and let $I = \{\mathbf{x}_{i_1},\mathbf{x}_{i_2},\cdots,\mathbf{x}_{i_{mn}}\}$ denote a particular ordering of the datapoints when training on $D$ for $m$ epochs (where $i_j \in [n])$. Note that we have $(n!)^m$ such combinations; for $D'$, we have $(n-1)!^m$ such combinations. For each $I$, there exists an $I'$ (corresponding to $D' = D \setminus \mathbf{x}^*)$, which is formed by removing all instances of $\mathbf{x}^*$ (in-place) from $I$. Note that for a given $I'$, we have $n^m$ corresponding choices of $I$ (as for each epoch we have $n$ choices to place $\mathbf{x}^*$ per epoch, and $m$ epochs in total). Let $\weights_I$ represent the deterministic final weights resulting from training with the data ordering $I$, starting from $\weights_0$. Let $\mathbf{g}$ denote the random variable which represents the noise on the final weights (\ie we assume the noise per step accumulates so we can simply add some random variable onto the final weights) when training for $m \cdot n$ steps. Thus, the random variable representing the final weights when training with $I$ is $\mathbf{z}_{I} = \weights_I + \mathbf{g}$. Similarly, we define $\mathbf{z}_{I'} = \weights_{I'} + \mathbf{g}'$ where $\mathbf{g}'$ represents the noise when training $(n-1) \cdot m$ steps. Note that, if training is deterministic, we have $\weights_{I'} = \weights_{I} - \mathbf{d}_I$ where $\mathbf{d}_I$ is some constant that only depends on $\weights_0$ and the ordering $I$ (as under deterministic operations $\weights_{I'}$ and $\weights_{I}$ are constants depending only on $\weights_0$ and the ordering $I$ and thus $\weights_{I} - \weights_{I'} = \mathbf{d}_I$ is a constant that only depends on them). Lastly, we make an assumption that the noise from training with $m \cdot n$ steps is equivalent to that training from $(n-1) \cdot m$ steps, \ie that $\mathbf{g}$ = $\mathbf{g}'$. This is based on the fact that this noise should only be a function of the number of training steps, and that noise per step is small (see \cite[\S~6]{jia2021proof} for a discussion on noise during training)\footnote{Thus, adding or removing $m$ steps (1 per epoch) when compared to the $m \cdot n$ total steps when training with ordering $I$ is insignificant}. Thus we have $\mathbf{z}_{I'} = \mathbf{z}_{I} - \mathbf{d}_{I}$.


% \anvith{@Nicolas added remark on d not being a random variable} \varun{why?}\anvith{in the notes he sent a while back when we were thinking of pushin to arxiv he mentioned explaining it more}
% (where recall $\mathbf{d}_{I}$ isn't a random variable by the above definition).

%\anvith{@Nicolas changed typo from minibatches to datapoints} 

%\varun{do we wanna change the lipschitz constant from L to something else, given the lebesgue stuff earlier?} \anvith{I think it should be fine as we say Lipschits constant L and $L^p$ has an addition $^p$); L doesn't really mean anything on its own in the previous context for lebesque measure}
Given that SGD samples individual datapoints uniformly, the probability of obtaining a given data ordering is constant. Further, if $\mathbb{P}_I(\weights)$ is the density function corresponding to $\mathbf{z}_{I}$ and $\mathbb{P'}_{I'}(\weights)$ is the density function corresponding to $\mathbf{z}_{I'}$ (which is equal to $\mathbb{P}_{I}(\mathbf{w}-\mathbf{d}_{I})$), then $\mathbb{P}(\weights) = \frac{1}{n!^m}\sum_{I}\mathbb{P}_{I}$ and $\mathbb{P'}(\weights) = \frac{1}{(n-1)!^m}\sum_{I'}\mathbb{P'}_{I'}(\weights)$.

\begin{lemma}
If every $\mathbb{P}_I$ is Lipschitz with Lipschitz constant $L$ (which is true if $\mathbf{g}$ is gaussian), and if we let $d = \frac{1}{n!^m}\sum_{I} ||\mathbf{d}_I||_{2}$, then:

\begin{equation}
\label{eq: l2_prob_difference_1}
||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2} \leq L \cdot d
\end{equation}

\label{lem:dif_train_retrain}
\end{lemma}
We refer the reader to Appendix~\ref{sec: Appendix A: Proofs} for the detailed derivation. This result shows that by accounting for all the individual distributions (for each ordering $I$), we were able to obtain a Lipschitz condition on the combined distribution (of final weights obtained by training $m$ epochs starting at a fixed intial weight $\weights_0$).  The Lipschitz condition is expressed with respect to the datasets including or excluding the point to be unlearned.%\todo{check interpretation is correct}\anvith{is good}

Now, we are also interested in the difference between the density function obtained after the application of an approximate unlearning method on $M$ (\ie $\mathbb{P''}(\weights)$), and $\mathbb{P'}(\weights)$. If the approximate unlearning method only considers $\weights_0$, $I$ to define an unlearning update $\mathbf{u}_I$, and obtains the approximately unlearned weights by adding $\mathbf{u}_I$ to $\mathbf{w}_I$, \ie $\weights_{I}'' = \weights_I + \mathbf{u}_I$, then:

%To understand how this relates to verification error and approximate unlearning, let's consider an approximate unlearning method which only looks at $\weights_0$ and $I$ and to $\weights_I$ obtains the approximately unlearned weights $\weights_{I}'' = \weights_I + u_I$ where $u_I$ is some unlearning update. Note then we can analogously define a $\mathbf{z}_{I}''= \weights_{I} + \mathbf{u}_I + \mathbf{g}$ as before with corresponding density function $\mathbb{P}''_{I}(w)$. Defining $\mathbf{v}_I = \mathbf{u}_I + \mathbf{d}_I$ we get $\mathbf{z}_{I'} = \mathbf{z}_{I}'' - \mathbf{v}_I$ where $\mathbf{v}_I$ represents the analytic (ignoring noise) verification error for the given ordering $I$ (\ie the difference between the weights obtained from the approximate unlearning $\weights_{I}''$ and the retrained weights $\weights_{I'}$). At this point it's clear all the previous steps follow and defining $v$ as the average of all the $||\mathbf{v}_I||_2$ we get

\begin{corollary}
If every $\mathbb{P}_I$ is Lipschitz with constant $L$ (true if $\mathbf{g}$ is gaussian), and if we let $v = \frac{1}{n!^m}\sum_{I} ||\mathbf{d}_I + \mathbf{u}_I||_{2}$, then:
\begin{equation}
\label{eq: l2_dif_bounded_ver_err}
||\mathbb{P''}(\weights) - \mathbb{P'}(\weights)||_{2} \leq L \cdot v
\end{equation}
\label{cor:ver_err_bound_probs}
\end{corollary}
The detailed proof is in Appendix~\ref{sec: Appendix A: Proofs}. This naturally follows from the same accounting procedure used for the previous lemma, but now $\mathbf{d}_I$ have been swapped for $\mathbf{d}_I + \mathbf{u}_I$. This gives us a bound on the supremum norm by the average verification error $v$ (times some constant) on the difference of the probability distributions after approximate unlearning $\mathbb{P''}(\weights)$ and ideal retraining $\mathbb{P'}(\weights)$. Note, however, that there is a necessary assumption on the form of this approximate unlearning method: to obtain Equation~\ref{eq: l2_dif_bounded_ver_err}, we require the unlearning update to only be dependant on the initial weight $\weights_0$ and $I$. We will introduce such an unlearning approach in \S~\ref{sec:A Closed Form Approximation of SGD}. Finally, an analogous bound  going in the opposite direction is provided in Appendix~\ref{sec: Appendix A: Proofs}.


%\varun{you wanna end with a small blurb that reiterates why VE is ground truth metric}\anvith{added below}

%\paragraph{Final Remark on Verification Error} So what we've shown in \S~\ref{} is that verification error in the limit to 0 implies pointwise convergence of the outputs of the approximately unlearned model $M''$ to $M$, and in \S~\ref{} that using a particular form of approximate unlearning we have verification error leads to uniform bounds on the difference of of weight distributions of $M''$ and $M'$. What we conclude then is that verification error captures all the categories of metrics presented on the y-axis of Figure~\ref{fig:unlearning_table}, and acts as a ground truth metric.
\vspace{1mm}
\noindent{\bf Summary:} In \S~\ref{ssec:weights-supersede-outputs}, we demonstrated how verification error captures the changes in outputs, and thus encompasses metrics that measure unlearning using {\bf Def 2}. We then proceeded to demonstrate how, using a particular form of approximate unlearning (and assumptions about noise), verification error also leads to uniform bounds in the difference in weight distributions of $M'$ (the retrained model) and $M''$ (the approximately unlearned model). Thus, verification error also encompasses a large class of metrics that measure unlearning using {\bf Def 1}. %\anvith{commented out the next line}

%Thus, verification error is able to encompass all metrics defined earlier. 

%\subsection{Strawman: Privacy Leakage}

%The privacy risk score (PRS) of Song \etal~\cite{song2021systematic} is an example of an MI-based metric to measure unlearning (see taxonomy from \S~\ref{sec:overview_unlearning}). To understand the relation between metrics based on MI and verification error, we thus test the correlation between PRS and verification error after applying an approximate unlearning method to unlearn a datapoint $\mathbf{x}^*$. Here, we choose  amnesiac machine learning~\cite{graves2020amnesiac}.\footnote{We reproduced the approach because it was originally evaluated on an MI attack by Yeom \etal~\cite{yeom2018privacy}.}

%To this end, we train the original model $M$, the naively retrained model $M'$, and unlearned model $M''$ (using amnesiac unlearning~\cite{graves2020amnesiac}) on the CIFAR-10~\cite{krizhevsky2009learning} and CIFAR-100 datasets~\cite{krizhevsky2009learning}, using the ResNet18 and VGG19 architectures~\cite{resnet, simonyan2014very}. We obtain numerous triplets $M$,$M''$,$M'$ by changing the training settings (\ie different amounts of training, batch sizes, learning rates etc). For each triplet we measured the PRS of the unlearned point $\mathbf{x}^*$ on $M''$, and the verification error $||M'' - M'||_{2}$. The results are presented in Figure~\ref{fig:amnesiac_prs_vs_ver}. Observe that there is little to {\em no correlation} between PRS and the verification error; this is suggestive that MI as a metric does not always capture {\bf Def 1}. 


%\begin{figure}
    %\centering
    %\includegraphics[width = 3.2in]{plots/fig2.png}
 %\caption{Correlation between privacy risk score and verification error in different training setups for CIFAR-10 and CIFAR-100. The correlations are -0.29 and -0.02, respectively.}
 %\label{fig:amnesiac_prs_vs_ver}
%\end{figure}


%\vspace{1mm}\noindent{\bf Verification Error to Unify Them All:} From our discussion of MI, we see that the most popular metric for {\bf Def 2} does not generally imply {\bf Def 1}, though the opposite is true. 

%To make explicit why verification error can unify the various metrics considered for {\bf Def 1} of approximate unlearning, we prove that a bound on (average) verification error leads to a uniform bound on the difference of probability density functions of the final weights for a specific approximate unlearning approach and retraining (under some assumptions). A uniform bound, and more importantly a uniform convergence to 0 on that bound, is a strong condition; it is easy to see how this can give DP-like guarantees, and guarantees of a similar form to that considered by Guo et al \cite{guo2019certified}. 


% \subsection{Uniform Bounds and Verification Error}
%\label{sec:Probability Difference bounded by Verification Error}

%\anvith{Do we not want the other bound going in the opposite direction showing equivalence? Perhaps just for the appendix?}


%\subsection{Verification error unifies all metrics}
%\label{sec:Verification Error unifies all metrics}


%\nicolas{the paragraph below needs to be rephrased to clearly state at a high level how we prove that verification error captures all existing metrics}\anvith{added}

%Instead, verification error, as we will proceed to show, captures all the categories of metrics depicted on the y-axis of Figure \ref{fig:unlearning_table}. That is we will show:

%\begin{enumerate}
    %\item difference in distributions of weights of $M''$ and $M'$ is uniformly bounded by the average verification error
    %\item remark how the limit as verification error goes to 0 implies the difference in outputs for any datapoint goes to 0, implying the general output space category of metrics stemming from {\bf Def 2}
%\end{enumerate}




%We first show that the difference in distributions of weights of $M''$ and $M'$ is uniformly bounded by the average verification error, and so decreasing it decreases this bound (and so verification error captures the "distribution of weights" metric). We then remark by continuity that as verification error goes to zero (\ie the $\ell_2$ difference in weights of $M'$ and $M''$) the difference in the distribution of outputs of $M'$ and $M''$ must go to zero also, and thus verification error captures the remaining {\bf Def 2} (\ie output space) class of metrics and so covers all the general metrics.





%Old Version

%Verification error can replace other metrics to measure the efficacy of unlearning for the following reasons: (a) as verification error approaches 0, then so does the the difference in outputs between $M'$ and $M''$ by continuity (\ie {\bf Def 1} implies {\bf Def 2}); (b) popularly used metrics like MI are ineffective in practice; and (c) if the average verification error is $0$ then the distribution of final weights of $M'$ and $M''$ are practically identical, and thus we see verification error also captures metrics broadly used to measure the {\em distribution of weights} in Table~\ref{}. Thus, we observe that verification error captures all the general metrics stated on the y-axis of Figure~\ref{fig:unlearning_table}.

%\paragraph{Distribution Difference Uniformly bounded by Verification Error.} The focus here will be first comparing the probability distributions of final weights obtained by training $m$ epochs starting at a fixed initial weight $\weights_0$ with dataset $D$ and dataset $D'= D \setminus \mathbf{x}^*$ with SGD (and not mini-batch SGD, \ie considering batch sizes of 1). We will represent the density functions respectively as $\mathbb{P}(\weights)$ and $\mathbb{P'}(\weights)$. 


% \vspace{1mm}
% \nj{maybe have a table of notation as what we did in PoL}\anvith{think it might be hard as we're doing some math-albeit rather simple math- at the same time as introducing the notation}
%\noindent{\em Notation:} Let the size of $D$ be $|D|=n$, and let $I = \{\mathbf{x}_{i_1},\mathbf{x}_{i_2},\cdots,\mathbf{x}_{i_{mn}}\}$ denote a particular ordering of the datapoints when training on $D$ for $m$ epochs (where $i_j \in [n])$. Note that we have $(n!)^m$ such combinations; for $D'$, we have $(n-1)!^m$ such combinations. For each $I$, there exists an $I'$ (corresponding to $D' = D \setminus \mathbf{x}^*)$, which is formed by removing all instances of $\mathbf{x}^*$ (in-place) from $I$. Note that for a given $I'$, which is an ordering of batches when trained on $D'$, we have $n^m$ corresponding choice of $I$ (as for each epoch we have $n$ choices to place $\mathbf{x}^*$ per epoch, and $m$ epochs in total). Let $\weights_I$ represent the deterministic final weights resulting from training with the data ordering $I$, starting from $\weights_0$. Let $\mathbf{g}$ denote the random variable which represents the noise when training for $m \cdot n$ steps. Thus, the random variable representing the final weights when training with $I$ is $\mathbf{z}_{I} = \weights_I + \mathbf{g}$. Similarly, we define $\mathbf{z}_{I'} = \weights_{I'} + \mathbf{g}'$ where $\mathbf{g}'$ represents the noise when training $(n-1) \cdot m$ steps. Note that, if training is deterministic, we have $\weights_{I'} = \weights_{I} - \mathbf{d}_I$ where $\mathbf{d}_I$ is some constant that only depends on $\weights_0$ and the ordering $I$. Lastly, we make an assumption that the noise from training with $m \cdot n$ steps is equivalent to that training from $(n-1) \cdot m$ steps, \ie that $\mathbf{g}$ = $\mathbf{g}'$. This is based on the fact that this noise should only be a function of the number of training steps, and that noise per step is negligible\footnote{Thus, adding or removing $m$ steps (1 per epoch) when compared to the $m \cdot n$ total steps when training with ordering $I$ is insignificant}. Thus we have $\mathbf{z}_{I'} = \mathbf{z}_{I} - \mathbf{d}_{I}$.

%Note that, assuming the probability of a given batch ordering is constant (\ie a uniform distribution of batch orderings), and if $\mathbb{P}_I(\weights)$ is the density function corresponding to $\mathbf{z}_{I}$ and $\mathbb{P'}_{I'}(\weights)$ is the density function corresponding to $\mathbf{z}_{I'}$ (which is equal to $\mathbb{P}_{I}(\mathbf{w}-\mathbf{d}_{I})$), then $\mathbb{P}(\weights) = \frac{1}{n!^m}\sum_{I}\mathbb{P}_{I}$ and $\mathbb{P'}(\weights) = \frac{1}{(n-1)!^m}\sum_{I'}\mathbb{P'}_{I'}(\weights)$.

%\begin{lemma}
%If every $\mathbb{P}_I$ is Lipschitz with Lipschitz constant $L$ (true if $\mathbf{g}$ is gaussian), and if we let $d = \frac{1}{n!^m}\sum_{I} ||\mathbf{d}_I||_{2}$, then:

%\begin{equation}
%\label{eq: l2_prob_difference_1}
%||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2} \leq L \cdot d
%\end{equation}

%\label{lem:dif_train_retrain}
%\end{lemma}

%We refer the reader to Appendix~\ref{sec: Appendix A: Proofs} for the detailed derivation. We are also interested in the difference between the density function obtained after the application of an approximate unlearning method on $M$ (\ie $\mathbb{P''}(\weights)$), and $\mathbb{P'}(\weights)$. If the approximate unlearning method only considers $\weights_0$, $I$ to define an unlearning update $u_I$, and obtains the approximately unlearned weights by adding $u_I$ to $w_I$, \ie $\weights_{I}'' = \weights_I + \mathbf{u}_I$, then:

%To understand how this relates to verification error and approximate unlearning, let's consider an approximate unlearning method which only looks at $\weights_0$ and $I$ and to $\weights_I$ obtains the approximately unlearned weights $\weights_{I}'' = \weights_I + u_I$ where $u_I$ is some unlearning update. Note then we can analogously define a $\mathbf{z}_{I}''= \weights_{I} + \mathbf{u}_I + \mathbf{g}$ as before with corresponding density function $\mathbb{P}''_{I}(w)$. Defining $\mathbf{v}_I = \mathbf{u}_I + \mathbf{d}_I$ we get $\mathbf{z}_{I'} = \mathbf{z}_{I}'' - \mathbf{v}_I$ where $\mathbf{v}_I$ represents the analytic (ignoring noise) verification error for the given ordering $I$ (\ie the difference between the weights obtained from the approximate unlearning $\weights_{I}''$ and the retrained weights $\weights_{I'}$). At this point it's clear all the previous steps follow and defining $v$ as the average of all the $||\mathbf{v}_I||_2$ we get

%\begin{corollary}
%If every $\mathbb{P}_I$ is Lipschitz with constant Lipschitz $L$ (true if %$\mathbf{g}$ is gaussian), and if we let $v = \frac{1}{n!^m}\sum_{I} ||\mathbf{d}_I + \mathbf{u}_I||_{2}$, then:
%\begin{equation}
%\label{eq: l2_dif_bounded_ver_err}
%||\mathbb{P''}(\weights) - \mathbb{P'}(\weights)||_{2} \leq L \cdot v
%\end{equation}
%\label{cor:ver_err_bound_probs}
%\end{corollary}

%The detailed proof is in Appendix~\ref{sec: Appendix A: Proofs}. This gives us a uniform bound on the difference of the probability distribution after approximate unlearning and the ideal retraining, but note the necessary assumption on the form of this approximate unlearning method; to obtain Equation~\ref{eq: l2_dif_bounded_ver_err}, we require the unlearning update to only be dependant on the initial weight $\weights_0$ and $I$. An analogous bound, but going in the opposite direction is provided in Appendix~\ref{sec: Appendix A: Proofs}.

%Nevertheless, the main takeaway for now is that verification error does give us a uniform bound on the difference in probability distributions between the approximate unlearning method and ideal retraining.

%The focus here will be first comparing the probability distributions of final weights obtained by training $m$ epochs starting at a fixed initial weight $\weights_0$ with dataset $D$ and dataset $D'= D \setminus \mathbf{x}^*$ with SGD (and not mini-batch SGD, \ie considering batch sizes of 1). We will represent the density functions respectively as $\mathbb{P}(\weights)$ and $\mathbb{P'}(\weights)$. 


% \vspace{1mm}
% \nj{maybe have a table of notation as what we did in PoL}\anvith{think it might be hard as we're doing some math-albeit rather simple math- at the same time as introducing the notation}
%\noindent{\em Notation:} Let the size of $D$ be $|D|=n$, and let $I = \{\mathbf{x}_{i_1},\mathbf{x}_{i_2},\cdots,\mathbf{x}_{i_{mn}}\}$ denote a particular ordering of the datapoints when training on $D$ for $m$ epochs (where $i_j \in [n])$. Note that we have $(n!)^m$ such combinations; for $D'$, we have $(n-1)!^m$ such combinations. For each $I$, there exists an $I'$ (corresponding to $D' = D \setminus \mathbf{x}^*)$, which is formed by removing all instances of $\mathbf{x}^*$ (in-place) from $I$. Note that for a given $I'$, which is an ordering of batches when trained on $D'$, we have $n^m$ corresponding choice of $I$ (as for each epoch we have $n$ choices to place $\mathbf{x}^*$ per epoch, and $m$ epochs in total). Let $\weights_I$ represent the deterministic final weights resulting from training with the data ordering $I$, starting from $\weights_0$. Let $\mathbf{g}$ denote the random variable which represents the noise when training for $m \cdot n$ steps. Thus, the random variable representing the final weights when training with $I$ is $\mathbf{z}_{I} = \weights_I + \mathbf{g}$. Similarly, we define $\mathbf{z}_{I'} = \weights_{I'} + \mathbf{g}'$ where $\mathbf{g}'$ represents the noise when training $(n-1) \cdot m$ steps. Note that, if training is deterministic, we have $\weights_{I'} = \weights_{I} - \mathbf{d}_I$ where $\mathbf{d}_I$ is some constant that only depends on $\weights_0$ and the ordering $I$. Lastly, we make an assumption that the noise from training with $m \cdot n$ steps is equivalent to that training from $(n-1) \cdot m$ steps, \ie that $\mathbf{g}$ = $\mathbf{g}'$. This is based on the fact that this noise should only be a function of the number of training steps, and that noise per step is negligible\footnote{Thus, adding or removing $m$ steps (1 per epoch) when compared to the $m \cdot n$ total steps when training with ordering $I$ is insignificant}. Thus we have $\mathbf{z}_{I'} = \mathbf{z}_{I} - \mathbf{d}_{I}$.

%Note that, assuming the probability of a given batch ordering is constant (\ie a uniform distribution of batch orderings), and if $\mathbb{P}_I(\weights)$ is the density function corresponding to $\mathbf{z}_{I}$ and $\mathbb{P'}_{I'}(\weights)$ is the density function corresponding to $\mathbf{z}_{I'}$ (which is equal to $\mathbb{P}_{I}(\mathbf{w}-\mathbf{d}_{I})$), then $\mathbb{P}(\weights) = \frac{1}{n!^m}\sum_{I}\mathbb{P}_{I}$ and $\mathbb{P'}(\weights) = \frac{1}{(n-1)!^m}\sum_{I'}\mathbb{P'}_{I'}(\weights)$.

%\begin{lemma}
%If every $\mathbb{P}_I$ is Lipschitz with Lipschitz constant $L$ (true if $\mathbf{g}$ is gaussian), and if we let $d = \frac{1}{n!^m}\sum_{I} ||\mathbf{d}_I||_{2}$, then:

%\begin{equation}
%\label{eq: l2_prob_difference_1}
%||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2} \leq L \cdot d
%\end{equation}

%\label{lem:dif_train_retrain}
%\end{lemma}

%We refer the reader to Appendix~\ref{sec: Appendix A: Proofs} for the detailed derivation. We are also interested in the difference between the density function obtained after the application of an approximate unlearning method on $M$ (\ie $\mathbb{P''}(\weights)$), and $\mathbb{P'}(\weights)$. If the approximate unlearning method only considers $\weights_0$, $I$ to define an unlearning update $u_I$, and obtains the approximately unlearned weights by adding $u_I$ to $w_I$, \ie $\weights_{I}'' = \weights_I + \mathbf{u}_I$, then:

%To understand how this relates to verification error and approximate unlearning, let's consider an approximate unlearning method which only looks at $\weights_0$ and $I$ and to $\weights_I$ obtains the approximately unlearned weights $\weights_{I}'' = \weights_I + u_I$ where $u_I$ is some unlearning update. Note then we can analogously define a $\mathbf{z}_{I}''= \weights_{I} + \mathbf{u}_I + \mathbf{g}$ as before with corresponding density function $\mathbb{P}''_{I}(w)$. Defining $\mathbf{v}_I = \mathbf{u}_I + \mathbf{d}_I$ we get $\mathbf{z}_{I'} = \mathbf{z}_{I}'' - \mathbf{v}_I$ where $\mathbf{v}_I$ represents the analytic (ignoring noise) verification error for the given ordering $I$ (\ie the difference between the weights obtained from the approximate unlearning $\weights_{I}''$ and the retrained weights $\weights_{I'}$). At this point it's clear all the previous steps follow and defining $v$ as the average of all the $||\mathbf{v}_I||_2$ we get

%\begin{corollary}
%If every $\mathbb{P}_I$ is Lipschitz with constant Lipschitz $L$ (true if $\mathbf{g}$ is gaussian), and if we let $v = \frac{1}{n!^m}\sum_{I} ||\mathbf{d}_I + \mathbf{u}_I||_{2}$, then:
%\begin{equation}
%\label{eq: l2_dif_bounded_ver_err}
%||\mathbb{P''}(\weights) - \mathbb{P'}(\weights)||_{2} \leq L \cdot v
%\end{equation}
%\label{cor:ver_err_bound_probs}
%\end{corollary}

%The detailed proof is in Appendix~\ref{sec: Appendix A: Proofs}. This gives us a uniform bound on the difference of the probability distribution after approximate unlearning and the ideal retraining, but note the necessary assumption on the form of this approximate unlearning method; to obtain Equation~\ref{eq: l2_dif_bounded_ver_err}, we require the unlearning update to only be dependant on the initial weight $\weights_0$ and $I$. An analogous bound, but going in the opposite direction is provided in Appendix~\ref{sec: Appendix A: Proofs}.


%\paragraph{Final Remark on {\bf Def 2}}
%Finally, observe that for any $\mathbf{x} \in D$, defining $v = ||\weights'' - \weights'||_2$ where $\weights''$ and $\weights'$ are the weights of $M''$ (the approximately unlearned model) and $M'$ (the naively retrained model) respectively, then $\lim_{v \to 0} ||M'(\mathbf{x} - M''(\mathbf{x})||_2 = 0$ under continuity of the outputs of the models as functions of the weights (i.e fixing the input $\mathbf{x}$ to a model, $M(\mathbf{x})$ is a continuous function of the weights).

%What this means is that the limit as verification error goes to 0 implies that all the outputs of $M''$ and $M'$ are the same and so we see that verification error implies the general {\bf Def 2} category of metrics (under point-wise convergence).

%as verification error approaches 0, then so does the difference in outputs between $M'$ and $M''$ by continuity, so verification error implies {\bf Def 2}. 

%Thus, we have that verification error captures broadly all the metrics we've considered (all the metrics on the y-axis of Figure \ref{fig:unlearning_table}).


% \iffalse
% \subsubsection{Verification Error bounded by Uniform Bound on Distribution Difference}

% \varun{still don't see why this is necessary; can you please explain?}
% \anvith{oh this is just to see how work that claim to reduce a uniform bound (say DP with epsilon 0 or something like that) also reduces avergae verification error}

% We now proceed to get a bound on the average verification error $v$ based on a uniform bound between the density function after the approximate unlearning and the density function for ideal retraining.

% Note, assuming the noise has $0$ mean, $v$ is simply the difference in expectation of $\mathbb{P''}(\weights)$ and $\mathbb{P'}(\weights)$, and let us for the time being assume that the union of the support of $\mathbb{P''}(\weights)$ and $\mathbb{P'}(\weights)$ is bounded, \ie if $\mathbf{W}$ is the union of the supports, then $\int_{\mathbf{W}} ||\weights||_{2} d\weights = a < \infty$. This is reasonable as we'd expect the noise from training to be bounded; in fact in general we'd only need the integral outside a bounded domain to be finite, but the reasoning is analogous to what follows and would simply add an extra constant term. Now if say $||\mathbb{P''}(\weights) - \mathbb{P'}(\weights)||_{2} < b$ for some scalar $b$ for all $w$ (\ie $b$ is a uniform bound), we have:

% \begin{multline}
% \label{eq:exp_ver_err}
% v = ||\mathbb{E}(\mathbb{P''}(\weights)) - \mathbb{E}(\mathbb{P'}(\weights))||_{2} \\
% = ||\int_{\mathbf{W}} \mathbb{P''}(\weights) \weights d\weights - \int_{\mathbf{W}} \mathbb{P'}(\weights) \weights d\weights||_{2} \\
% \leq \int_{\mathbf{W}} ||\mathbb{P''}(\weights) - \mathbb{P'}(\weights)||_{2} \cdot ||\weights||_{2} d\weights \\
% \leq ba
% \end{multline}

% and so in this sense we see reducing the max value of $||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2}$ gives a smaller bound on the expectation of verification error $v$.

% Thus we see the relation between verification error and $||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2}$ runs both ways (\ie reducing either gives a tighter bound on the other), and as $||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2}$ captures the difference in probability distributions when training with and without a datapoint $\mathbf{x}^*$, we generally expect that similar metrics trying to minimize the shift in the probability distributions would follow similar relations as described above.

% \subsubsection{Main Takeaway from Bounds}

% What we've shown with the two Bounds \ref{eq: l2_dif_bounded_ver_err}, \ref{eq:exp_ver_err} is that decreasing the average verification error decreases the uniform bound on the difference in probability density functions, and decreasing the uniform bound on the probability density functions decreases the bound on the average verification error; we've shown they are practically interchangeable if one is simply interested in bounds.

% This is of interest as note if $||\mathbb{P''}(\weights) - \mathbb{P'}(\weights)||_{2} < b$ then we have $\mathbb{P''}(\weights) \leq b + \mathbb{P'}(\weights)$ and $\mathbb{P'}(\weights) \leq b + \mathbb{P''}(\weights)$, giving bounds reminiscent of DP and that used by Guo et al \cite{guo2019certified}; so we see by working with the uniform bound we retrieve bounds of the form used by the other work we mentioned trying to measure {\bf Def 1}. The link to KL divergence is less obvious to us (though it should be there as generally a uniform bound is a strong condition) so we leave it for future work to resolve, or possibly past work we are not aware of.

% \fi





==> Contents/5_Verifying_Unlearning_Good.tex <==
\section{Are we doing what we want to?}

%\anvith{for me: brief blurb on reasoning to just check that we're actually achieving what we want to (reducing true discrepency), i.e our approximation is justified, but it is an approximation, and it is worth checking we are indeed accomplishing what we want to}

At this point, with our SD Loss, we see we can significantly reduce $e$, and similarly we see pretraining is also a viable option. However it is reasonable to wonder whether in fact decreasing $e$ as we've done with the two methods does in fact decrease the true discrepancy, i.e whether our approximation are justified and good (i.e are we doing what we want to), which is what we verify in this section.

Note the main point for computing $e$ instead of the true discrepancy is simply that, as you'll see with our experimental setup described in \ref{ssec:verifying experimental setup}, the true discrepancy requires computing the properly retrained model $M'$, and so in practice having to compute $M'$ to assess error would negate the computational benefit of the approximate unlearning method. It is also not clear what exactly one needs to change to reduce the verification error, however it is more apparent with unlearning error.

However, as will be the main takeaway from this section, decreasing $e$ with the methods we've described earlier does in fact decrease the true discrepancy and the correlation between $e$ and the true discrepancy is very strong; thus one can reasonably only work with $e$ to compare how effectively one has unlearned.

\subsection{Experimental Setup}
\label{ssec:verifying experimental setup}
We are interested in determining what is the relationship between our proposed unlearning error in equation~\ref{eq:error bound} with the actual error in a practical setting, the true discrepancy as we've been calling it. Using the taxonomy defined in section~\ref{sec:define_unlearning}, we are interested in the relationship between the difference of our unlearned model compared to the gold standard of retraining ($||\model^{'} - \model^{''}||_{2}$) and our unlearning error. From now on we'll also refer to $||\model^{'} - \model^{''}||_{2}$ (the true discrepancy) as verification error, for reasons more apparent when we make the connection to proof of learning. 

The experiments in this section will be for the same models and datasets introduced in section~\ref{ssec:experimental setup}, and we modify the experimental procedure from section~\ref{ssec:experimental setup} as follows:
\begin{enumerate}
    \item Pretrain $\model_{0}$ by training $\model_{0}$ on the entirety of $D$ for N steps until we reach $\model_{N}$.
    \item Train $\model_{N}$ for a small number of steps $T$ on batches of data $\{x_1,x_2,\dots,x_T\}$ to get $\model_{N+T}$. We will consider $\model_{N+T}$ the model we wish to unlearn and WLOG the point we wish to unlearn is in batch $x_{1}$.
    \item Train $\model_{N}$ for $T-1$ steps on batches $\{x_2,\dots,x_T\}$. The resulting model is the naively retrained model $\model^{'}$ without batch $x_{1}$.
    \item Get $\model^{''}$ via adding back the gradient in the easy to compute term:
    $$ M^{''} = M_{N+T} + \eta  \frac{\partial L}{\partial w}|_{w_{N+T},x_1}$$
    \item Compute the unlearning error of $M_{N+T}$ and the verification error ($||\model^{'} -\model^{''}||_{2}$).
\end{enumerate}
Again, depending on the experiment we compute the unlearning error and verification error at regular intervals during the finetuning process.

\varun{what are the datasets used? what are the model architectures used?}\anvith{same as last time, added/modifed the sentence just before the enumeration}




\subsection{Experimental evidence}
%\anvith{for gabe: present here the experimental evidence showing that the methods we considered earlier for decreasing unlearning error are indeed decreasing the true discrepency}

\varun{i find the section on pretraining distracting as in 4.1 and 4.2 -- you've established why you'd not want to do it; the discussion in this section is also very thin -- you basically conclude with "there's strong correlation". no discussion on "why". }
\anvith{I think showing pretraining is still important, as the underlying phenomenon is the correlation with t, which strictly speaking we have no justification for why verification error should increase with unlearning error when increasing t}
\anvith{I'm adding more discussion, but the main "why" is that unlearning error is a good metric for verification error, this is to just prove this- tying back to the opening paragraphs to section 5}


\subsubsection{Changing t}

%The main underlying assumption for pretraining is that varying t varies the unlearning error $e$ proportionally; thus, with $t$ being our only variable, we'd like to see that the true discrepency and unlearning error are positively correlated, meaning that with pretraining we are in fact reducing the true discrepency when we are reducing the unlearning error (which is what we can relatively cheaply measure).

What we saw from Figure~\ref{fig:unl_t} is that unlearning error increases with t; the follow up question is now whether verification error does in fact increase with t, or more generally, with t as our only variable, is unlearning error and verification error correlated.

Figure~\ref{fig:pretrain} shows the relationship between the verification error and the unlearning error as a function of the number of SGD steps taken (i.e $t$). The model is a ResNet-18 pretrained for 80 epochs on CIFAR10 and then performs steps 1-5 in section~\ref{ssec:experimental setup} for $T=14000$ steps or approximately 5 epochs of training. The main takeaway here is that the verification error and unlearning error have a strong correlation of $0.9668$, and thus when we reduce the unlearning error with pretraining, we reduce the true discrpency.

%Furthermore, We also see that both verification and unlearning error are a similar function of $t$, and so we can conclude that when varying $t$, if we decrease unlearning error, we also decrease the true discrepancy; thus our assumption for pretraining . 

%\gabe{does this make sense? I think it's poorly worded, need to fix IMO} \anvith{I've reworded it a bit, basically the point is we want to state first the assumption for pretraining was varying t proportionally affect unlearning error, and we want to show that with this as our only variable, we have a strong correlation between verification error and unlearning error, which is what that figure shows; thus we conclude that our assumption for pretraining was correct, and thus pretraining is applicable}.

As another takeaway, these results also agree with the intuition behind why unlearning deep neural networks trained with iterative methods such as SGD are difficult. Even though $\model$ and $\model^{'}$ differ by a single batch, once the differing batch occurs during training, $\model$ and $\model^{'}$ begin to take two different sequences of updates and begin to diverge. As you increase the number of steps that a model learns for, the model is left to continue to diverge further and further, which is shown by the verification error increasing as a function of $t$.



\begin{figure}
    \centering
    \includegraphics[width = 3.2in]{plots/pretrain_plot.png}
    \caption{Unlearning error and verification error as a function of the finetuning steps (indicated by the color gradient) for ResNet-18 on CIFAR10. Unlearning error and verification error are measured every 100 SGD updates for a total of 14000 SGD updates. The correlation between unlearning error and verification error as a function of $T$ is 0.9668. Both unlearning error and verification error increase as a function of the number of finetuning steps}
    \label{fig:pretrain}
\end{figure}

\subsubsection{SD Loss}


\varun{could you explain, with the pearson coefficient values, why the correlation is strong in the text description as well?} \anvith{added}

As seen in figure~\ref{fig:corr_std_loss} we have a strong correlation between unlearning error and the verification error for ResNet-18 and VGG-19 on CIFAR10 of 0.96 and 0.81 respectively when varying the strength of our SD regularization; in fact for VGG-19 we see the relation between verification error and the regularization is stronger than that for unlearning error (note the y-axis in \ref{fig:corr_std_loss} (b) continually decreases with the strength of the regularization where as the x-axis has some noise).

%Thus the main takeaway here is that only changing the SD regularization, when we decrease the unlearning error we also decrease the verification error, and so we were justified in looking solely at the unlearning error (which is easier to compute).

This is a strong result, as only reasoning with the verification error, it is not clear how one might've come to the SD Loss to reduce it. This also shows more generally that the unlearning error accurately proxies the verification error when varying our loss function.

\begin{figure}[htp]
  % Fixed length
  \centering
 \subcaptionbox{ResNet-18\label{fig2:a}}{\includegraphics[width=1.6in]{plots/std_loss_correlation_resnet_cifar10.png}}
  \subcaptionbox{VGG-19\label{fig2:b}}{\includegraphics[width=1.6in]{plots/std_loss_correlation_vgg_cifar10.png}}
 \caption{Correlation between unlearning error and verification error for ResNet-18 and VGG-19 on CIFAR10 as a function of the regularization strength. The correlations are both high at 0.96 and 0.81 for ResNet-18 and VGG-19, respectively. Notice that the stronger the regularization (more blue) the more the verification and unlearning error decrease in both settings.}
\label{fig:corr_std_loss}
\end{figure}


\subsubsection{Considering all Models}


\varun{what are the parameters you vary in fig~\ref{fig:big_final_corr}?} \anvith{@gabe can you add it somewhere in the text: I believe it was just loss, regularization strength, finetuning steps, pretraining amount, model, and datasets}

Lastly as seen in figure~\ref{fig:big_final_corr} where we consider a 160 different variations of the methods and settings we've considered, we see that in general, regardless of architecture, when a model with a specific setup (one of the ones we've been considering) has lower unlearning error, it has lower verification error, as we see by the strong positive correlation between unlearning error and the verification error across the different settings and architecture considered.

This result is highly non-trivial, as simply using the number of training steps as a proxy for verification error (with the rather intuitive reasoning behind pretraining that error increases with steps), we would not be able to tell if one model had a higher error than another when trained the same number of steps, nor how a loss function might change this error.

\anvith{@varun added this to reiterate why this works, going back to the opening paragraphs for section 5}
In the end the reason why unlearning error does in fact serve as a good proxy for the true discrepancy is simply the mathematical basis for it presented in section \ref{sec:approximation}, which relied on several approximations but as we've seen in this section the metric still works (at least for all the scenarios we've considered).

\begin{figure*}[htp]
  % Fixed length
  \centering
 \subcaptionbox{CIFAR10\label{fig2:c}}{\includegraphics[width=3.26in]{plots/Large_correlation_cifar10.png}}\hspace{1em}%
  \subcaptionbox{CIFAR100\label{fig2:d}}{\includegraphics[width=3.26in]{plots/Large_correlation_cifar100.png}}\hspace{1em}%
 \caption{Unlearning and verification error for 160 settings across CIFAR10 and CIFAR100. The correlation between unlearning error and verification error for CIFAR10 and CIFAR100 are \textbf{0.9028} and  \textbf{0.8813}, respecively. Settings trained with SD loss (green) for both datasets have lower unlearning and verification error then those trained with regular cross entropy (red).}
\label{fig:big_final_corr}
\end{figure*}

==> Contents/Other_Metrics_and_Verification_Error.tex <==
\section{Other Metrics and Verification Error}
\anvith{I think we need to to the POL discussion before this for better context}

So far we've introduced and justified our unlearning error as a good metric for unlearning, as it serves to accurately represent the verification error which captures how close we are to truly unlearning, and has the added benefit of capturing the success rate of a proof of unlearning using the final weights given by an approximation (the verification error being the same verification error introduced by Jia et al in \cite{jia2021proof}). 

However the question now turns to whether other metrics used in the literature succeed in capturing the verification error.

\subsection{Membership Inference}

Memberhsip inference is used in several papers \cite{} as a metric to asses the effectiveness of unlearning. As discussed in the background, the justification for membership inference as a metric follows from definition (b) for approximate unlearning which looks at the similarity of outputs. However as outputs aren't what uniquely defines a model and the dataset it was trained on (two models trained on different datasets can have similar outputs if the datasets are similar enough) it is desirable to see if membership inference also captures definition (a) for approximate unlearning.

So to evaluate the relation between membership inference and verification error, we look at privacy risk score as introduced by Song et al \cite{song2021systematic} which they showed accurately captures the likelihood a data-point is a training point (i.e has a strong correlation with thelikelihood a data-point is a training point). They showed this method works even when the model employs membership inference defences such as Memguard [24] and AdversarialRegularization [25]. Fundamentally, the PRS score gives avalue between 0 and 1, where 0 (based on their experimentalevidence) means not likely to be a training point, and 1 is very likely to be a training point. 

\anvith{point below is that MI doesn't work well, and the fact it's not effective to SD Loss is a testament to how dependent it is on it's effectiveness}

As we've shown in section \ref{sec:SD_Loss_MI}, our SD Loss breaks the effectiveness of PRS score and so already shows one of the issues with membership inference- it's effectiveness. But regardless, for now the question is whether PRS score (a state of the art measurement for membership inference likelihood) is correlated to verification error under the methods we've introduced to change verification error (via association with unlearning error). To do this we consider a similar setup to figure \ref{fig:big_final_corr} however now we study the correlation between the verification error and privacy risk score. We see in \ref{fig:corr_prs_ver_err} that the correlation is relatively weak, with scores of -0.35 and 0.16 for CIFAR-10 and CIFAR-100; a far-cry from the statistically strong result we saw with unlearning error in \ref{fig:big_final_corr}.  

This shows that membership inference, or at least privacy risk score, wouldn't serve as a good proxy for verification error.


\begin{figure}[htp]
  % Fixed length
  \centering
 \subcaptionbox{CIFAR-10\label{fig2:a}}{\includegraphics[width=1.6in]{plots/MI_VER_corr_CIFAR-10.png}}
  \subcaptionbox{CIFAR-100\label{fig2:b}}{\includegraphics[width=1.6in]{plots/MI_VER_corr_CIFAR-100.png}}
 \caption{Correlation between privacy risk score (metric for unlearning used in~\ref{graves2020amnesiac} and other works) and verification error for CIFAR-10 and CIFAR100. The respective correlations for both datasets are -0.35 and 0.16, both statistically weak correlations.}
\label{fig:corr_prs_ver_err}
\end{figure}

\subsection{Similarity in Final Weights Probability Distributions}

The main result of section \ref{sec:The analysis of Probability Distributions} was that verification error (which makes up a component of $d_I$ in that case) is related to the max $\ell_2$ difference in the probability distributions when training with and without $x^*$, given by the upper bounds \ref{eq: l2_prob_difference_1} and \ref{eq: l2_prob_difference_2}; in this sense we see lower verification error means a smaller $d_I$, and thus a smaller bound on the difference, and so we see one direction of the relation between verification error and probability distribution shifts.

%and thus in a sense its relation to other metrics capturing things related to shifts in the probability distributions like KL-divergence used by Golatkar et al \cite{golatkar2020eternal},and the certified $\epsilon$ gurantee used by Guo et al \cite{guo2019certified}

Going the other way, showing a smaller max $\ell_2$ difference means a smaller bound on verification error, let's focus on the expectation of the difference in weights $d = E(\eta m\frac{\partial L}{\partial w}|_{w_{0},x^*} + \textit{verification error})$, which is simply the difference in expectation of $P(w)$ and $P'(w)$, and let us for the time being assume that the union of the support of $P(w)$ and $P'(w)$ is bounded, i.e if $\mathbf{W}$ is the union of the supports, then $\int_{\mathbf{W}} ||w||_{\ell_2} dw = v < \infty$. This is reasonable as we'd expect the noise from training to be bounded; in fact in general we'd only need the integral outside a bounded domain to be finite, but the reasoning is analogous to what follows. Now if say $||P(w) - P'(w)||_{\ell_2} < b$ for some scalar $b$, we have:

\begin{multline}
\label{eq:exp_ver_err}
d = ||E(P(w)) - E(P'(w))||_{\ell_2} &= ||\int_{\mathbf{W}} P(w) w dw - \int_{\mathbf{W}} P'(w) w dw||_{\ell_2} &\leq \int_{\mathbf{W}} ||P(w) - P'(w)||_{\ell_2} ||w||_{\ell_2} dw &\leq bv
\end{multline}

and so in this sense we see reducing the max value of $||P(w) - P'(w)||_{\ell_2}$ gives a smaller bound on $d$ and thus a smaller bound on the expectation of verification error as the expectation of verification error is bounded by $d$.

Thus we see the relation between verification error and $||P(w) - P'(w)||_{\ell_2}$ runs both ways (i.e reducing either gives a tighter bound on the other), and as $||P(w) - P'(w)||_{\ell_2}$ captures the difference in probability distributions when training with and without a datapoint $x*$, we generally expect similar metrics trying to minimize the shift in the probability distributions would follow similar relations as described above.

That is metrics such as KL divergence, certified epsilon gurantee, DP bounds, etc would likely be equivalent to verification error, based on the assumptions and analysis we've presented here and in section \ref{sec:The analysis of Probability Distributions}; we leave it to future work to empirically verify this.

\anvith{above is place-holder until we test whether DP bounds work}

However in general, to obtain those metrics would be more expensive than obtaining our unlearning error $e$, which is one of the main benefits of $e$.



==> Contents/POUL.tex <==
\section{\texit{True Discrepancy} and Proof of Learning}

What follows is another way of conceptually grasping our unlearning error, and in particular, the true discrepancy it approximates (which we for reasons that will now be clear have started calling it verification error). How we've introduced it and used it so far is that true discrepancy measures how far away we are from perfectly unlearning, however as we'll discuss, there is a natural way to talk about a \texit{proof of unlearning} based on the work done by Jia et al \cite{jia2021proof}, which also introduces \texit{verification error} to measure whether a said proof of learning should be accepted. In a specific context, this verification error is in fact the true discrepancy we've been working with, and so alternatively we can say our unlearning approach amounts to giving a \textit{cheap proof of unlearning} as we explain below; this we believe illustrates a viable practical procedure unlearning may be employed and verified by an entity and government.

\subsection{Proof of Unlearning}

A Proof of Learning $\mathfrak{P}$ is a a tuple consisting primarily of an ordered set of checkpoints $\mathfrak{W}$ taken during training with some check-pointing frequency $k$, and the ordered sequence of data points $\mathfrak{X}$ appearing during training, alongside various hyper parameters needed to reconstruct training. We say that $\mathfrak{P}$ is valid only if the associated verification error, i.e the difference between what an entity says they obtained for their weights at the n'th checkpoint, and what the verifier obtained when recreating the sequence of weights, is always below some threshold.

Thus if an entity claims to have unlearned, i.e to have never trained on $x^*$, we could explicitly verify this by asking for a $\mathfrak{P}'$ such that $x^* \not\in \mathfrak{X}'$. If this $\mathfrak{P}'$ passes verification, then we can say this is a \textit{proof of unlearning}.

\subsection{Costs and Becoming lazy}

The issue with the setup above is that providing $\mathfrak{P}'$ requires explicitly retraining, as based on the work from Jia et al \cite{jia2021proof}, obtaining a valid cheaper spoof is difficult (currently have no such methods). So in practice, as of now, obtaining a proof of unlearning means retraining, and thus is expensive.

However we can be lazy, and instead of properly retraining immediately after getting an unlearning request in order to obtain a valid $\mathfrak{P}'$, we instead only obtain the final weights of a valid proof (possibly cheaply by approximating them) and compute the rest of the proof some time in the future when it is needed; the benefit to this strategy is not having to retrain every time a request is sent, and only doing it once upon needing to provide a proof (saving costs). 

The associated verification error (more precisely the error in verifying the only step that might not pass verification which is the last one) is then the difference between the final weights you computed, and final weights you would obtain from the true $\mathfrak{P}'$.

Here, the final weights obtained by this valid $\mathfrak{P}'$ are the weights of $M'$, and using our approach the approximated final weights one would have obtained are those of $M"$. Thus the verification error is simply the difference in these two weights, which is what we've been calling the true discrepancy.

So we see in this context that our true discrepancy and the verification error from POL (proof of learning) are the same. A future direction of work could be to find a way to distribute this error throughout the steps in the proof as to pass verification more easily (that is to push each of the weights slightly in the direction of the final weight of $M''$ when retraining, as to distribute the error across the steps, and possibly pass verification for each step); doing this we'd understand by association the unlearning error we should aim for- that which roughly corresponds to the desired verification error which when distributed over the steps would pass verification.



%\anvith{going to finish this after taking a nap... 6am is way too early to start a day}

%Now we've been working with, and mainly trying to minimize, the \texit{true discrpency}, the actual difference in weights between $M'$ (a properly unlearned model) and $M''$ (the approximation of $M'$ we obtain), throughout the paper, and introduced this specific measurement as something relatively new. However this difference is in fact the \texit{verification error} used by Jia et al \cite{jia2021proof} in their Proof of Learning scheme.

%Essentially

==> Contents/Prob_distribution_analysis.tex <==
\section{The analysis of Probability Distributions}
\label{sec:The analysis of Probability Distributions}
%\anvith{So, I think it makes sense to present the results here as theorems and then give the proofs in the appendix, but we can decide that later depending on what we all think}


\anvith{reworded this paragraph to set it up in context of what we're previously doing}
Up to now we've focused on understanding unlearning from a deterministic view, treating noise and other issues as being negligible. This we've seen allows to capture what factors change when we remove a datapoint $x^*$ from the dataset while training, and how we can use this to unlearn and measure our associated error. This view of unlearning and data removal is seemingly different from the probablistic view taken by Guo et al \cite{guo2019certified} and Golatkar et al \cite{golatkar2020eternal} where they look at the changes in distributions of weights. However what follows is how we can see the relation between these views.

Here we will compare the probability distributions of final weights coming from training $m$ epochs starting at a fixed initial weight $w_0$ with dataset $D$ and dataset $D'= D-x^*$ with SGD (and not mini-batch sgd, i.e considering batch size is 1); we will represent the density functions respectively as $P(w)$ and $P'(w)$.

Before proceeding, if we let $n$ be the size of $D$, let us denote $I = \{x_{i_1},x_{i_2},\cdots,x_{i_{mn}}\}$ as a particular ordering of the datapoints when training on $D$ for $m$ epochs; note we have $(n!)^m$ such combinations, for $D'$ we have $(n-1)!^m$ such combinations. To each $I$, we associate to it $I' = I-x^*$ where here $I-x^*$ means removing all the instances of $x^*$ in $I$ while preserving the ordering. Note for a given $I'$, which is an ordering of batches when trained on $D'$, we have $n^m$ corresponding $I$ as for each epoch we have $n$ choices to place $x^*$ per epoch, and $m$ epochs in total.

\anvith{this paragraph is mostly new, I bascially made the definition of $w_I$ and $w_{I'}$ more formal}
Now, let $w_I$ represent the deterministic final weights resulting from training with the data ordering $I$ starting from $w_0$, and we now introduce the random variable $g_I$ which represent the noise when training with $I$, and so the random variable representing the final weights when training with $I$ is $z_I = w_I + g_I$. Similarly, we define $z_{I'} = w_{I'} + g_{I'}$. Note that if training is deterministic, we have $w_{I'} = w_{I} - d_I$ where $d_I$ is some constant that only depends on $w_0$, which we've fixed, and the ordering $I$ (as $I'$ is function of $I$ as described earlier by definition); this $d_I$ is what we've been approximating earlier in this paper. Lastly, we make an assumption that the noise from training with $I$ is the same as when training with $I'$, that is $g_{I} = g_{I'}$; this is based on the fact that this noise should only be a function of the number of training steps, and that noise per step is negligible (i.e almost 0), and so adding or removing $m$ steps (1 per epoch) when compared to the $nm$ total steps when training with ordering $I$ is insignificant. Thus we have $z_{I'} = z_{I} - d_{I}$.


%if $z_I$ denotes the random variable representing the output weights when training on $D$ with that particular batch ordering ($I$), and if $z_{I'}$ represent the random variable representing the output weights when training on $D'$ with the corresponding $I'$, note $z_{I'} = z_{I} - d_{I}$ where $d_{I}$ is some constant depending on $I$ and the initial weights $w_0$, both of which we've fixed here; this $d_{I}$ is what we've been trying to approximate in our previous sgd analysis, and this $d_{I}$ represents the change in weights between training with $I$ and $I'$ when training is deterministic.

Now note that, assuming the probability of a given batch ordering is constant (i.e a uniform distribution of batch orderings), and if $P_{I}(w)$ is the density function corresponding to $z_I$ and $P'_{I'}(w)$ is the density function corresponding to $z_{I'}$ (which note by above is equal to $P_{I}(w-d_{I})$), then $P(w) = \frac{1}{n!^m}\sum_{I}P_{I}$ and $P'(w) = \frac{1}{(n-1)!^m}\sum_{I'}P'_{I'}(w)$.

Thus we have:
\anvith{corrected slight typo in below calculations}
\begin{multline}
||P(w) - P'(w)||_{\ell_2} = ||P(w) - P'(w) + \frac{1}{n!^m}(n^mP'(w) - n^mP'(w))||_{\ell_2} &\leq ||\frac{1}{n!^m}\sum_{I} P_{I}(w) - P'_{I'}(w)||_{\ell_2} + |(\frac{n^m}{n!^m}-1)|P'(w) &\leq \frac{1}{n!^m}\sum_{I} ||P_{I}(w) - P_{I}(w-d_{I})||_{\ell_2} + |(\frac{1}{(n-1)!^m}-1)|P'(w)      
\end{multline}

\anvith{added sentence to below paragraph explaing the step form the first line to the second, an why we can do this without indexing issues}
Where for the step from the first line to the second line follows form noting that by having $n^m$ copies of $P'(W)$ we can associate to each $P_I(W)$ it's corresponding $P'_{I'}(w)$, which comes from the previous remark on counting of $I$ and $I'$. Also here $||\cdot||_{\ell_2}$ simply represents the euclidean norm.

Now if we assume every $P_I$ is lipschitz, then $||P_I(w) - P_I(w-d_{I})||_{\ell_2} \leq L_I||d_I||_{\ell_2}$, and thus from the above we get 

\begin{equation}
\label{eq: l2_prob_difference_1}
||P(w) - P'(w)||_{\ell_2} \leq \frac{1}{n!^m}\sum_{I} L_I||d_I||_{\ell_2} + |(\frac{1}{(n-1)!^m}-1)|P'(w)
\end{equation}


From this last expression, using the fact $P(w) - P'(w) \leq ||P(w) - P'(w)||_{\ell_2}$, we get the bound

\begin{equation}
\label{eq: Prob_distribution_bound_1}
P(w) \leq \frac{1}{n!^m}\sum_{I} L_I||d_I||_{\ell_2} + (\frac{1}{(n-1)!^m}+2)P'(w)
\end{equation}

which captures one direction in the difference in probability distributions.

For the other direction, to each $I'$, say $I'_j$, we associate $I'_{min} \in \{I~s.t~I' = I'_j \}$ s.t $L_{I'_{min}}||d_{I'_{min}}||_{\ell_2} = \min_{I~s.t~I' = I'_j} L_{I}||d_{I}||_{\ell_2}$. We then have, 

\begin{multline}
\label{eq: l2_prob_difference_2}
||P(w) - P'(w)||_{\ell_2} = ||P'(w) - P(w) + \frac{1}{(n-1)!^m}\sum_{I'}P_{I'_{min}} - \\ \frac{1}{(n-1)!^m}\sum_{I'}P_{I'_{min}} ||_{\ell_2} \\ &\leq 
\frac{1}{(n-1)!^m}\sum_{I'}||P_{I'} - P_{I'_{min}}||_{\ell_2} + (\frac{1}{(n-1)!^m} - \frac{1}{(n)!^m})\sum_{I'}P_{I'_{min}} + \\ \frac{1}{(n)!^m}\sum_{I \notin \{I'_{min}\}}P_I \\ &\leq \frac{1}{(n-1)!^m}\sum_{I'}L_{I'_{min}}||d_{I'_{min}}||_{\ell_2} + (\frac{1}{(n-1)!^m} - \frac{1}{(n)!^m})\sum_{I'}P_{I'_{min}} + \\ \frac{1}{(n)!^m}\sum_{I \notin \{I'_{min}\}}P_I \\ 
\end{multline}

and now noting $P'(w) - P(w) \leq || P'(w) - P(w)||_{\ell_2}$, we get the other bound

\begin{multline}
\label{eq: Prob_distribution_bound_2}
P'(w) \leq \frac{1}{(n-1)!^m}\sum_{I'}L_{I'_{min}}||d_{I'_{min}}||_{\ell_2} + \frac{1}{(n-1)!^m}\sum_{I'}P_{I'_{min}} + \\ \frac{2}{(n)!^m}\sum_{I \notin \{I'_{min}\}}P_I
\end{multline}

\anvith{added this paragraph to remark that we do indeed of $P(w)$ on the right-side, albeit with a bit extra}
Note that this right side has a term $\min(\{\frac{1}{(n-1)!^m},\frac{2}{(n)!^m}\})P(w)$ and some extra terms for some of the components of $P(w)$.


\subsection{Relation to Unlearning error and Some Intuition}

As remarked $d_I$ represents the deterministic difference between training with $x^*$ with the ordering $I$ and not; this is what we approximated in our section analyzing sgd, which we noted was approximated by $d_I \approx \eta m\frac{\partial L}{\partial w}|_{w_{0},x^*} + \textit{higher order terms}$, where $m$ is the number of epochs (i.e the number of times $x^*$ appears in training). We then further approximated these higher order terms, and saw we can model it with our unlearning error $e$; decreasing $e$ we've seen decreases the impact of the higher order terms.

As a consequence we have decreasing $e$, i.e with our SD Loss, also decreases $d_I$, and thus decreases our bounds \ref{eq: Prob_distribution_bound_1} and \ref{eq: Prob_distribution_bound_2} relating the probability shifts. It should be noted that these bounds may be very loose, but nevertheless we have an understanding for the mechanism that relates the deterministic view and the probabilistic view.

Lastly, to get some more intuition for what is going on in our bounds, let us focus specifically on the bound on the $\ell_2$ difference in \ref{eq: l2_prob_difference_1}. We see by increasing n (the size of the dataset) we decrease all the terms (albeit we increase the possible number of $I$ and so sum over more terms), so larger datasets to some extent mean less discrepancy in the final weight distribution due to losing a single data point for our bound. The term $d_I$ is what we explained above, and so in fact minimizing it (via our unlearning method applied post-hoc to $P(w)$ and our various methods to reduce the associated unlearning error) reduces the sum. Lastly the smaller $L_I$ the "flatter" or more "uniform" the probability distribution is and also the smaller the first sum; for example, if the noise $g_I$ was gaussian, then increasing the standard deviation would decrease the lipschitz constant, and thus decrease our bound (so higher standard deviation noise means the more similar the distributions when training on $D$ or $D'$ are).

%This last remark on high standard deviation decreasing differences in probability distribution differences was in fact remarked upon by Golatkar et al \cite{golatkar2020eternal} where they focus on the KL-divergence.

%Here $d_I$ is simply the difference between the final weights obtained by training with $D$ with fixed $I$, i.e the weights of $M$, and the final weights obtained by training with $I'$, i.e the weights of $M'$; we note this difference is approximated by our unlearning rule of adding $\eta  \frac{\partial L}{\partial w}|_{w_{0},x^*}$ with associated error which is our unlearning error. So in total $d_I \aprox \frac{\partial L}{\partial w}|_{w_{0},x^*} + \textit{e}_I$ where here $\textit{e}_I$ is the true discrepancy which we've seen we can approximate (without keeping true to scale) by our unlearning error. And so by decreasing our unlearning error we decrease $d_I$ and thus the above bound.

\subsection{In context with other work}

What we've now shown is that our unlearning error captures to some extent the differences in probability distributions, and by decreasing it we decrease that difference. In this regard we see our metric for unlearning is related to the analysis of probability distribution shifts for unlearning seen in the work by Guo et al \cite{guo2019certified} and Golatkar et al \cite{golatkar2020eternal}. As discussed in the background, Golatkar et al \cite{golatkar2020eternal} use KL divergence as measure for the differences in distributions, where as Guo et al \cite{guo2019certified} define $\epsilon$-certified removal (i.e their measure for how close the distributions are) as $e^{-\epsilon} \leq \frac{P(w)}{P'(w)} \leq e^{\epsilon}$, which is similar to differential privacy, but not quite; as they remark, differential privacy gives sufficient conditions for this.

Our above bounds are most reminiscent of the type of bounds discussed by Guo et al \cite{guo2019certified}, however not quite as we have additional constant terms and we double-count some parts of $P(w)$ in \ref{eq: Prob_distribution_bound_2}. Nevertheless, this illustrate the relation between the deterministic view and the probablistic view, and perhaps explains the effectiveness of our SD loss on both unlearning error and membership inference attacks (via making the distributions less distinguishable).

Also the dependency on $L_I$ which is specific to the noise suggests that one might be able to control this bound by better understanding the noise when training; Jia et al \cite{jia2021proof} show that viewing training as a markov process that entropy from noise grows linearly, however that is to the best of our knowledge the only work relevant to understanding the noise. Alternatively one could simply add noise to change $L_I$, and this would suggest DP like procedures to decreasing this bound. 

Lastly for the reader who is justified in wondering what really differentiates this from DP bounds, a simple consideration is that all we've specifically looked at is the differences for some of the possible adjacent datasets to a dataset $D$ (i.e those obtained by taking away a data point), and not those that could come from adding a datapoint. 

%It is perhaps a question for the community whether what we're really interested in for privacy leakage is the former and not the latter (clearly the former is what is of interest for unlearning).










==> Contents/Unused/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}



The goal of machine unlearning to to provide a mechanism for removing the impact a data point in the training set had on the final model; forgetting that datapoint, so to say. Simply assuming the impact a single datapoint had on the final model is negligible and doing nothing is naive as a ML model can memorize some of its training data~\cite{carlini2019secret,fredrikson2015model}. This motivates the development of machine unlearning in multiple settings. In privacy, a model which has not unlearned may leak~\cite{shokri2017membership, abadi2016deep} some of the private information contained in a point even after the user who initially contributed to the model's training set revoked access to their data---a possibility popularized by the right-to-be-forgotten in the GDPR~\cite{mantelero2013eu}\my{this sentence should be reversed. start with the motivating example of GDPR and then explain the privacy angle of it} \anvith{I think the idea of revoking is more general than the motivation, no?}. In the presence of an adversary~\cite{gu2017badnets}, a model owner may realize that some of its training data was poisoned by the adversary; without unlearning it is unclear how much of the poisoned samples' effect is remaining within the model. More generally, machine unlearning affords a natural mechanism for patching ML models, especially when it is combined with fine-tuning techniques~\cite{torrey2010transfer,tan2018survey}. 



\gabe{Phrase it as 3 ways, where the third is approximate unlearning, not retraining. ie: no retraining is performed at all. we should say that this is the easiest for model owners to peform unlearning and is currently only studied poorly}.\anvith{I think just the two ways, but have changed the second to approximate unlearning}

There are currently two broad approaches to machine unlearning: retraining and approximate unlearning. With retraining, the point to be unlearned is removed from the training set, and a new model \gabe{"newly initialized model", ie: it is the same model, same hyperparameters, but just on D-$x^{*}$}\anvith{think new model means the same thing no?} is trained from scratch on this updated training set. This approach has the advantage of carrying a strong intuition for why the new model was not influenced in any ways by the point to be unlearned\my{potential re-write: This approach has the advantage that through exclusion of a sample, the model owner can soundly claim that  the sample can have no impact on the model whatsoever}\anvith{leaving as is now becuase I think both are the same, but intuition is more true as we are not sure how a claim is verified yet- proof of unlearning}. 


This is a non-trivial advantage when unlearning needs to be transparent, e.g., in the context of right-to-be-forgotten requests. Naively retraining from scratch can be made more efficient if the model owner adapts their initial training procedure to analyze training data in a carefully chosen order and saves intermediate model parameter states, as demonstrated by the SISA framework~\cite{bourtoule2019machine}. \gabe{should we add the negative of retraining here? Because it seems like we are saying exact retraining is really good and we do not really address how it is not good enough for unlearning techniques, which is why we need cheaper, but maybe not perfect methods (ie: approximate unlearning)} In approximate unlearning,\nj{do you consider the influence-function based methods part of approximate retraining? If so maybe mention it (e.g. as an example) since it is well known in this field}\anvith{gonna leave as now, worth thinking about} the model owner instead chooses to keep the same model and rather change the final weights \gabe{parameter updates is too restrictive, some work just removes certain logits or layers. Phrase as "additional transformations"} as to reach a similar model (in however sense similar is defined) to a model exactly retrained. This can be done for example through a form of gradient ascent~\cite{graves2020amnesiac}, which is the opposite of gradient descent performed to train the model normally. Approximate retraining has the advantage of being more computationally efficient than exact retraining but this comes at the expense of a guarantee that is less intuitive and harder to understand for an end user. \nj{I guess you could also say most approximate methods do not guarantee 100\% of the impact of the data point is removed}\gabe{In response to Nick's comment: "Approximate methods have the benefit of being significantly faster than exact retraining methods at the cost of not being able to guarantee that the impact of the data point is removed in its entirety".}

%\anvith{for future self-note, as we have a new loss, and the results are very very strong (almost 0 error) we can make stronger claims in this paragraph, also should emphasize how this focus on analyzing the error through SGD is novel, and also the recent analysis linking it back to more probabilistic views that are agnostic to the exact behaviour of training}

In this paper, we demonstrate that this dichotomy is not necessary. We present an analysis of stochastic gradient descent---the most common learning algorithm and the de facto choice for training deep neural networks---which allows us to effectively assess the error of approximate approaches to unlearning. Such an analysis is made difficult by the stochasticity, recursiveness, and inherent entropy\my{this is not a well defined terem for me. May want to not use it before defining it precisely.} from implementations of stochastic gradient descent. This metric for unlearning is useful in two ways. First, an objective comparison of existing approaches to unlearning follows naturally from this bound: we are able to interpolate between an exact retraining approach achieving an unlearning error of 0, approximate approaches achieving a non-zero error, and the absence of unlearning resulting in an high unlearning error. Second, our metric for unlearning error provides insights into aspects of stochastic gradient descent that are important for designing new training and unlearning algorithms that best approximate exact unlearning. One of our key contributions as a result of this is to propose a new \textit{standard deviation (SD) regularizer} to facilitate better unlearning, which we see can have drastic impacts on certain architectures with no additional changes to the training pipeline.

Intuitively, our approach to defining unlearning error can be interpreted as ``unrolling'' stochastic gradient descent to capture the effect of earlier updates on later updates.\my{I think we need another sentence here explaining intuitively what unrolling is before moving on into its motivation/advantage} Unrolling allows us to characterize the contribution of a training point on the model's parameters throughout training, what part of this contribution we can forget cheaply, and in particular what we can not quite forget, which is our associated error.\my{this last which clause can be removed here. o.w. the sentence is too long.} 
During training, we log some of the variables involved in our final  error metric (i.e the top singular values) to analyze post-hoc the error achieved when unlearning. This allows us to quantify\nj{estimate?} the unlearning error that one would experience when unlearning by simply adding back gradients taken with respect to the initial weights as proposed by our analysis; it is this error that we can significantly drop by using our \textit{SD Loss}.\my{these two sentences need a re-write. Make them less technical and more intuitive if possible.} \nj{try to be consistent in terminology -- you used SD regularizer earlier}

We further show experimentally that this metric does in fact capture the true discrepancy which we are trying to capture, by considering various situations and showing the correlation between the true discrepancy and our error is very strong.

Furthermore, we also show that our SD loss breaks the strong correlation between privacy risk score and the likelihood of being a training point, as proposed by Song et al \cite{song2021systematic}. We find that our unlearning error is also related to a bound on distribution shifts in final weights when training/not training with a specific data point~\cite{guo2019certified}; as a consequence this suggest that decreasing our unlearning error would make it harder to distinguish between a model trained with and without a datapoint, possibly explaining why our SD Loss broke privacy risk score, and linking our unlearning error to the intuitive definition of privacy leakage as a measure of how well someone has unlearned. \nj{the previous sentence is too long}


%Our experiments on X, Y, Z trained on A, B, C show that INSERT \anvith{@gabriel want to briefly write the main takeaways from our experiments, particularly what we can do with reducing it, not the choice of 3 here is more or less arbitrary}. To provide some intuition for why our approach captures the effect of unlearning accurately, we test our approach by measuring the success of membership inference on our models before and after unlearning. We chose to use membership inference because it is perhaps the most well-understood attack on private information contained in the training set.\todo{anvith + gabe: read this past paragraph and introduce some specifics of your approach} \anvith{I think this is really the paragraph where we describe at a high-level our experimental results, so @gabriel maybe take a crack at this after finishing the experiments section below}

Finally, our approach shares certain conceptual insights with the proof-of-learning (PoL) framework of Jia et al.~\cite{jia2021proof}. PoL introduces a logging mechanism which enables a model owner to provide a third party with a verifiable proof that they have expended the compute resources needed to perform stochastic gradient descent, and that the integrity of stochastic gradient descent is guaranteed. Such a proof contains certain information about intermediate states of the model (i.e., its parameters) and entropy sources (e.g., which minibatches of training data are sampled) throughout stochastic gradient descent. A verifier can then validate this proof to confirm that the model owner indeed trained the model, and that the training procedure was correct. We observe then that a proof of unlearning\nj{maybe define this term} would simply amount to a proof of learning without a datapoint, and that the true discrepancy which we have been approximating is in fact the verification error associated with this proof of unlearning. We, therefore, illustrate how our framework fits in practice when tasked with providing a proof of unlearning.

%instead develop the concept of logging to facilitate a proof-of-\textbf{un}learning: our model owner would like to prove to the end user (or an auditor) that they have indeed unlearned a training point by sharing intermediate states of their gradient descent. When combined with our new Hessian regularizer, proof-of-unlearning is a step forward making unlearning more practical for ML practitioners. 

To summarize, our contributions are the following: \nj{you could uncomment the following line to remove the vertical spacing between the bullet points}
\begin{itemize}
% \itemsep0em
    \item We propose a novel metric to quantify the  error of unlearning for models originally trained with stochastic gradient descent. 
    \item We show that our unlearning error allows us to evaluate the effectiveness of gradient ascent for unlearning objectively. We also show that it is intuitive in that it is related to privacy leakage of unlearning through a subsequent analysis on probability\my{distribution, instead of probability?} shifts.
    \item We propose a new standard deviation regularizer that results in models with lower unlearning error. Our experiments show that \my{compared to what?...} it decreases unlearning error by $25\%$ for certain architectures and datasets with little drop in test accuracy, and significantly more when allowing for large drops in test accuracy.\my{I do not think you need the next sentence in contributions} We leave it to future work to further tune this and propose better losses to minimize unlearning error.
    \item We show that this standard deviation regularizer breaks the PRS attack proposed by Song et al \cite{song2021systematic}.
    \item Lastly, we illustrate a scenario for how our framework could be used in practice when faced with the verifier from Jia et al \cite{jia2021proof}.
\end{itemize}

%\anvith{@gabriel just a future note we have to fill in the x above after writing the experiments section}

%\anvith{also will be interesting discussion for what we should call this loss function, we have to give it a cooler name than just hessian regularizer, especially when it seemingly regularizes the weights more and in a way that's better than l2 regularization, but also not a big deal}

%\varun{in the intro, the flow should be as follows: (a) define the problem of unlearning, (b) taxonimize prior work into (i) exact unlearning, and (ii) approximate unlearning, (c) discuss pros and cons of each of the 2 approaches of unlearning. by now, you'd have established that there are various {\em methods} to perform unlearning. (d) now you must establish how there are multiple {\em metrics} to measure unlearning success and how it is hard for the common person to compare between the two, (e) establish that the primary contribution of this work is proposing a new {\em metric} that somehow manages to unify all previous metrics + supercede it, (f) establish a new {\em method} based on the modification to the loss function that is custom designed for the specific metric you are proposing in (e), (g) explain that to provide more intuition on whether your method and metric capture the effect of unlearning accurately, you test the approach with {\em white box membership inference} to establish if there's a correlation b/w unlearning and MI, (h) then you can draw connections b/w this work and the PoL work, (i) finally summarize some results of the evaluation}

%\anvith{I think this is obsolete, or will need to be changed to focus on something else as I think it's just a more wordy abstract, but I guess maybe that's what an introduction is}

%The motivation for this work is two-fold. The recent work done on proof of learning in \cite{jia2021proof} has an immediate consequence for a "proof of unlearning", given by a proof of learning without a datapoint. This formalized structure then naturally encompasses several ideas proposed in the growing body of literature around machine unlearning for neural networks, and will possibly lead to a more aligned body of literature moving forward as the problem is formalized, particularly, as the metric used for unlearning is formalized (the verification error associated with proof of learning); it has been a growing question whether the common use of membership inference is justified, considering the precision with the method is rather low (citation) and hasn't been justifiably linked to the notion of unlearning (citation?).

%In particular, in our work we show that the form of unlearning that is of interest for much of the literature on the topic, that of a form of approximate unlearning, is immediately related to the problem of understanding what the downstream impact of training on a particular datapoint is on the final weights, as that is what is associated with the verification error for a proof of learning; unlearning then becomes simply a problem of changing the final state of the model to fit a proof which doesn't use a certain data point.

%We propose several methods to minimize the associated error, and describe the error associated with each strategy. Though what is an acceptable error is left for legal entities to decide (as acceptable here is the same as acceptable for a proof of learning, or possibly with some greater lee-way) but as less is better for verification, we focus on the task of decreasing the error and not meeting a specific threshold, though that goal may change once thresholds are defined.

%In short, we believe that this work makes unlearning a well-defined feasible process for entities to enact and enforce, and for the community around the topic to study in a manner such that different methods can be directly compared.

%Upon reaching a closed-form approximation for SGD, we apply this to the problem of unlearning to understand how effective various approaches are at forgetting the impact of a data point on the trained model. In essence we provide a way to assess error in unlearning.

%Though our motivation is on the topic of machine unlearning, we expect the decomposition's we provide to be useful in understanding general questions relating data position and their effect on learning, and we provide some interesting mathematical insights.


==> Contents/Unused/2_background.tex <==
\section{Background \& Notation}

%\varun{missing; need this section to establish the notation that's going to be used throughout the paper; also need to discuss prior work}

\varun{i would split this into 2 sections; background is quite detailed (but can be better presented) + notation can be a separate section. it would help if you can discuss the various sources of randomness involved in training as it better motivates why unlearning is hard.}

\subsection{Introduction to Deep Learning}
\label{sec:intro_dl}

%\varun{1. write shorter sentences; 2. use $\mathbf{x}$ to denote a vector/tensor i.e. bold-faced notation denotes vectors/tensors (like data), and the regular $y$ to denote a scalar label}

%Here we quickly run through the basic ingredients for deep learning, and introduce the notation we will use throughout the paper. 

We consider a dataset \dataset which consists of pairs $\{(\mathbf{x}_i,y_i)_{i \in [N]}\}$, where $\mathbf{x}$ is a datapoint (e.g., an image) and $y$ is its label. We wish to train a model M, which is a parameterized function of weights \weights that we can modify (or learn). To learn the weights, we use a loss function $\mathcal{L}$ that measures the error of our model (in predicting the labels $y$ from inputs $\mathbf{x}$); examples of such loss functions include cross-entropy loss~\cite{cox1958regression} and hinge loss~\cite{cortes1995support}. The weights are learnt in an iterative manner using optimization schemes such as mini-batch stochastic gradient descent (SGD)~\cite{kiefer1952stochastic}. Formally speaking, mini-batch SGD works as follows:

\begin{equation*}
\weights_{t+1} = \weights_t - \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_t,\hat{\mathbf{x}}_t}
\end{equation*}

where weights at step $t$ are obtained using the weights from step $t-1$, $\hat{\mathbf{x}}_t$ is the mini-batch of data used at step $t$, and $\eta$ denotes the learning rate hyperparameter.

%which computes the average loss on a mini-batch of data $\mathbf{x}$ and then changes the weights in the direction of greatest descent (i.e in the negative direction of the gradient of the loss with respect to the current weights)

% \varun{explain mini-batch SGD as you're going to be using it a lot, or provide a forward reference to it if it is defined later in the paper} 
% \anvith{added brief explanation}. At times we will use $\weights_t$ to refer specifically to the weights after $t$ training updates, and $\mathbf{x_t}$ to the mini-batch of data used for the $t^{th}$ training update when using mini-batch gradient descent. 

% \varun{this is confusing as you've defined a dataset to be pairs of $(\mathbf{x},y)$ implying that each $\mathbf{x}$ is a single datapoint; why would $x_t$ denote a mini-batch of data? alternatively, you could define $\hat{x}_t$ as a mini-batch of data} 
% \anvith{from explanation of mini-batch I explained for training we take min-batches, and so I changed here to be specifically referrring to the mini-batch used in the t'th update with mini-batch gradiet descent}

% \varun{avoid short forms like we'll; use "we will/shall" instead}

%This generic setup is what we will consider throughout the paper, with a focus on classification tasks and the typical datasets and models associated with that.

\subsection{Introduction to Unlearning}
\label{sec:overview_unlearning}

We begin by discussing the semantics behind unlearning (\S~\ref{sec:define_unlearning}), and proceed to discuss metrics to measure the efficacy of unlearning (\S~\ref{sec:unlearning_metrics}) and methods to achieve them (\S~\ref{sec:unlearning_methods}).

\subsubsection{Defining Unlearning}
\label{sec:define_unlearning}

% in this dataset, or more generally a sample of datapoints $\mathbf{\mathbf{x}^*}$ \varun{again, notational confusion. why $\mathbf{x}^*$? can't simply $\mathbf{x}$ suffice?}
% \anvith{I refer to the unlearning data really often so I was thinking in the later presentation it helps to disinguish the unlearning datapoints from the regular datapoints}, and make the according change to our model; what this represents is the responsibility of an entity to uphold an individual's (in the case when data is personal) right to be forgotten from a corporation's dataset, and thus an entity must modify their model to meet this change.

% , and this is what we will call \textit{naive retraining}. \varun{\textit{emphasize} instead of using quotes} 
% \anvith{thanks, changed}

Unlearning is the mechanism of \textit{forgetting} a datapoint $\mathbf{x}^*$ from a trained model $M$. The task now is to define how this forgetting occurs. The naive approach to unlearning is to simply train another model $M'$ from scratch on $D'= D \textbackslash \mathbf{x}^*$. However the issue with \textit{naive retraining}~\cite{bourtoule2019machine} is the large computational overhead associated with them, i.e retraining, especially for increasingly popular large models, like GPT-3~\cite{brown2020language}. 
% \anvith{any good references to the costs related to big model like GPT-3}, and so an entity stands to expend valuabe computational resources \varun{expend valuable computational resources} \anvith{changed} if they're required to retrain every time and unlearning request is sent to them. 
%In this vain, there is a need for a computationally-efficient manner to unlearn, which naive retraining doesn't provide; this is the motivation for many 
\textit{Approximate unlearning} methods~\cite{} \anvith{think shouldn't have citation here as we're coining the phrase, and example will be cited later} (i.e., methods that do not perform retraining) try to alleviate these cost-related concerns by not requiring retraining, but rather some computationally less expensive operation on the final weights, for example a scrubbing procedure \cite{golatkar2020eternal}. 

%\varun{unclear what you're hoping to communicate with this last sentence; are you going to propose a new measure of cost?} 
% \anvith{yep agreed it was a bit vague, I've changed it to state this is the motivation for approximate unlearning methods, which perhaps is a restatement of the introduction? I think it's needed to flow into the next paragraph and basic classification of approaches. Opinions?}

% We can broadly classify the various approximate unlearning approaches. To do this it helps to work in reference to what we know is a truly unlearned model, the naively retrained model $M'$ as defined earlier. Relative to the ideal unlearned model $M'$, we can define two approaches to defining whether another model $M''$ obtained through some approximate unlearning process from the original model $M$ has truly unlearned a datapoint $\mathbf{x}^*$, alongside the original definition of unlearning in terms of retraining (which we will stop calling naive as various approaches are more sophisticated despite still being retraining):

% \varun{what is the difference b/w $M'$ and $M''$? $M'$ is obtained through retraining, and $M''$ is obtained using some other mechanism? ; why these 3 below?} 
% \anvith{yes to the first (I added an extra word to emphasize $M''$ is from some approximate unlearning process, and the below are how we can define whether $M''$ has unlearned, I'm going to drop the old third one and replace it with the baseline retraining}

%\anvith{so we actually don't give any examples or have any discussion for this third definition, so I think it's a bit useless defining this here, I think it makes more sense, considering SISA, to make the third definition "general retraining methods to provide $M'$"}

%The vast majority of the literature on this topic of unlearning for deep neural networks fall into considering one of these three categories, where the focus on third definition of retraining is to make obtaining $M'$ cheaper. 

\noindent{\bf A Taxonomy of Approximate Unlearning Approaches:} Broadly speaking approximate unlearning tries to make the approximately unlearned model $M''$ and the naively retrained model $M'$ as similar as possible, and here similarity between models broadly falls into two categories :(a) the weights of $M'$ and $M''$ (or distribution of weights) are similar, (b) the distribution of outputs generated by $M'$ and $M''$ are similar (refer \S~\ref{sec:unlearning_metrics}).

However, models are defined by the data they are trained on, and their final weights. For this reason, we will focus on the first definition of approximate unlearning in our work, and understanding the impact $\mathbf{x}^*$ has on the final weights; forgetting/minimizing this will be the bulk or our contributions.


% Keeping these broad approaches in mind, what follows are metrics and approaches that we categorize as being one of these. 

% \varun{now that we've established these 3 categories, what next?}
% \anvith{just added a sentence setting up the next bit, this was mainly just to introduce the broad definitions to keep in mind as we won't be particularly interested in (b) for reasons described in the next paragraph}.

%and (c) we simply obtain $M'$ from retraining where similarity is measured using a distance metric (refer \S~\ref{sec:unlearning_metrics}). \varun{now that we've established these 3 categories, what next?}

% \varun{i don't understand category 3} 
% \anvith{yeah the third actually does make any sense under approximte unlearning, I originaly had it as basically the three forms of unlearning, but I like this better, it's less redundant; I've commented mention of the 3rd option out} 

% Ideally all three of these categories would be equivalent, but it's clear that two models can have more or less very similar outputs but not be very similar in weights, which is the case when training high accuracy models, where as the opposite direction is more or less true (as having the same weights means the same outputs), though depending on the various local properties around a neighbourhood of the weights of $M'$, the relation may not be perfectly monotonic. The point here is that the first two definitions aren't interchangeable. 
% \varun{on reading this paragraph, i am missing the crux of the discussion. what do you wish to convey?}



%\anvith{below discussion is perhaps a bit too early, I restate this at the beginning of the sgd section so I don't think we need to state this here}

\subsubsection{Unlearning Metrics} 
\label{sec:unlearning_metrics}

We provide an overview of the main techniques used to measure \textit{similarity} between $M'$ and $M''$ (in the first two definitions provided in \S~\ref{sec:define_unlearning}). 

%we emphasize this now as one of the contributions of our work will be an analysis of what similarity means and how we can quantify it. 

\vspace{1mm}
\noindent{\bf 1. $\ell_2$ Distance:} For definition (a), a simple metric is the $\ell_2$ distance between the weights of $M'$ and $M''$. However, this first requires computing $M'$ (through naive retraining), which is expensive. Another issue is that it has widely been seen that one can retrain on the same sequence of data from the same initialization and obtain different terminal weights~\cite{jia2021proof} (which is caused by the build up of slight hardware randomnesses); if $M'$ changes each time it is recomputed, it is difficult to use \textit{any} computed $M'$ as a baseline to compute $\ell_2$ distances with respect to. One solution to this issue is to simply look at smaller retraining intervals, i.e 1 or 2 epochs so that $M'$ doesn't change much, or look at an average, or focus on correlations with proxy metrics (such as what we propose in \S~\ref{sec:approximation})

% \anvith{just us as far as I'm aware}). 
% \varun{how?} 
% \anvith{commented out, main way is to shift away from $\ell_2$ and look at probability distribution similarity, which is the following}


% but other work have found other ways to work with definition (a), such as the following. \varun{how?} \anvith{reworded, main way is to shift away from $\ell_2$ and look at probability distribution similarity, like the following}

%\anvith{I changed it to be more concrete what exactly the issue is, is it better?}

%So in general one cannot simply blindly compare the $\ell_2$ distance between the weights of $M'$ and $M''$; this will be an issue we address, but let's move on for now.

%and in fact using it to some degree (by acknowledging training is stochastic, though perhaps in additional ways to just random batching), 

\vspace{1mm}
\noindent{\bf 2. KL Divergence:} Bypassing the issue of hardware randomness in training as mentioned above, Golatkar et al.~\cite{golatkar2020eternal} consider measuring the similarity of the weights of $M''$ with respect to a distribution of weights of $M'$, and do this by looking at Kullback-Leiber (KL) divergence of the two distributions (as they consider $M''$ as being the result of another stochastic process on the original model $M$).

%\varun{is the first metric the 2 norm b/w the weights? if so, state that upfront, maybe in bold?}
%\anvith{yes, changed}

% \varun{grammar incorrect} 
% \anvith{omitted that section because I think it wasn't particularly relevant}

\vspace{1mm}
\noindent{\bf 3. Membership Inference (MI):} For definition (b), a standard method used to measure similarity in the outputs between $M'$ and $M''$ is by comparing the MI prediction for $\mathbf{x}^*$ on $M'$. This approach is used by Graves et al.~\cite{graves2020amnesiac} and Baumhauer et al.~\cite{baumhauer2020machine}. The reasoning here is that as $M'$ was properly retrained without $\mathbf{x}^*$, a MI attack (MIA) should return that it was not trained with $\mathbf{x}^*$; if a MIA on $M''$ also consistently outputs that $M''$ was not trained with $\mathbf{x}^*$, then we could say their outputs are similar (in the sense that their output on $\mathbf{x}^*$ are similar enough that the MIA believe $M''$ has not been trained on $\mathbf{x}^*$). However, such approaches are not \textit{precise}: it is possible a MIA will give a false positive that $M'$ had indeed trained on $\mathbf{x}^*$, in which case simply lowering the MI likelihood of $\mathbf{x}^*$ for $M''$ does not necessarily make it resemble $M'$. 

% \varun{what if there are many points that are (a) exactly equal to $\mathbf{x}^*$ or (b) the value of $\mathbf{x}^*$ can be inferred from other points because of correlations in the dataset?} 
% \anvith{added discussion on it, is it better?}

\anvith{for the following, I've realized it also fall under definition (a) as the DP like gurantees they give is in terms of the final model returned after training, i.e in the weight space, so I've actually changed this to be about definition (a) and (b) and commented the old version out; opinions?}

\vspace{1mm}
\noindent{\bf 4. Privacy Leakage:} For definition (a), another common metric for measuring similarity is in terms of privacy leakage: clearly $M'$ leaks no information about $\mathbf{x}^*$ as it was not trained on it, and so the smaller the privacy leakage of $M''$ in terms of its weights (specifically for $\mathbf{x}^*$), the closer $M''$ is to being unlearned; so here similarity between weights is measured in terms of of how little the privacy leakage (however privacy leakage is defined) of $x*$ is from $M''$ when looking at the weights. This sort of reasoning about privacy leakage is commonly presented in terms of differential private learning~\cite{abadi2016deep} through the calculation of the privacy parameter $\varepsilon$, but also in the work of Sekhari et al.~\cite{sekhari2021remember} and Guo et al.~\cite{guo2019certified}.


% \varun{you want to say auditing privacy (or obtaining the privacy parameter $\epsilon$); differential privacy is a general mechanism right?} 
% \anvith{yes you're right, changed the statement to be about privacy leakage, which is what Nicolas referred to in the introduction, is it better?}

\subsubsection{Unlearning Methods}
\label{sec:unlearning_methods}

We turn our attention to the following question: \textit{how exactly does one unlearn}? What follows are some examples.

\vspace{1mm}
\noindent{\bf 1. SISA Training:} The SISA framework by Bourtoule et al.~\cite{bourtoule2019machine} works by partitioning the data between different smaller models so that one never has to truly retrain the entire model; only a smaller model is impacted by a request to unlearn a datapoint. This is an example of naive retraining, where the authors still perform retraining to obtain $M'$ from $D'$, but in a cost effective manner.

\vspace{1mm}
\noindent{\bf 2. Scrubbing:} The scrubbing procedure by Golatkar et al.~\cite{golatkar2020eternal} is an example of definition (a) of approximate unlearning. Here, the authors provide a stochastic method applied to a given $M$ to output a model $M''$ whose weights are in the distribution of the ideal retrained model $M'$, which they accomplished by minimizing a "forgetting Lagrangian" which introduced a weighted term measuring the KL-divergence of the the distribution outputted by this stochastic method and $M'$. 

% \varun{you want to give a little bit more info on the method; look at the explanation for sisa} 
% \anvith{added a bit more}

%the metric they use to measure the discrepancy in the distributions of weights is KL-divergence, as discussed in the previous section. 

% \varun{repetetive; you've explained this before.} \anvith{yep, I commented it out and am just leaving the statement of what they do, before we were talking about how they measure the effectiveness of what they do}

\vspace{1mm}
\noindent{\bf 3. Amnesiac Unlearning:} Amnesiac unlearning~\cite{graves2020amnesiac} works by removing training updates that use $\mathbf{x}^*$ (that is adding back all the gradient updates with $x*$ during training) to obtain an unlearnt model $M''$. As a preface, this is quite different from what we'll propose, as all we need is to compute a single gradient update with respect to the initial weights (and train on a specific loss function to get good results) and don't need to store anything but the initial weights, as compared to storing all the updates with amnesiac unlearning. However the idea of adding back gradients (though different gradients in our case) is similar.

% In their work, they measure the effectiveness of this procedure by following definition (b), by comparing the outputs of MIA on $M''$, however, with the work we will do, we see we can also analyze the effectiveness of this method in terms of the first definition of unlearning. 
% \varun{do they add training updates or remove them?} 
% \anvith{yeah sorry, I was thinking about how you add back gradients, but it's more correct to just say they remove the training updates}

\vspace{1mm}
\noindent{\bf 4. Differentially Private Learning} \varun{what category is this? approximate? if so, which definition?} \anvith{added} Lastly, DP naturally allows one to approximately forget a data point by doing nothing as it gives bounds on how indistinguishable a given model is to one not trained on a data point (so is an approximate unlearning method under definition (a) as we look at the distribution of final models in the weight space). However Sekhari et al.~\cite{sekhari2021remember} show that DP learning only allows one to delete $O(\frac{n}{\sqrt{d}})$ data points while retaining meaningful bounds, and propose an unlearning algorithm for convex and strongly convex losses that improves the number of datapoints one can delete by adding a hessian update and noise to the final weights. 



% \varun{more details on how this is achieved} \anvith{added}



%focus on unlearning also by the second definition, however here the focus is how differential private learning (or the adapted version they propose) allows one to delete $\mathbf{x}^*$ (or more generally a number of data points less than some maximum number of delete requests) without needing to do anything under the guarantees of differential privacy. 

% \varun{could you please expand upon the last sentence? also this seems like it was explained earlier ... }
% \anvith{yep agreed again, I just changed to get to the point and say what they're doing at a high level}


\anvith{as of now doesn't look like we'll do this}
\subsubsection{The Pros and Cons/A Comparison}

%\anvith{feel free to give this section a better title}

%\anvith{I'll leave this for Gabriel, feel free to also add more methods to the anlysis, I just felt I should stop at one I explained above just because I felt it was a good survey and showcasing more would be for diminishing returns}









 







==> Contents/Unused/3_SGDaprox.tex <==
%As briefly discussed in the background, the question we need to ask when trying to define unlearning is what is it that we're truly interested in forgetting; do we simply want a model to be similar in outputs to a model that hadn't trained on the point we want to forget, or be similar in weights? Fundamentally, the question underlying what we define as unlearning is what is the 

%there is inherently no wrong answer, as entities may require different things by what they mean by unlearning, however as discussed there is seemingly a slight hierarchy to the definitions. 
% \varun{be precise! }
% \anvith{dropped the latter half of the above paragraph, and just going straight to the next paragraph, which is a bit more precise now, right?}




%It follows then that by understanding the impact $\mathbf{x}^*$ has on these updates, we might be able to understand what it is we have to do to unlearn, and perhaps understand bounds on how much we can truly unlearn. That will be the outcome of this section.

% \varun{not clear what you're trying to convey in the previous 2 paragraphs; do you want to say that unlearning implies that there should be some reversal in terms of the weights learned during training? if so - just state that and provide motivation. }
% \anvith{yeah I dropped the second paragraph you were referring to, and keeping the first to set up the following paragraph where I added a a slight change to say "the main outcome is understanding the closed form (approximate) affect of $\mathbf{x}^*$ on the final weights of a model,.." after saying we look at SGD}

%\varun{enumerate the two terms to make it clearer}

% We understand that really what we're working with is an approximation, and so in the following section we empirically correlate our estimate (which will have a slightly different scale) and the true discrepancy between $M'$ and $M''$ which we can compute by simply retraining without $\mathbf{x}^*$ to obtain $M'$, and then taking the difference in weights with the model we obtain $M''$ and then noting we bypass the issues of randomness as we're interested in the general correlation\varun{how do you obtain said true discrepency?}\anvith{added}; we see we have a strong positive correlation, and so it follows that by minimizing our estimate we are minimizing the true discrepancy, which is beneficial as we find our analysis leads to natural ways of doing this.

% Lastly, one might reasonably ask what is difference in what we're about to do from influence functions as introduced by Koh \& Liang~\cite{koh2017understanding}, and the main difference is the results of our derivations; the method they propose is comparatively expensive to what we'll eventually propose as a method for unlearning (with our associated error), however, the idea of linearizing is central to both and in that way there are some fundamental similarities, however the differences here are more important. It is however an interesting line of future work to compare our two approaches. \varun{i think this is presented ahead of where it should be; i don't know what your method is so it's unreasonable to expect me to understand this comparison as of yet.} \anvith{yeah agreed, I just know I have to present it somewhere, let me see where I can put it: possibly after we've written up more stuff in the section where we compare different methods}

% Nevertheless, we now proceed to explain this approximation, what it says about unlearning (i.e removing the impact of $\mathbf{x}^*$ in the weight space), and the general bounds it gives.

% \subsection{Introducing the approximation}

%\anvith{Take the wording below as rough, and the main point with the stuff here rn is the math; I'll add wording to justify thoroughly why look at an approximation, and then fit the rest of the section with that context- the one thing that won't change is the math}

%What follows is essentially the standard SGD taylor approximation used in other papers for error analysis, as seen in equation 13 in \cite{smith2021origin} (though we keep a few more of the higher order terms, though not all), however we go through the steps of deriving it here for clarity and to be consistent with our notation. However the similarities with past work end with the expression for the approximation, as we then analyze it to understand the dependence on a given datapoint $\mathbf{x}^*$, and what that tells us about unlearning.

%\varun{you want to approximate $\weights_2$ such that it only relies on $\weights_0$ and nothing else.}

%Thus we wish to approximate $\eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0-\eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0},\hat{\mathbf{x}}_1}$ so that it only depends on $\weights_{0}$ and not on the previous gradient computation. 


%We can do this by using a first order taylor series approximation on the partial derivative under the assumption that $\eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0}$ is small (i.e $\ell_{\infty}<1$), which as the learning rate $\eta$ is less than 1, is a fair assumption for machine learning models; our later experiments quantifying how effective our approximation is verify our assumptions. The result is the following:

% \varun{discuss now!}
% \anvith{I added a blurb on why we are ultimately justified in doing this, but I actually think this discussion is obsolete as we are anyways going to present why this approximation is correct, so I've commented it out as it seems more like a digression right now}.



\section{A Closed Form Approximation of SGD}
\label{sec:A Closed Form Approximation of SGD}

As noted earlier, there is a tension associated with defining what it means to truly unlearn: does it require similarity between the distribution of weights (definition (a)) or the distribution of outputs (definition (b))? However, note that what is common to both is understanding the effect of a datapoint $\mathbf{x}^*$ on a model trained on it. The effect of $\mathbf{x}^*$ is viewed through its influence on the sequence of training updates, which in turn changes the weights learned. Thus, the change in outputs can be viewed as a byproduct of the change in weights.

Keeping this in mind, what follows is an approximation of the outcome of SGD using a Taylor series, and a subsequent analysis of the approximation. The main outcome is an understanding of the \textit{closed form} (approximate) effect of $\mathbf{x}^*$ on the final weights of a model. 

%In particular, we obtain a decomposition of SGD into (a) terms one can seemingly forget \textit{cheaply}, and (b) terms that would require at least as much computation to forget as training. Unlearning is possible by simply removing (a subset of) these terms from the final weights. Note that from these \textit{expensive} terms (category (b)), we can estimate an \textit{unlearning error} which represents the distance in the weight space between the naively retrained $M'$ and the model $M''$ we get by unlearning as above. The remainder of this paper is centered around how one can reduce the unlearning error. 

\subsection{Expanding SGD} 

We begin with the definition of a single SGD learning update:

% \varun{use $\mathbf{w}$ for weights}
% \anvith{changed so macro \weights is boldface, using that}

\begin{equation}
\label{eq1:}
\weights_{1} = \weights_0 - \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0}
\end{equation}

where $\mathbf{w}_0$ denotes the weights at step 0, and $\hat{\mathbf{x}}_0$ denotes the mini-batch of data sampled at step 0. We obtain $\weights_{2}$ as follows:

\begin{equation*}
\weights_{2} = \weights_0 - \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0} - \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_1,\hat{\mathbf{x}}_1}
\end{equation*}

\begin{equation}
\implies \weights_{2} = \weights_0 - \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0} - \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0-\eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0},\hat{\mathbf{x}}_1}
\end{equation}


This can further be expanded and approximated as follows:

\begin{equation}
\weights_{2} \approx \weights_0 - \eta (\frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0} + \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_1} + \frac{\partial^2 \mathcal{L}}{\partial^2 \weights}|_{\weights_0,\hat{\mathbf{x}}_1} (- \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0}))
\end{equation}

Our end goal is obtaining a closed form that explicitly only depends on the initial weights $\mathbf{w}_0$ and sequence of mini-batches of data. To scale the above for a sequence of $t$ updates, notice that the hessian terms from the expansion recursively depend on each other. Thus we have the final approximation:

\begin{equation}
\weights_{t} \approx \weights_0 - \eta \sum_{i=0}^{t-1} \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_i} + \sum_{i=1}^{t-1} f(i) \label{eq:approx}
\end{equation}

where $f(i)$ is defined recursively as:
\begin{equation}
\label{eq: recursivedef}
f(i) = -\eta \frac{\partial^2 \mathcal{L}}{\partial^2 \weights}|_{\weights_0,\hat{\mathbf{x}}_i} (- \eta \sum_{j=0}^{i-1} \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_j} + \sum_{j=0}^{i-1} f(j))
\end{equation}

with $f(0) = 0$.

% \subsection{Understanding The Approximation}
% \label{sec:approximation}

% \varun{equation broken}
% \anvith{yeah I'm blind and didn't realize I already had a label for the equation, which I put at the end}

\paragraph{Understanding The Approximation:} From Equation~\ref{eq:approx}, observe that one can represent the weights obtained after training $t$ updates as the sum of two sums. We now wish to understand how $\mathbf{x}^*$ affects this expression (and thus the approximate outcome of training). The terms in the \textit{first sum} are simply gradients taken with respect to the initial weights $\weights_0$ and a mini-batch $\mathbf{\hat{\mathbf{x}}_i}$ following the order we give data to the model. Notice, however, that the exact order does not matter as we are simply adding them. In this case, it is clear that the effect of $\mathbf{x}^*$ (provided at any step in training) on this first sum is a gradient (or gradients) computed with respect to $\weights_0$ and $\mathbf{x}^*$. To reverse this effect, we simply have to \textit{add back these gradients} (times the learning rate $\eta$ and $\frac{1}{b}$ where $b$ is the batch size)\footnote{Note that gradients on mini-batches are just a sum of the individual gradients on each datapoint averaged, so in fact we can single out the gradients from just $\mathbf{x}^*$ which are multiplied by $\frac{1}{b}$ from averaging.}.  This process is computationally inexpensive. 
% , as it amount to simply adding $\frac{\eta m}{b} \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0}$, where here $m$ is the number of times $\mathbf{x}^*$ appear in a mini-batch during training (i.e the cost is a single gradient computation). 

% \varun{well, you have to store all of these updates ... }
% \anvith{no we don't, we just need the initial weights and the datapoint; I added a bit more detail to make this clearer, it amounts to a single gradient computation}

The \textit{second sum} is more complex, as the expression is recursive, and there is an inherent dependence on order. To compute all the terms that contain a particular $\mathbf{x}^*$, one would require at least as much computation as training; this term behaves as an upper-bound on how well we can cheaply unlearn. In \S~\ref{sec:approximation}, we describe how one can estimate the magnitude of this term, which we call our \textit{unlearning error}--this term captures the true discrepancy we expect between perfectly removing the effect of $\mathbf{x}^*$ on our model, i.e. perfectly retraining to obtain $M'$, and what we can cheaply do by removing the effect of $\mathbf{x}^*$ on the first sum i.e., our $M''$. Note the method to remove the effect of $x^*$ in the first sum is our unlearning method, which we'll later couple with a regularizer on the loss function to improve its effectiveness (i.e minimizes our unlearning error).


%The first important detail to note is that the first sum is commutative with respect to the indices; that is, any permutation of $\hat{\mathbf{x}}_{i}$ results in the same value. Thus, we will continue call this the order independent part.

%The recursive component is not invariant to permutations, and so we will call it the order dependent part.

%Though we leave it to later sections to further elaborate, the error we're interested between $w'_t$ and $\weights_t$ is approximated by the magnitude of the order dependent part averaged over the size of the dataset, i.e the contribution of a given datapoint to that term; this is simply as the modified state $f'$ we can feasibly achieve undoes the effect of a given $x*$ on the first part, but not the second, and thus the approximate associated error is the contribution of $x*$ to the second term.

%\subsection{Understanding Order Independent Component}

%There is not much to say now other than this introduces an ideal scenario in order to remove updates, i.e unlearn. This is also analogous to the update rule in distributed learning and batch SGD.

\subsection{Approximating the Second Sum Series}
\label{sec:approximation}

The global structure of the second sum follows $\eta^2 c_{t} + \eta^3 c_{t-1} + ... +\eta^{2+t-1} c_{1}$, where $c_{i}$ represent a vector. Thus, we can focus primarily on the $\eta^2$ dependent term as $\eta$ is almost always a magnitude or more less than $1$ and so $\eta^2$ is the dominate term (in the case it's not less than 1 focusing on $\eta^2$ will be wrong in the sense that we're ignoring other more dominant terms). Thus, the second sum can be rewritten as:

\begin{equation}
\label{eq:error}
\eta^2 c_{t} = \sum_{i=1}^{t-1} \eta^{2} \frac{\partial^2 \mathcal{L}}{\partial^2 \weights}|_{\weights_0,\hat{\mathbf{x}}_i}  \sum_{j=0}^{i-1} \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_j} 
\end{equation}

We can further approximate $\sum_{j=0}^{i-1} \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_j}$ by its expectation $\frac{i(\weights_{t}-\weights_{0})}{t}$. We further normalize the vector, and thus have:

\begin{equation}
\label{eq: Detailed_Aprox}
\eta^2 c_{t} \approx \eta^{2} \frac{||\weights_{t}-\weights_{0}||_{2}}{t} \sum_{i=1}^{t-1} \frac{\partial^2 \mathcal{L}}{\partial^2 \weights}|_{\weights_0,\hat{\mathbf{x}}_i} \frac{\weights_{t}-\weights_{0}}{||\weights_{t}-\weights_{0}||_{2}} i
\end{equation}


% \varun{what does $||.||$ denote?}
% \anvith{l2-norm, I'm going to add it as a subscript}

By focusing on $||c_{t}||_{2}$, note that 

$$||\frac{\partial^2 \mathcal{L}}{\partial^2 \textbf{w}}|_{\textbf{w}_0,\hat{\mathbf{x}}_i} \frac{\textbf{w}_{t}-\textbf{w}_{0}}{||\textbf{w}_{t}-\textbf{w}_{0}||_{2}}||_{2} \leq ||\frac{\partial^2 \mathcal{L}}{\partial^2 \textbf{w}}|_{\textbf{w}_0,\hat{\mathbf{x}}_i}||_{2}$$ 

by definition of the induced $\ell_{2}$ norm, which is simply the square root of the largest eigenvalue of the hessian , i.e., $\sigma_{1,i}$ the first singular value of the hessian on $\hat{\mathbf{x}}_{i}$. For sake of simplicity we consider $\sigma = \max(\sigma_{1,i})$, and thus have:

\begin{equation}
||\eta^{2} c_{t}||_{2} \leq \eta^{2} \frac{||\weights_{t}-\weights_{0}||_{2}}{t} \sigma \frac{t^{2} - t}{2} \label{eq:error bound}
\end{equation}

Thus, we can observe that the second sum linearly depends on $||\weights_{t}-\weights_{0}||_{2}$, $\sigma$, and $t$. $\sigma$ captures the non-linearity of the loss landscape from the hessian, and thus we see that the more linear the loss landscape, the lower the value. We also see from this that in the scenario $t=1$ or $\sigma = 0$, this bound, and thus the term, is 0.  

%this insights motivate what we later do in trying to reduce this.

%Though this bound is nice for the intuitive picture of what is going on, it can be a rather loose bound to work with as we took $\sigma = max(\sigma_{1,i})$, so for our later experiments we will stick to approximating \ref{eq: Detailed_Aprox} by taking the average singular values over epochs.

% \varun{what is the takeaway from this explanation?}
% \anvith{mainly to have a nice equation that gives an intuituve understanding of what is goinf on, it's also what gives the insights into what we later try to reduce it (added a brief blurb at the end of the second last paragraph on that point)}

%\todo{np: this is cool for intuition. you should illustrate the intuition we discussed on our call for each of the terms of the bound on a linear model where you know that everything will hold exactly. you could also consider a deep linear network (look up on internet there is long line of work started by andrew saxe) to make things more interesting with non-linear learning dynamics}

%\anvith{That sounds interesting, I'm taking a look into it. What's actually weird is that the non-linearity of the loss, i.e value of the hessian, is actually dominated by the contribution from the final softmax (see equation 10 and the discussion above it from "Emergent properties of the local geometry of neural loss landscapes"), but I guess those deep linear networks wouldn't have a softmax (or at least those that don't are the ones we'd look at to see extremely low to no error)}

%Perhaps most importantly, this quantity is seemingly the same units as the loss, as we expect $||\weights_{t}-\weights_{0}|| \propto t$, and units of $\sigma$ are $\frac{loss}{w^2} = \frac{loss}{t^2}$, thus all together we have  $\frac{loss * t^3}{t^3} = loss$. This helps justify the universality of our $d(A,A')$ if indeed the loss is a universal metric (i.e comparable between models and datasets).

%However in general we expect $||\weights_{t}-\weights_{0}|| \propto t$, and so we expect a quadratic growth with $t$ (or at least a faster growth than simply linear) but interestingly, experimentally we found that the error grows linearly with t, suggesting that $||\weights_{t}-\weights_{0}||* \sigma = constant$.


%\subsection{Noteworthy Properties}
%So far in our analysis we have set $\weights_{0}$ and $\weights_{t}$ to be arbitrary, though perhaps implied that they are the starting and end point in training. In general we can consider any $\weights_{0}$ and $\weights_{n}$, and split this further into smaller arbitrary intervals $\weights_{0},\weights_{t},\weights_{2t}, ... \weights_{n}$. Thus we see that we can simply approximate any $\weights_{i*t}$ with respect to $\weights_{(i-1)t}$ rather than needing to approximate $\weights_{n}$ with respect to $\weights_{0}$. We emphasize this now as this will be particularly relevant in our analysis of amnesiac unlearning and how pretraining is beneficial.


\paragraph{Counting Terms:} Now, with an understanding of what the dominant terms in the second sum of Equation~\ref{eq:approx} are, we can understand the computational costs needed to forget higher order terms, besides simply the first sum of Equation~\ref{eq:approx}. To do so we now focus on the expression in Equation~\ref{eq:error}, and letting $i^*$ denote the first index where $\mathbf{x}^*$ appears in a mini-batch, we are interested in what terms would contain $\hat{\mathbf{x}}_{i^*}$ and thus $\mathbf{x}^*$, i.e., what terms would we need to remove in order to forget $\hat{\mathbf{x}}_{i^*}$ from the dominant term in our second sum in Equation~\ref{eq:approx}.

% \varun{not $\mathbf{x}^*$?} 
% \anvith{completely forgot to say $i^*$ is the first index $\mathbf{x}^*$ appears in, added it, so hopefully clear now?}.


\varun{can you re-word the paragraph below? it's quite convoluted to read} \anvith{made some changes (removed some redundancies) is it better?}
First thing to note is that $\hat{\mathbf{x}}_i^*$ does not appear in any terms in the expression until $i= i^*$; for this index we see we have $i^*$ terms dependent on $\hat{\mathbf{x}}_{i^*}$ as every term in the second sum in eq \ref{eq:error} is multiplied by $\frac{\partial^2 \mathcal{L}}{\partial^2 \weights}|_{\weights_0,\hat{\mathbf{x}}_{i^*}}$. Now for all the indices $i>i^*$ (i.e $t-1-i^*$ indices), we have exactly one term with $\hat{\mathbf{x}}_{i^*}$ which comes from a $\frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_{i^*}}$ appearing in the second sum once. Lastly note that each term we see $\hat{\mathbf{x}}_{i^*}$ in is a hessian vector product, as all terms here are hessian-vector products.

So in total we have $t-1-i^*+i^* = t-1$ terms, and note that all these terms are hessian vector products (because all the terms in Equation \ref{eq:error} are hessian vector products). In general it is possible to implement hessian products in O(n) ~\cite{pearlmutter1994fast} by implementing a differential operator numerically (i.e finite differences) and so runs close to the computation required for a gradient which we would need to compute twice in order to use the method. \varun{explain this in a bit more detail, but in a line?}
\anvith{done}

%Consider that we focus on a uniform distribution over datapoints $\hat{\mathbf{x}}_i$ so that our expectation of i is $t/2$. In this case, every indexed term $j$ where $(t/2) \leq j$ will thus contain an $\hat{\mathbf{x}}_i$ in the second sum. Furthermore, the term $j=t/2$ would have $\hat{\mathbf{x}}_i$ in the hessian, meaning every term in the second sum for $i=t/2$ would have a coefficient with $\hat{\mathbf{x}}_i$. Thus on average we'd expect to compute $t$ gradients and $t/2$ hessian.


% (or well at least as expensive as computing $t-1$ of the $t$ training steps, which for all intents and purposes is practically the same)

Importantly, as these hessian vector product are at least as expensive as a gradient computation, we have that the computational requirement to compute all these terms containing $\hat{\mathbf{x}}_{i^*}$ in Equation~\ref{eq:error}, in particular just computing the $x^*$ component in these batch terms, is at least as much as computing $t$ gradient updates on a single data point (when also including the one gradient we need to compute for our unlearning method). In the case the batch size is $1$, this would be equivalent to the cost for training, and in general is $1/b$ the cost of training (where $b$ is the batch size). However this can still be a significant amount in practice (as $t$ here is not the epochs but the number of individual training steps), so we see that this second sum in Equation~\ref{eq:approx} which we can approximate with Equation~\ref{eq:error} is a bound to how well we can reasonably forget the effect of $\mathbf{x}^*$. Future work could be looking into computing all these terms and assessing the error then (by looking at the even higher order terms in the second sum of \ref{eq:aprox}).

\anvith{below is new, realized we need to properly define unlearning error}

\paragraph{Unlearning Error} Based on the above discussions for estimating the second sum, and how it bounds how well we can unlearn (without adding on significant computational costs), we define equation \ref{eq:error bound} to be our \textit{unlearning error} $e$, with the slight modification that as in practice this bound can be loose we take $\sigma$ to be the average of all the $\sigma_{1,i}$ rather than the max, as to better approximate equation \ref{eq:error} (though without having the proper inequality for \ref{eq:error bound} given by using the max). To be precise, defining $\sigma_{avg} = \frac{1}{t}\sum_{i=1}^{t} \sigma_{1,i}$, we define unlearning error as 

\begin{equation}
e = \eta^{2} \frac{||\weights_{t}-\weights_{0}||_{2}}{t} \sigma_{avg} \frac{t^{2} - t}{2} \label{eq:unl_err}
\end{equation}


Working with the average also allows to only compute $\sigma_{1,i}$ every couple of steps instead of every step, saving costs. Lastly note computing $e$ doesn't require us to have applied our unlearning method first, we can preemptively know what the unlearning error $e$ will be.


% , and so this is our measure for the discrepancy between trying to forget the effect of some $\mathbf{x}^*$ from the first sum of Equation~\ref{eq:approx} and what a truly unlearnt model (i.e $M'$ which was retrained without $\mathbf{x}^*$) achieves for its final weights.


%This means trying to properly compute all these $\hat{\mathbf{x}}_{i^*}$ terms to remove them is infeasible, or at least if you were to do so, you might as well simply properly retrain to unlearn.


% Our goal now, having a way to unlearn (albeit for only a part of our expression), is to minimize this second sum as to more effectively forget the effect of $\mathbf{x}^*$, which will be the focus for a later section. The question now is just how good our approximation of this discrepency between the ideal $M'$ and the model we obtain we obtain by removing the effect on the first sum, $M''$ is (which we'll call our "unlearning error"), which is what we discuss in the following section.

%\todo{np you should expand discussion here to say whether there are valuable uses to computing an approximation of the hessian instead}


==> Contents/Unused/3_definitions_not_used.tex <==


\section{Defining Proof of Unlearning}

%We consider the following setup based on the work done for a proof of learning \cite{jia2021proof}. 

\varun{why talk about a proof of unlearning? there's currently no motivation for why this is needed; a lot of this first paragraph is fluff that's from the PoL paper so you can refer the reader to that paper. for example, unless you are going to use the terms (W,I,H,A) somewhere -- why even define it here?}

We define a proof of unlearning in the following situation. An individual $T$ has a model $f$ trained on a dataset $D$ and now must prove to a verifer $V$ that the model (or more accurately a modified version of $f$ which we'll call $f'$) was trained on $D/x*$ where $x*$ represents a batch of data. From the recent work done on proof of learning \cite{jia2021proof}, this verifier $V$ has been well defined, and the process of proving having trained a model requires providing a proof of learning, $P$, which is the set $(W,I,H,A)$ consisting of $W$ the sequence of model states during training, $I$ the sequence of datapoints during training, $H$ the signatures of these datapoint, and $A$ the other necessaary information for reproduction such as hyperparamters. Given $P$, the verifier checks that indeed the given proof is correct by computing all (or some subset of) the gradient steps and verifying the error is "acceptable", where this error is measured as distance in the weight space from what the verifier obtains and what you claimed to have obtained.

So, building on this framework, we can say that for $f'$ to be an unlearned model, it must have an associated $P$ such that $I$ does not use $x^*$, so then the verifier $V$ can check that $f'$ did not train on $x^*$ by validating $P$. The process of obtaining such an $f'$ that has such a proof $P$ is what we call unlearning, where $f'$ is the unlearned model, the associated $P$ the proof of unlearning, and the associated verification error is the unlearning error (as lower verification error means higher confidence that $f'$ belongs to such a proof of unlearning), which we'll denote as $e$.

\varun{lower verification error implies that the proof associated with it is a {\em correct/well-formed} proof; needn't be a valid one for an unlearned model. please correct me if i am wrong}

\subsection{Categorizing Approaches to Unlearning}

\varun{why do we want this taxonomy?}

So far it would seem that in order to obtain an unlearned model $f'$ one in the process would need to also compute or obtain all the information necessary for the corresponding proof of unlearning $P$, however this may not in general be the case, i.e the act of obtaining $f'$ could be mutually exclusive of the act of obtaining the corresponding $P$. It may in fact be in an entities interest to simply obtain $f'$ and understand it's error, and not compute $P$ as doing so would add additional computational costs.

So it makes sense to make a distinction between unlearning approaches based on whether the approach produces $P$ alongside $f'$, or not.

\anvith{Does it make sense to just call it Mutually Inclusice and Mututally Exclusive and drop the old names? I think it's a more formal and justified way of talking about these things}

\begin{enumerate}
\item Mutually Inclusive Unlearning: This is where $T$ obtains a $P$ (and so also $e$) alongside $f'$
\item Mutually Exclusive Unlearning: This is where $T$ obtains $f'$ and the associated $e$ but not $P$
\end{enumerate}

\anvith{This uses the new terminology, see below commented out for what I wrote before using old terminology}

For reference, an example of mutually inclusive unlearning is retraining or SISA \cite{bourtoule2019machine}, as in those scenarios one computes (or has computed) all the training steps that lead to $f'$, and so if $T$ keeps track of the necessary information, $T$ could obtain $P$ while also obtaining $f'$. Examples of mutually exclusive unlearning will be discussed later, but the main idea is one can more often than not modify $f$ in a relatively cheap manner to achieve $f'$.

The reason we explicitly state in both cases that $T$ obtains $e$ is for the simple reason of having to know whether $f'$ is any good; it may be that $T$ actually knows what $e$ will be before obtaining $f'$, or that $T$ can obtain $e$ while obtaining $f'$. Which ever way we will not differentiate too much in this paper.

There is however one more additional scenario, where for Mutually Exclusive unlearning it might not be possible to obtain $e$ without obtaining $P$, but it is possible to obtains a reasonable approximation of $e$, which we'll denote $e_a$, in this case we have the addtional scenerio

\begin{enumerate}[resume]
    \item Approximate Mutually Exclusive Unlearning: This is where $T$ obtains $f'$ and the associated approximate error $e_a$
\end{enumerate}

This last scenario is what we'll focus on for the latter part of the paper when we consider cheap unlearning methods but then try and keep the verification error low, so though it seems sort of niche for now, we'll see it is quite useful as obtaining a closed form for $e_a$ leads to an understanding of how to lower it, and thus lower $e$.


%\anvith{following stuff uses the old terminology}

%\begin{enumerate}
%\item Proper Unlearning: This is where $T$ obtains a valid $P$ for $f'$
%\item Approximate Unlearning: This is where $T$ obtains an approximate $P$ for $f'$
%\end{enumerate}

%Where approximate means providing a valid (or close to valid) proof without having to retrain.


%For this paper we'll focus on scenario two, where because of various constraints, such as cost and time, it's in the interest of $T$ to approximate a $P$ without retraining. As thresholds for verification are yet to be determined by various entities (such as legal bodies and governments), we focus on how one can mitigate the expected error during verification, and to do this we study a taylor approximation of training, and from this provide various methods to mitigate the error for a certain proof. Furthermore, we consider the scenario where $T$ is not interested in actually creating a $P$, but in the guarantee of an approximate $P$ existing; the point here is to emphasize that actually computing a $P$ isn't necessary if one has reasonable confidence in their approximation/process (this is to further make viable options in which to compute the new $P$ would be unreasonably expensive, on par with training, but the modification necessary for $f$ to fit this new $P$ is relatively cheap).

\subsection{Context with previous approaches to Unlearning}

\varun{keep notation consistent -- $x^*$ not $X^*$; a lot of the content here can be used in the introduction }

Though there's been a plethora of recent work on the problem of unlearning, how to verify unlearning (and hence how to approach it in practice) has been up to interpretation.

As was defined in \cite{bourtoule2019machine} and much of the work following it, unlearning is achieving a model that could have been achieved by honestly training without $X*$, however the process of verifying a model has unlearned has been left upto various authors to interpret.

A prominent definition of unlearning, or at least measuring the plausibility of a model having been retrained in practice, is membership inference accuracy \cite{graves2020amnesiac}, \cite{baumhauer2020machine} . However modern membership inference are generally not reliable (as it's precision is low) and though dataset inference does improve precision, it works only on batches of data and gives little to no individual information of unlearning; this is not to say the approaches to unlearning were flawed, as we'll see amnesiac unlearning fits with the approach we provide (and we do not doubt future work will be able to reorganize other methods in the context of proofs), however the use of membership inference for evaluation is perhaps not ideal based on the current state of the art. 

The approach of membership inference for evaluation is part of a general idea of defining unlearning through the distribution of outputs between a model achieved from a unlearning approach and a properly untrained model, which is inherently not well-defined as it is plausible (though less so for completely disjoint datasets) for two models trained with and without a certain datapoint to behave similar (and conversely, due to the stochasticity in batching, for the same dataset and architecture to lead to two different models). Despite this, taking advantage of stability under removing small samples of data, \cite{golatkar2020eternal} were able to give certain gurantees, however their work was under the assumption of pretraining (an assumption we'll later show gives better proofs in our framework too). 

Another common approach to measuring/guaranteeing unlearning is differential privacy, which under the right scenarios gives gurantees for the information gained by learning on a datapoint $x*$ to be forgotten through some process, or at least having a bound on privacy leakage \cite{sekhari2021remember}. As far as we are aware, there is nothing inherently wrong in this, though perhaps more work needs to be done on how one approaches the gurantees in practice. Regardless we'll consider such privacy gurantees to be tangential to the unlearning scenario we've set up.


\begin{comment}


\section{OLD Defining Unlearning}

Before going on, it is important to give a definition of unlearning which we'll be using in our analysis. Generally speaking, the goal of machine unlearning is defined as removing the contribution of a data point to the training of the model, in essence forgetting that the data point ever existed; this is the idea behind Cao and Yang's approach. Other papers have considered a more general definition to unlearning, where they considered removing the effect of the data point on various metric spaces, for example achieving outputs similar to a model not trained on the datapoint. As we'll discuss, this is not the same as the former stricter definition. 

%\todo{np: what do you mean by effect? you might want to forward point to your discussion of input+weight+output spaces} 

A significant focus of this paper will be devoted
to considering approximate unlearning schemes; that is, not the provably robust approaches such as SISA and retraining, but those that give a relation to how close you are to such an approach. However we'll see that our analysis naturally leads to unlearning schemes that give no error, which are identical to known methods.

\anvith{the case of SISA and retraining is that of t=1 (i.e forgetting every step), which gives 0 error. }

%\todo{np: your comment above made me wonder. do we have to limit this analysis to provably robust approaches? could we include things like retraining and SISA in the framework and show that their error is 0? in other words they are a corner case of your error formulae} 

Having now defined unlearning broadly, we'll discuss why the general definition is not same as the stricter concept by illustrating the ambiguity with such metrics, where as the stricter case has a well-defined mathematical formulation.

\subsection{Issues with Unlearning Metrics}

When dealing with a neural network, your faced with essentially three metric spaces: the input space, the weight space, and the output space. The challenge now is to figure out which of these spaces (if any of them) colloquially defines the relation between learned models and unlearned models, i.e which space must we use to understand how close a model is to an unlearned model. However there are inherent flaws in simply following any arbitrary distance metric in one of those spaces, which relates to the natural stochasticity in training discussed in "Machine Unlearning". Our essential point is that these metrics have non-zero probability of being either from a learned or unlearned model, and thus capture a probabilistic state, where as the stricter definition appeals to a non-probabilistic formulation of training.

It is clear that the input space is something possibly shared between models, and does not give information specific to the model. Furthermore, as the output space is often of lower dimension than the weight space, outputs are not necessarily unique to a model; this is seen by the implicit function theorem which under certain conditions guarantees the existence of multiple solutions. As outputs are not unique, we do not have that measures on outputs necessarily relate to a measure of how well an entity has unlearned, simply because a learned model might still behave in a very similar way, and vice-versa. So we see that outputs do not necessarily capture distinct differences between unlearned and learned models.

For the weight space, it's well-know that the same training procedure from the same initial state and dataset can lead to different weights. We also cannot rebuke whether two different data sets could not lead to the same final weights. For example, consider constructing an image such that it's gradient is in the direction from the initial weights to the final weights and take the necessary learning rate to take you to the final state in one step; such an image may or may not exist, but it illustrates the problem with making the statement that positions in the weight space are unique to the dataset.

In essence the best we could do is give a probabilistic answer, which give varying degrees of gurantees (one would expect that a single datapoint would shift the distributions by a negligible amount). We avoid such issues by considering an analytical approach to unlearning, which at its heart is just accounting.

%This problem extends to the weight space, as we're now asked whether any position in the weight space is unique to a dataset, which is analogous to asking if there is only one such path to a final model state, which is not necessarily true; consider constructing an image such that it's gradient is in the direction from the initial weights to the final weights and take the necessary learning rate to take you to the final state in one step; such an image may or may not exist, but it illustrates the problem with making the statement that positions in the weight space are unique to the dataset, and thus the ambiguity in knowing whether a model has truthfully unlearned by being in such a position. \todo{np: i feel like an easier to understand argument may be to say that if you repeat multiple runs of the same training procedure on a fixed dataset, you could obtain multiple points in the weight space. this is an argument related to the definition we had in SISA of the "distribution of models" being identical after learning+unlearning than after learning without the point }

\subsection{Unlearning as Accounting}

We appeal to the work done by Cao and Yang on machine unlearning, where machine unlearning was defined by accounting for the terms in summations (representing the learned procedure) that contained the data point you want to forget; here the task of unlearning is to subtract the terms with the given data points, provably forgetting them.  \todo{this accounting terminology is very appealing. I wonder if this suggests that we could develop a similar tool to what was proposed for accounting in differential privacy. see for instance the moments accountant of abadi et al.}


In the following section we give a closed form approximation of SGD that is broken down into sums; from this we have a natural way to unlearn by removing terms with a given data point $x^*$, however it won't be possible to remove all such terms. The terms we miss gives us a measure of how effectively we've unlearned as the larger their magnitude (taken in the weight space), the stronger their effect on the final state of the model, and thus the larger the error we have in removing the effect of $x^*$ from the model. 

In essence, we define our unlearning metric absolutely in the weight space as $e = d(A,A')$ where $d(A,A')$ is the magnitude of the terms that sill contain $x^*$.

This metric is irrespective of model architecture, as we will consider lower dimensional weight spaces to be subspaces of larger dimensional weight spaces, and thus the distance metric is comparable. Intuitively what we're saying is that we do not consider any scaling to account for the size of the model or its architecture; if it is that a larger model or a particular architecture tends to have higher unlearning error, then we say it is just harder to unlearn. In other words, we assume they all have the same unit. This is simply a decision we have made for our analysis; there are cases where we consider certain scaled quantities, such as error per step, however note that such scales do not intuitively measure absolute error. For example, scaling by size would give 'error per neuron" which isn't quite the same as total error. We will later discuss how our metric relates to the probabilistic metrics discussed earlier to further justify this decision.

\anvith{we may actually want to conduct experiments to just see how the different scaled metrics relate to the more probabilistic metrics such as outputs. I'm slightly hesitant as that would essentially be appealing to the old thing we have a problem with in order to justify our new thing. However, at the same time it would be a nice (but I guess not sufficient) reinforcement to see whether our approach is merited; I think we already know, based of comparing the results we got on a rather higher error approach to that of amnesiac unlearning with relatively low error, that the error correlates to metrics such as comparing distances in outputs, but more work would be nice I guess.}

What all this means is that given two models $A$ and $B$ that we've used our unlearning approach on, and the two respective completely unlearned model $A'$ and $B'$, if $d(A,A') = m$ and $d(B,B') = n$ in the weight space, then if $m \leq n$ we will say that A is better unlearned than B as in our context these distances are from the terms that still have $x*$ . The significance of this is that we can directly compare different models and approaches by the error we get, and thus give provable claims on which models unlearn better.


\todo{np we discussed this on the call but I feel this paragraph doesn't handle this well yet. right now i am fairly confident we can say that we can compare d(A, A') and d(A, A'') where A' and A'' are two models unlearned from A. but I don't feel we can compare unlearned models obtained from two different and unrelated initial models}


\end{comment}

%\subsection{Our Unlearning metric}

%As will be presented in the following section, we give an approximation for SGD, and in doing so a natural unlearning procedure and it's error. This error will be our unlearning metric as it gives a ubiquitous value for how well an unlearning approach is expected to perform; regardless of length of training scheme, model, we know the smaller this is the better. To get an intuition for this, simply note that we know that it's easier to unlearn one step rather than many, which is seen when considering the error absolutely, but not necessarily true when taking it relative to the first term.


==> Contents/Unused/4_Verification_Error_Best.tex <==
\section{Focusing on Verification Error}
\label{sec:Focusing on Verification Error}

%Looking at the taxonomy, one of the main issues we see is the diversity of different metrics used; it is fair to say the field has diversified into many different branches. It is a benefit for the field to look into relating these metrics in order to understand them holistically, and possibly understand the benefits that one metric might have compared to another.

The goal of this section is to show that focusing on verification error we can unify the main pursuits people have looked at for measuring {\bf D1} for approximate unlearning; that is we'll show a bound on average verification error leads to a uniform bound on the difference of probability density functions of the final weights for a specific approximate unlearning approach and retraining (making some reasonable assumptions), and vice versa. A uniform bound, and more importantly a uniform convergence to 0 on that bound, is generally a strong condition, and it's easy to see how it gives DP like guarantees, and guarantees of a similar form to that considered by Guo et al \cite{guo2019certified}. We leave relating uniform bounds to KL divergence for future work (or possibly previous results we are not aware of).

We also illustrate how verification error is analogous to the verification error associated with a proof of learning \cite{jia2021proof}, and more importantly how then focusing on verification error could be important for the concept of a proof of unlearning where an entity is required to prove to a verifier they trained without a data point $\mathbf{x}^*$. 

\subsection{Uniform Bounds and Verification Error}

\subsubsection{Distribution Difference Uniformly bounded by Verification Error}
\label{sec:Probability Difference bounded by Verification Error}

The focus here will be first comparing the probability distributions of final weights coming from training $m$ epochs starting at a fixed initial weight $\weights_0$ with dataset $D$ and dataset $D'= D-\mathbf{x}^*$ with SGD (and not mini-batch SGD, i.e considering batch sizes of 1); we will represent the density functions respectively as $\mathbb{P}(\weights)$ and $\mathbb{P'}(\weights)$. We'll later see how this analysis immediately translates to understanding the difference in density function of $\mathbb{P'}(\weights)$ and $\mathbb{P''}(\weights)$ (the density function after an approximate unlearning method).

Before proceeding, if we let $n$ be the size of $D$, let us denote $I = \{\mathbf{x}_{i_1},\mathbf{x}_{i_2},\cdots,\mathbf{x}_{i_{mn}}\}$ as a particular ordering of the datapoints when training on $D$ for $m$ epochs; note we have $(n!)^m$ such combinations, and for $D'$ we similarly have $(n-1)!^m$ such combinations. To each $I$, we associate to it $I' = I-\mathbf{x}^*$ where here $I-\mathbf{x}^*$ means removing all the instances of $\mathbf{x}^*$ in $I$ while preserving the ordering. Note for a given $I'$, which is an ordering of batches when trained on $D'$, we have $n^m$ corresponding $I$ as for each epoch we have $n$ choices to place $\mathbf{x}^*$ per epoch, and $m$ epochs in total.

%\anvith{this paragraph is mostly new, I bascially made the definition of $\weights_I$ and $\weights_{I'}$ more formal}
Now, let $\weights_I$ represent the deterministic final weights resulting from training with the data ordering $I$ starting from $\weights_0$, and we now introduce the random variable $\mathbf{g}$ which represent the noise when training for $nm$ steps, and so the random variable representing the final weights when training with $I$ is $\mathbf{z}_{I} = \weights_I + \mathbf{g}$. Similarly, we define $\mathbf{z}_{I'} = \weights_{I'} + \mathbf{g}'$ where $\mathbf{g}'$ represents the noise when training $(n-1)m$ steps. Note that if training is deterministic, we have $\weights_{I'} = \weights_{I} - \mathbf{d}_I$ where $\mathbf{d}_I$ is some constant that only depends on $\weights_0$, which we've fixed, and the ordering $I$ (as $I'$ is function of $I$ as described earlier by definition). Lastly, we make an assumption that the noise from training with $nm$ steps is equivalent to that training from $(n-1)m$ steps, i.e that $\mathbf{g}$ = $\mathbf{g}'$; this is based on the fact that this noise should only be a function of the number of training steps, and that noise per step is negligible (i.e almost 0), and so adding or removing $m$ steps (1 per epoch) when compared to the $nm$ total steps when training with ordering $I$ is insignificant. Thus we have $\mathbf{z}_{I'} = \mathbf{z}_{I} - \mathbf{d}_{I}$.

Now note that, assuming the probability of a given batch ordering is constant (i.e a uniform distribution of batch orderings), and if $\mathbb{P}_I(\weights)$ is the density function corresponding to $\mathbf{z}_{I}$ and $\mathbb{P'}_{I'}(\weights)$ is the density function corresponding to $\mathbf{z}_{I'}$ (which note by above is equal to $\mathbb{P}_{I}(\mathbf{w}-\mathbf{d}_{I})$), then $\mathbb{P}(\weights) = \frac{1}{n!^m}\sum_{I}\mathbb{P}_{I}$ and $\mathbb{P'}(\weights) = \frac{1}{(n-1)!^m}\sum_{I'}\mathbb{P'}_{I'}(\weights)$.

Thus we have:
%\anvith{corrected slight typo in below calculations}
\begin{multline}
||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2} = \\ 
||\mathbb{P}(\weights) - \mathbb{P'}(\weights) +  \frac{(n-1)!^m}{n!^m}(n^m\mathbb{P'}(\weights) - n^m\mathbb{P'}(\weights))||_{2} \\
\leq ||\frac{1}{n!^m}\sum_{I} \mathbb{P}_I(\weights) - \mathbb{P'}_{I'}(\weights)||_{2} + |(\frac{(n-1)!^mn^m}{n!^m}-1)|\mathbb{P'}(\weights) \\
\leq \frac{1}{n!^m}\sum_{I} ||\mathbb{P}_I(\weights) - \mathbb{P}_{I}(\mathbf{w}-\mathbf{d}_{I})||_{2}     
\end{multline}

Where the step from the first line to the second line follows form noting that by having $n^m$ copies of $(n-1)!^m\mathbb{P'}(\weights) = \sum_{I'}\mathbb{P'}_{I'}(\weights)$ we can associate to each $\mathbb{P}_I(\weights)$ it's corresponding $\mathbb{P'}_{I'}(\weights)$, which comes from the previous remark on counting of $I$ and $I'$. Also here $||\cdot||_{2}$ simply represents the euclidean norm.

\varun{can state the text below is a lemma and move the detailed derivation to the appendix; this will allow you to define lesser notation + keep the discussion crisp}\anvith{yeah I agree}

%Now if we assume every $\mathbb{P}_I$ is lipschitz (which is true for Gaussian noise), then $||\mathbb{P}_I(\weights) - \mathbb{P}_I(\mathbf{w}-\mathbf{d}_{I})||_{2} \leq L_I||\mathbf{d}_I||_{2}$; furthermore as generally all $\mathbb{P}_I$ are just the same distributions but shifted (as we have the same noise for each), we have all the $L_I$ are equal, i.e $L_I = L$ for every $I$. Lastly if we let $d$ be the average of all the $\mathbf{d}_I$, that is $d = \frac{1}{n!^m}\sum_{I} ||\mathbf{d}_I||_{2}$, we have

%\begin{equation}
%\label{eq: l2_prob_difference_1}
%||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2} \leq Ld
%\end{equation}

%which gives a uniform bound on the l2 difference of $\mathbb{P}(\weights)$ and $\mathbb{P'}(\weights)$.

The above analysis leads to the following lemma which gives a uniform bound on the l2 difference of $\mathbb{P}(\weights)$ and $\mathbb{P'}(\weights)$:

\begin{lemma}
If every $\mathbb{P}_I$ is lipschitz with constant $L$ (true if $\mathbf{g}$ is gaussian), and if we let $d = \frac{1}{n!^m}\sum_{I} ||\mathbf{d}_I||_{2}$, then:

\begin{equation}
\label{eq: l2_prob_difference_1}
||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2} \leq Ld
\end{equation}

\end{lemma}

So far we've looked at the difference between $\mathbb{P}(\weights)$ and $\mathbb{P'}(\weights)$, however in general we're interested the difference between $\mathbb{P''}(\weights)$, the density function after an approximate unleanring method on $M$, and $\mathbb{P'}(\weights)$. If the approximate unlearning method only looks at $\weights_0$ and $I$ and to $\weights_I$ obtains the approximately unlearned weights $\weights_{I}'' = \weights_I + u_I$ where $u_I$ is some unlearning update we get the following corollary:

%To understand how this relates to verification error and approximate unlearning, let's consider an approximate unlearning method which only looks at $\weights_0$ and $I$ and to $\weights_I$ obtains the approximately unlearned weights $\weights_{I}'' = \weights_I + u_I$ where $u_I$ is some unlearning update. Note then we can analogously define a $\mathbf{z}_{I}''= \weights_{I} + \mathbf{u}_I + \mathbf{g}$ as before with corresponding density function $\mathbb{P}''_{I}(w)$. Defining $\mathbf{v}_I = \mathbf{u}_I + \mathbf{d}_I$ we get $\mathbf{z}_{I'} = \mathbf{z}_{I}'' - \mathbf{v}_I$ where $\mathbf{v}_I$ represents the analytic (ignoring noise) verification error for the given ordering $I$ (i.e the difference between the weights obtained from the approximate unlearning $\weights_{I}''$ and the retrained weights $\weights_{I'}$). At this point it's clear all the previous steps follow and defining $v$ as the average of all the $||\mathbf{v}_I||_2$ we get

\begin{corollary}
If every $\mathbb{P}_I$ is lipschitz with constant $L$ (true if $\mathbf{g}$ is gaussian), and if we let $v = \frac{1}{n!^m}\sum_{I} ||\mathbf{d}_I + \mathbf{u}_I||_{2}$, then:

\begin{equation}
\label{eq: l2_dif_bounded_ver_err}
||\mathbb{P''}(\weights) - \mathbb{P'}(\weights)||_{2} \leq Lv
\end{equation}

\end{corollary}

%where now $\mathbb{P''}(\weights) = \frac{1}{n!^m}\sum_{I}\mathbb{P}''_{I}$ represents the probability density function of the weights after applying the approximate unlearning method on $M$ to obtain $M''$. 

This gives us a uniform bound on the difference of the probability distribution after approximate unlearning and the ideal retraining, but note the necessary assumption on the form of this approximate unlearning method; to get the Bound \ref{eq: l2_dif_bounded_ver_err} we require the unlearning method to only be dependant on the initial weight $\weights_0$ and $I$. At the moment it isn't clear how someone would do this, but that's what we'll do later. The main takeaway for now is that verification error does give us a uniform bound on the difference in probability distributions between the approximate unlearning method and ideal retraining.

\subsubsection{Verification Error bounded by Uniform Bound on Distribution Difference}

We now proceed to get a bound on the average verification error $v$ based on a uniform bound between the density function after the approximate unlearning and the density function for ideal retraining.

Note, assuming the noise has $0$ mean, $v$ is simply the difference in expectation of $\mathbb{P''}(\weights)$ and $\mathbb{P'}(\weights)$, and let us for the time being assume that the union of the support of $\mathbb{P''}(\weights)$ and $\mathbb{P'}(\weights)$ is bounded, i.e if $\mathbf{W}$ is the union of the supports, then $\int_{\mathbf{W}} ||\weights||_{2} d\weights = a < \infty$. This is reasonable as we'd expect the noise from training to be bounded; in fact in general we'd only need the integral outside a bounded domain to be finite, but the reasoning is analogous to what follows and would simply add an extra constant term. Now if say $||\mathbb{P''}(\weights) - \mathbb{P'}(\weights)||_{2} < b$ for some scalar $b$ for all $w$ (i.e $b$ is a uniform bound), we have:

\begin{multline}
\label{eq:exp_ver_err}
v = ||\mathbb{E}(\mathbb{P''}(\weights)) - \mathbb{E}(\mathbb{P'}(\weights))||_{2} \\
= ||\int_{\mathbf{W}} \mathbb{P''}(\weights) \weights d\weights - \int_{\mathbf{W}} \mathbb{P'}(\weights) \weights d\weights||_{2} \\
\leq \int_{\mathbf{W}} ||\mathbb{P''}(\weights) - \mathbb{P'}(\weights)||_{2} \cdot ||\weights||_{2} d\weights \\
\leq ba
\end{multline}

and so in this sense we see reducing the max value of $||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2}$ gives a smaller bound on the expectation of verification error $v$.

Thus we see the relation between verification error and $||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2}$ runs both ways (i.e reducing either gives a tighter bound on the other), and as $||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2}$ captures the difference in probability distributions when training with and without a datapoint $\mathbf{x}^*$, we generally expect that similar metrics trying to minimize the shift in the probability distributions would follow similar relations as described above.

\subsubsection{Main Takeaway from Bounds}

What we've shown with the two Bounds \ref{eq: l2_dif_bounded_ver_err}, \ref{eq:exp_ver_err} is that decreasing the average verification error decreases the uniform bound on the difference in probability density functions, and decreasing the uniform bound on the probability density functions decreases the bound on the average verification error; we've shown they are practically interchangeable if one is simply interested in bounds.

This is of interest as note if $||\mathbb{P''}(\weights) - \mathbb{P'}(\weights)||_{2} < b$ then we have $\mathbb{P''}(\weights) \leq b + \mathbb{P'}(\weights)$ and $\mathbb{P'}(\weights) \leq b + \mathbb{P''}(\weights)$, giving bounds reminiscent of DP and that used by Guo et al \cite{guo2019certified}; so we see by working with the uniform bound we retrieve bounds of the form used by the other work we mentioned trying to measure {\bf D1}. The link to KL divergence is less obvious to us (though it should be there as generally a uniform bound is a strong condition) so we leave it for future work to resolve, or possibly past work we are not aware of.

\subsection{Verification Error and Proof of Unlearning}

\varun{this seems like a good point to discuss in a later section (say discussion) and less so here; also, if i use an approximate unlearning method to "unlearn" -- i can log those steps along with the original proof and the resulting proof is still "valid" (as it's not really non deterministic in your case or in the case of amnesiac unlearning) -- this is not really expensive is it?} \anvith{I don't think I completely understand what you mean by logging unlearning steps, but we can talk about it in our meeting. Generally yes I agree I think this is good for the discussion. I originally put it here thinking it further motivates why we look at the verification error, but now I see how it really just disrupts the flow as we don't refer to it anywhere else- if anything we can just gives a brief pointer to this in section 4.3}.

What follows is another way of conceptually grasping why verification error is a good metric. So far it's been introduced as simply a metric to measure similarity in weights, however as we'll discuss, there is a natural way to talk about a \textit{proof of unlearning} based on the work done by Jia et al \cite{jia2021proof}, which also introduces their own \textit{verification error} to measure whether a said proof of learning should be accepted. In a specific context, these two verification errors are the same, and so alternatively we can say approximate unlearning methods aimed at reducing unlearning verification error amount to giving a \textit{cheap proof of unlearning} as we explain below; this we believe illustrates a viable practical procedure for how unlearning may be employed and verified by an entity.

\subsubsection{Proof of Unlearning}

A Proof of Learning $\mathfrak{P}$ is a a tuple consisting primarily of an ordered set of checkpoints $\mathfrak{W}$ taken during training with some check-pointing frequency $k$, and the ordered sequence of data points $\mathfrak{X}$ appearing during training, alongside various hyper parameters needed to reconstruct training. We say that $\mathfrak{P}$ is valid only if the associated verification error, i.e the difference between what an entity says they obtained for their weights at the n'th checkpoint, and what the verifier obtained when recreating the sequence of weights, is always below some threshold.

Thus if an entity claims to have unlearned, i.e to have never trained on $\mathbf{x}^*$, we could explicitly verify this by asking for a $\mathfrak{P}'$ such that $\mathbf{x}^* \not\in \mathfrak{X}'$. If this $\mathfrak{P}'$ passes verification, then we can say this is a \textit{proof of unlearning}.

\subsubsection{Costs and Becoming lazy}

The issue with the setup above is that providing $\mathfrak{P}'$ requires explicitly retraining, as based on the work from Jia et al \cite{jia2021proof}, obtaining a valid cheaper spoof is difficult (currently have no such methods). So in practice, as of now, obtaining a proof of unlearning means retraining, and thus is expensive.

However we can be lazy, and instead of properly retraining immediately after getting an unlearning request in order to obtain a valid $\mathfrak{P}'$, we instead only obtain the final weights of a valid proof (possibly cheaply by approximating them) and compute the rest of the proof some time in the future when it is needed; the benefit to this strategy is not having to retrain every time a request is sent, and only doing it once upon needing to provide a proof (saving costs). 

The associated verification error for the proof we finally give (more precisely the error in verifying the only step that might not pass verification which is the last one) is then the difference between the final weights you computed/approximated, and final weights you would obtain from the true $\mathfrak{P}'$; we assume you cannot change your final weights to those obtained from $\mathfrak{P}'$ as some entity would notice this and call foul play.

Here, the final weights obtained by this valid $\mathfrak{P}'$ are the weights of $M'$, and using an approximate unlearning method the final weights one would have obtained are those of $M"$. Thus the verification error for the proof is simply the difference in these two weights, which is what we've been calling the verification error for unlearning.

Thus approximate unlearning methods that reduce verification error can be employed to give a \textit{cheap proof of unlearning} following the setup just described.

\subsection{Drawback of Verification Error}

\varun{@varun:reword}

So far we've justified verification error as being a good metric as it unifies other metrics and is the same as the error used to verify a proof of unlearning. However verification error has it's own drawbacks.

Primarily, computing verification error to know what it is after employing a certain method would require first computing $M'$, at which point one might as well use $M'$ as their unlearned model. It's also not clear what variables we should focus on to decreases verification error. Furthermore, based on the analysis in Section \ref{sec:Probability Difference bounded by Verification Error} we have to focus on approximate unlearning methods that only focus on the initial weights and ordering $I$.

What we proceed to do is to first tackle this last problem by understanding the deterministic impact (so ignoring noise) of a data point $\mathbf{x}^*$ on the final weights of a model when trained starting at $\weights_0$; we do this by obtaining and analyzing a closed form approximation of SGD. This leads to an unlearning method that only depends on the initial weights $\weights_0$. We then find a proxy metric, which we call our \textit{unlearning error}, for the associated verification error, which allows us to approximate the verification error cheaply by only recording some values during training. Lastly our approximation of unlearning error explicitly shows what variables we want to decrease to decrease it, and we later verify that in fact decreasing our unlearning error decreases the verification error (which also serves to show unlearning error is a good proxy for verification error).


%So we see in this context that our verification error and the verification error from POL (proof of learning) are the same. A future direction of work could be to find a way to distribute this error throughout the steps in the proof as to pass verification more easily (that is to push each of the weights slightly in the direction of the final weight of $M''$ when retraining, as to distribute the error across the steps, and possibly pass verification for each step); doing this we'd understand by association the unlearning error we should aim for- that which roughly corresponds to the desired verification error which when distributed over the steps would pass verification.

%Now to understand how this relates to verification error, let us denote $\textit{w}$ , $\textit{w'}$ and $\textit{w''}$ as the expected weights of $M$, $M'$, and $M''$ respectively, where $M''$ is obtained form some approximate unlearning method which changes the weights. Then note $d = ||w - w'||_{2} \leq ||\mathbf{w}-w''||_{2} + ||w'' - w'||_{2}$, and note that $||w''-w'||_{2}$ is the average verification error, which we'll denote as $v$. We see we then have the bound $||\mathbb{P}(\weights) - \mathbb{P'}(\weights)||_{2} \leq L(||\mathbf{w}-w''||_{2} + ||w'' - w'||_{2})$, and now if we were to apply the approximate unlearning method on $M$ to make it $M''$ then the first term would go away (as the distributions are the same now)







==> Contents/Unused/4_unlrn_err_good.tex <==
\section{Evaluating our Approximation}
\anvith{overview is what is in the google doc, I suggest first presenting the correlation with verification error as the first subsection, then tying this to the question of how do other things correlate}

\subsection{Correlation with True Discrepancy}
Although we provided a theoretical derivation of the unlearning error and how it correlates to the true discrepancy between $\model$ and $\model''$, we may be interested in this correlation empirically and in a practical setting. We consider training standard computer vision model, ResNet-18 and VGG-19 on the CIFAR10 and CIFAR100 dataset (specifics about the model and dataset are left in the appendix). The notation we will be using is the following: for a dataset $D$, we train a model $\model_{0}$ on $D$ for $T$ iterations to get to model $\model_{T}$. We can represent $\model_{0}$ and $\model_{T}$ by their parameters $w_0$ and $w_{T}$, respectively. The experimental setup is as follows:
\begin{enumerate}
    \item Pretrain $\model_{0}$ by training $\model_{0}$ on the entirety of $D$ for N steps until we reach $\model_{N}$.
    \item Train $\model_{N}$ for a small number of steps $T$ on batches of data $\{x_1,x_2,\dots,x_T\}$ to get $\model_{N+T}$. We will consider $\model_{N+T}$ the model we wish to unlearn and WLOG the point we wish to unlearn is in batch $x_{1}$.
    \item Train $\model_{N}$ for $T-1$ steps on batches $\{x_2,\dots,x_T\}$. The resulting model is the naively retrained model $\model^{'}$ without batch $x_{1}$.
    \item Get $\model^{''}$ via adding back the gradient in the easy to computer term:
    $$ M^{''} = M_{N+T} + \eta  \frac{\partial L}{\partial w}|_{w_{N+T},x_1}$$
    \item Compute the unlearning error of $M_{N+T}$ and the true discrepancy between between $M^{'}$ and $M^{''}$.
\end{enumerate}
%By varying $T$, the number of finetuning steps, we can determine the correlation between the unlearning error and the true discrepancy. $N$, the number of pretraining steps is important to set. At one extreme, $N=0$ corresponds to a model that has learned nothing and has likely learned very little by finetuning T steps. On the other hand, $N \rightarrow \infty$ will result into a model that that has likely already reached a local minimum. This would result into $\model_{N} \approx \model_{N+T} \approx \model^{'} \approx \model^{''}$ as the gradient at each SGD update is close to zero.

The correlation between the true discrepancy and unlearning error for both datasets and both models trained for 80 epochs is shown in figure~\ref{fig1:ind_corr_bs=16}. For each scenario, a batch size of 16 was used for the finetuning process and the verification and unlearning error were measured every 100 SGD updates for a total of 5 finetuning epochs. The correlation values are 0.967, 0.971, 0.959 and 0.955, respectively. We see that the correlation is significant across all 4 settings.


\begin{figure*}[htp]
  % Fixed length
  \centering
  \subcaptionbox{ResNet18 - CIFAR10\label{fig3:a}}{\includegraphics[width=1.63in]{plots/cifar10_resnet.png}}\hspace{1em}%
  \subcaptionbox{VGG19 - CIFAR10\label{fig3:b}}{\includegraphics[width=1.63in]{plots/cifar10_vgg.png}}\hspace{1em}%
  \subcaptionbox{ResNet18 - CIFAR100\label{fig3:c}}{\includegraphics[width=1.63in]{plots/cifar100_resnet.png}}\hspace{1em}%
  \subcaptionbox{VGG19 - CIFAR100\label{fig3:d}}{\includegraphics[width=1.63in]{plots/cifar100_vgg.png}}
  
 \caption{Unlearning error and verification error over 5 epochs of finetuning for 4 scenarios pretrained for 80 epochs. Unlearning error and verification error measured every 100 SGD steps for a total of 156 measurements. The correlation from (a) to (d) are 0.967, 0.971, 0.959 and 0.955, respectively.}
\label{fig1:ind_corr_bs=16}
\end{figure*}
Additionally, we would like to see if this correlation still holds across settings of finetune and pretrain batch sizes, number of pretraining epochs and models. Figure~\ref{fig2:causation} shows 160 different settings of hyperparameters for both CIFAR10 and CIFAR100. The correlation for CIFAR10 and CIFAR100 over these settings are 0.866 and 0.863, respectively. \gabe{Is there where we should have plots that divide this up by each parameter and discuss it's affect? ie: do we have a table with correlation values where 1 out of the N parameters change and the rest vary and we have a correlation for each and we discuss where our method begins to break. For example, if you pretrain a very small amount, sigma makes no sense}.

\begin{figure*}[htp]
  % Fixed length
  \centering
  \subcaptionbox{CIFAR10\label{fig3:a}}{\includegraphics[width=3.26in]{plots/big_cifar10.png}}\hspace{1em}%
  \subcaptionbox{CIFAR100\label{fig3:b}}{\includegraphics[width=3.26in]{plots/big_cifar100.png}}
 \caption{Unlearning error and verification error for 160 different settings for both CIFAR10 and CIFAR100}
\label{fig2:causation}
\end{figure*}

%The true discrepancy and unlearning error as a function of the number of fine-tuning steps for 20 epochs of pretraining is shown in figure~\ref{fig1:corr20}. We notice that as $T$ increases, the verification error is monotonically increasing (color gradient only increasing as a function of y-value). On the other hand, unlearning error generally increases as function of $T$ but due to the inherent noisiness of calculating singular values of a hessian over a batch (shown in figure~\ref{fig:noisy_sigma}), it may sometimes decrease. Regarding the relationship between the true discrepancy and unlearning error, we get a correlation value of 0.9108 up to $T=100$ and 0.856 up to $T=200$. This is indicated by the strong linear relationship at smaller $T$ in dark red and starts to degrade at larger $T$ in the greens and dark blues. This degradation is due 




\subsection{How does Membership Inference Compare?}

\section{Reducing unlearning error}
\gabe{This is where the initial experiments of hessian loss function will come into play}

==> Contents/Unused/5_SGD_approx_copy.tex <==
\section{Defining the Unlearning Error}
\label{sec:A Closed Form Approximation of SGD}

%As noted earlier, there is a tension associated with defining what it means to truly unlearn: does it require similarity between the distribution of weights (definition (a)) or the distribution of outputs (definition (b))? However, note that what is common to both is understanding the effect of a datapoint $\mathbf{x}^*$ on a model trained on it. The effect of $\mathbf{x}^*$ is viewed through its influence on the sequence of training updates, which in turn changes the weights learned. Thus, the change in outputs can be viewed as a byproduct of the change in weights.

What follows is an approximation of the outcome of SGD using a Taylor series, and a subsequent analysis of the approximation. The main outcome is an understanding of the \textit{closed form} (approximate) effect of $\mathbf{x}^*$ on the final weights of a model. Specifically what we can forgot for little cost and only depends on $w_0$ (which will define our unlearning method), and what is more expensive to forget which will be our verification error. We then approximate this verification error to obtain our \textit{unlearning error}.

%In particular, we obtain a decomposition of SGD into (a) terms one can seemingly forget \textit{cheaply}, and (b) terms that would require at least as much computation to forget as training. Unlearning is possible by simply removing (a subset of) these terms from the final weights. Note that from these \textit{expensive} terms (category (b)), we can estimate an \textit{unlearning error} which represents the distance in the weight space between the naively retrained $M'$ and the model $M''$ we get by unlearning as above. The remainder of this paper is centered around how one can reduce the unlearning error. 

\subsection{Expanding SGD} 

We begin with the definition of a single SGD learning update:

% \varun{use $\mathbf{w}$ for weights}
% \anvith{changed so macro \weights is boldface, using that}

\begin{equation}
\label{eq1:}
\weights_{1} = \weights_0 - \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0}
\end{equation}

where $\mathbf{w}_0$ denotes the weights at step 0, and $\hat{\mathbf{x}}_0$ denotes the mini-batch of data sampled at step 0. We obtain $\weights_{2}$ as follows:

\begin{equation*}
\weights_{2} = \weights_0 - \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0} - \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_1,\hat{\mathbf{x}}_1}
\end{equation*}

\begin{equation}
\implies \weights_{2} = \weights_0 - \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0} - \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0-\eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0},\hat{\mathbf{x}}_1}
\end{equation}


This can further be expanded and approximated as follows:

\begin{equation}
\weights_{2} \approx \weights_0 - \eta (\frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0} + \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_1} + \frac{\partial^2 \mathcal{L}}{\partial^2 \weights}|_{\weights_0,\hat{\mathbf{x}}_1} (- \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0}))
\end{equation}

Our end goal is obtaining a closed form that explicitly only depends on the initial weights $\mathbf{w}_0$ and sequence of mini-batches of data. To scale the above for a sequence of $t$ updates, notice that the hessian terms from the expansion recursively depend on each other. Thus we have the final approximation:

\begin{equation}
\weights_{t} \approx \weights_0 - \eta \sum_{i=0}^{t-1} \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_i} + \sum_{i=1}^{t-1} f(i) \label{eq:approx}
\end{equation}

where $f(i)$ is defined recursively as:
\begin{equation}
\label{eq: recursivedef}
f(i) = -\eta \frac{\partial^2 \mathcal{L}}{\partial^2 \weights}|_{\weights_0,\hat{\mathbf{x}}_i} (- \eta \sum_{j=0}^{i-1} \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_j} + \sum_{j=0}^{i-1} f(j))
\end{equation}

with $f(0) = 0$.

% \subsection{Understanding The Approximation}
% \label{sec:approximation}

% \varun{equation broken}
% \anvith{yeah I'm blind and didn't realize I already had a label for the equation, which I put at the end}

\paragraph{Understanding The Approximation:} From Equation~\ref{eq:approx}, observe that one can represent the weights obtained after training $t$ updates as the sum of two sums. We now wish to understand how $\mathbf{x}^*$ affects this expression (and thus the approximate outcome of training). The terms in the \textit{first sum} are simply gradients taken with respect to the initial weights $\weights_0$ and a mini-batch $\mathbf{\hat{\mathbf{x}}_i}$ following the order we give data to the model. Notice, however, that the exact order does not matter as we are simply adding them. In this case, it is clear that the effect of $\mathbf{x}^*$ (provided at any step in training) on this first sum is a gradient (or gradients) computed with respect to $\weights_0$ and $\mathbf{x}^*$. To reverse this effect, we simply have to \textit{add back these gradients} (times the learning rate $\eta$ and $\frac{1}{b}$ where $b$ is the batch size)\footnote{Note that gradients on mini-batches are just a sum of the individual gradients on each datapoint averaged, so in fact we can single out the gradients from just $\mathbf{x}^*$ which are multiplied by $\frac{1}{b}$ from averaging.}.  This process is computationally inexpensive. 
% , as it amount to simply adding $\frac{\eta m}{b} \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_0}$, where here $m$ is the number of times $\mathbf{x}^*$ appear in a mini-batch during training (i.e the cost is a single gradient computation). 

% \varun{well, you have to store all of these updates ... }
% \anvith{no we don't, we just need the initial weights and the datapoint; I added a bit more detail to make this clearer, it amounts to a single gradient computation}

The \textit{second sum} is more complex, as the expression is recursive, and there is an inherent dependence on order. To compute all the terms that contain a particular $\mathbf{x}^*$, one would in the case of proper SGD (i.e mini-batch size of 1) require as much compute at training; this term behaves as an upper-bound on how well we can cheaply unlearn. In \S~\ref{sec:approximation}, we describe how one can estimate the magnitude of this term, which we call our \textit{unlearning error}--this term captures the verification error we expect between perfectly removing the effect of $\mathbf{x}^*$ on our model, i.e. perfectly retraining to obtain $M'$, and what we can cheaply do by removing the effect of $\mathbf{x}^*$ on the first sum i.e., our $M''$. Note the method to remove the effect of $x^*$ in the first sum is our unlearning method, which we'll later couple with a regularizer on the loss function to improve its effectiveness (i.e minimizes our unlearning error).


%The first important detail to note is that the first sum is commutative with respect to the indices; that is, any permutation of $\hat{\mathbf{x}}_{i}$ results in the same value. Thus, we will continue call this the order independent part.

%The recursive component is not invariant to permutations, and so we will call it the order dependent part.

%Though we leave it to later sections to further elaborate, the error we're interested between $w'_t$ and $\weights_t$ is approximated by the magnitude of the order dependent part averaged over the size of the dataset, i.e the contribution of a given datapoint to that term; this is simply as the modified state $f'$ we can feasibly achieve undoes the effect of a given $x*$ on the first part, but not the second, and thus the approximate associated error is the contribution of $x*$ to the second term.

%\subsection{Understanding Order Independent Component}

%There is not much to say now other than this introduces an ideal scenario in order to remove updates, i.e unlearn. This is also analogous to the update rule in distributed learning and batch SGD.

\subsection{Approximating the Second Sum Series}
\label{sec:approximation}

The global structure of the second sum follows $\eta^2 c_{t} + \eta^3 c_{t-1} + ... +\eta^{2+t-1} c_{1}$, where $c_{i}$ represent a vector. Thus, we can focus primarily on the $\eta^2$ dependent term as $\eta$ is almost always a magnitude or more less than $1$ and so $\eta^2$ is the dominate term (in the case it's not less than 1 focusing on $\eta^2$ will be wrong in the sense that we're ignoring other more dominant terms). Thus, the second sum can be rewritten as:

\begin{equation}
\label{eq:error}
\eta^2 c_{t} = \sum_{i=1}^{t-1} \eta^{2} \frac{\partial^2 \mathcal{L}}{\partial^2 \weights}|_{\weights_0,\hat{\mathbf{x}}_i}  \sum_{j=0}^{i-1} \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_j} 
\end{equation}

We can further approximate $\sum_{j=0}^{i-1} \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_j}$ by its expectation $\frac{i(\weights_{t}-\weights_{0})}{t}$. We further normalize the vector, and thus have:

\begin{equation}
\label{eq: Detailed_Aprox}
\eta^2 c_{t} \approx \eta^{2} \frac{||\weights_{t}-\weights_{0}||_{2}}{t} \sum_{i=1}^{t-1} \frac{\partial^2 \mathcal{L}}{\partial^2 \weights}|_{\weights_0,\hat{\mathbf{x}}_i} \frac{\weights_{t}-\weights_{0}}{||\weights_{t}-\weights_{0}||_{2}} i
\end{equation}


% \varun{what does $||.||$ denote?}
% \anvith{l2-norm, I'm going to add it as a subscript}

By focusing on $||c_{t}||_{2}$, note that 

$$||\frac{\partial^2 \mathcal{L}}{\partial^2 \textbf{w}}|_{\textbf{w}_0,\hat{\mathbf{x}}_i} \frac{\textbf{w}_{t}-\textbf{w}_{0}}{||\textbf{w}_{t}-\textbf{w}_{0}||_{2}}||_{2} \leq ||\frac{\partial^2 \mathcal{L}}{\partial^2 \textbf{w}}|_{\textbf{w}_0,\hat{\mathbf{x}}_i}||_{2}$$ 

by definition of the induced $\ell_{2}$ norm, which is simply the square root of the largest eigenvalue of the hessian , i.e., $\sigma_{1,i}$ the first singular value of the hessian on $\hat{\mathbf{x}}_{i}$. For sake of simplicity we consider $\sigma = \max(\sigma_{1,i})$, and thus have:

\begin{equation}
||\eta^{2} c_{t}||_{2} \leq \eta^{2} \frac{||\weights_{t}-\weights_{0}||_{2}}{t} \sigma \frac{t^{2} - t}{2} \label{eq:error bound}
\end{equation}

Thus, we can observe that the second sum linearly depends on $||\weights_{t}-\weights_{0}||_{2}$, $\sigma$, and $t$. $\sigma$ captures the non-linearity of the loss landscape from the hessian, and thus we see that the more linear the loss landscape, the lower the value. We also see from this that in the scenario $t=1$ or $\sigma = 0$, this bound, and thus the term, is 0.  

%this insights motivate what we later do in trying to reduce this.

%Though this bound is nice for the intuitive picture of what is going on, it can be a rather loose bound to work with as we took $\sigma = max(\sigma_{1,i})$, so for our later experiments we will stick to approximating \ref{eq: Detailed_Aprox} by taking the average singular values over epochs.

% \varun{what is the takeaway from this explanation?}
% \anvith{mainly to have a nice equation that gives an intuituve understanding of what is goinf on, it's also what gives the insights into what we later try to reduce it (added a brief blurb at the end of the second last paragraph on that point)}

%\todo{np: this is cool for intuition. you should illustrate the intuition we discussed on our call for each of the terms of the bound on a linear model where you know that everything will hold exactly. you could also consider a deep linear network (look up on internet there is long line of work started by andrew saxe) to make things more interesting with non-linear learning dynamics}

%\anvith{That sounds interesting, I'm taking a look into it. What's actually weird is that the non-linearity of the loss, i.e value of the hessian, is actually dominated by the contribution from the final softmax (see equation 10 and the discussion above it from "Emergent properties of the local geometry of neural loss landscapes"), but I guess those deep linear networks wouldn't have a softmax (or at least those that don't are the ones we'd look at to see extremely low to no error)}

%Perhaps most importantly, this quantity is seemingly the same units as the loss, as we expect $||\weights_{t}-\weights_{0}|| \propto t$, and units of $\sigma$ are $\frac{loss}{w^2} = \frac{loss}{t^2}$, thus all together we have  $\frac{loss * t^3}{t^3} = loss$. This helps justify the universality of our $d(A,A')$ if indeed the loss is a universal metric (i.e comparable between models and datasets).

%However in general we expect $||\weights_{t}-\weights_{0}|| \propto t$, and so we expect a quadratic growth with $t$ (or at least a faster growth than simply linear) but interestingly, experimentally we found that the error grows linearly with t, suggesting that $||\weights_{t}-\weights_{0}||* \sigma = constant$.


%\subsection{Noteworthy Properties}
%So far in our analysis we have set $\weights_{0}$ and $\weights_{t}$ to be arbitrary, though perhaps implied that they are the starting and end point in training. In general we can consider any $\weights_{0}$ and $\weights_{n}$, and split this further into smaller arbitrary intervals $\weights_{0},\weights_{t},\weights_{2t}, ... \weights_{n}$. Thus we see that we can simply approximate any $\weights_{i*t}$ with respect to $\weights_{(i-1)t}$ rather than needing to approximate $\weights_{n}$ with respect to $\weights_{0}$. We emphasize this now as this will be particularly relevant in our analysis of amnesiac unlearning and how pretraining is beneficial.


\paragraph{Counting Terms:} Now, with an understanding of what the dominant terms in the second sum of Equation~\ref{eq:approx} are, we can understand the computational costs needed to forget higher order terms, besides simply the first sum of Equation~\ref{eq:approx}. To do so we now focus on the expression in Equation~\ref{eq:error}, and letting $i^*$ denote the first index where $\mathbf{x}^*$ appears in a mini-batch, we are interested in what terms would contain $\hat{\mathbf{x}}_{i^*}$ and thus $\mathbf{x}^*$, i.e., what terms would we need to remove in order to forget $\hat{\mathbf{x}}_{i^*}$ from the dominant term in our second sum in Equation~\ref{eq:approx}. Note this will actually be an under count as $\mathbf{x}^*$ could appear in another batch, so the final cost we get, although already significant, will be less that what we'd need.

% \varun{not $\mathbf{x}^*$?} 
% \anvith{completely forgot to say $i^*$ is the first index $\mathbf{x}^*$ appears in, added it, so hopefully clear now?}.


%\varun{can you re-word the paragraph below? it's quite convoluted to read} \anvith{made some changes (removed some redundancies) is it better?}
First thing to note is that $\hat{\mathbf{x}}_i^*$ does not appear in any terms in the expression until $i= i^*$; for this index we see we have $i^*$ terms dependent on $\hat{\mathbf{x}}_{i^*}$ as every term in the second sum in eq \ref{eq:error} is multiplied by $\frac{\partial^2 \mathcal{L}}{\partial^2 \weights}|_{\weights_0,\hat{\mathbf{x}}_{i^*}}$. Now for all the indices $i>i^*$ (i.e $t-1-i^*$ indices), we have exactly one term with $\hat{\mathbf{x}}_{i^*}$ which comes from a $\frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_0,\hat{\mathbf{x}}_{i^*}}$ appearing in the second sum once. Lastly note that each term we see $\hat{\mathbf{x}}_{i^*}$ in is a hessian vector product, as all terms here are hessian-vector products.

So in total we have $t-1-i^*+i^* = t-1$ terms, and note that all these terms are hessian vector products (because all the terms in Equation \ref{eq:error} are hessian vector products). In general it is possible to implement hessian products in O(n) ~\cite{pearlmutter1994fast} by implementing a differential operator numerically (i.e finite differences) and so runs close to the computation required for a gradient which we would need to compute twice in order to use the method. 

%\varun{explain this in a bit more detail, but in a line?}
%\anvith{done}

%Consider that we focus on a uniform distribution over datapoints $\hat{\mathbf{x}}_i$ so that our expectation of i is $t/2$. In this case, every indexed term $j$ where $(t/2) \leq j$ will thus contain an $\hat{\mathbf{x}}_i$ in the second sum. Furthermore, the term $j=t/2$ would have $\hat{\mathbf{x}}_i$ in the hessian, meaning every term in the second sum for $i=t/2$ would have a coefficient with $\hat{\mathbf{x}}_i$. Thus on average we'd expect to compute $t$ gradients and $t/2$ hessian.


% (or well at least as expensive as computing $t-1$ of the $t$ training steps, which for all intents and purposes is practically the same)

Importantly, as these hessian vector product are at least as expensive as a gradient computation, we have that the computational requirement to compute all these terms containing $\hat{\mathbf{x}}_{i^*}$ in Equation~\ref{eq:error}, in particular just computing the $x^*$ component in these batch terms, is at least as much as computing $t$ gradient updates on a single data point (when also including the one gradient we need to compute for our unlearning method). In the case the batch size is $1$, this would be equivalent to the cost for training, and in general is $1/b$ the cost of training (where $b$ is the batch size). However this can still be a significant amount in practice (as $t$ here is not the epochs but the number of individual training steps), so we see that this second sum in Equation~\ref{eq:approx} which we can approximate with Equation~\ref{eq:error} is a bound to how well we can reasonably forget the effect of $\mathbf{x}^*$. Future work could be looking into computing all these terms and assessing the error then (by looking at the even higher order terms in the second sum of \ref{eq:aprox}).

%\anvith{below is new, realized we need to properly define unlearning error}

\paragraph{Unlearning Error} Based on the above discussions for estimating the second sum, and how it bounds how well we can unlearn (without adding on significant computational costs), we define equation \ref{eq:error bound} to be our \textit{unlearning error} $e$, with the slight modification that as in practice this bound can be loose we take $\sigma$ to be the average of all the $\sigma_{1,i}$ rather than the max, as to better approximate equation \ref{eq:error} (though without having the proper inequality for \ref{eq:error bound} given by using the max). To be precise, defining $\sigma_{avg} = \frac{1}{t}\sum_{i=1}^{t} \sigma_{1,i}$, we define unlearning error as 

\begin{equation}
e = \eta^{2} \frac{||\weights_{t}-\weights_{0}||_{2}}{t} \sigma_{avg} \frac{t^{2} - t}{2} \label{eq:unl_err}
\end{equation}


Working with the average also allows to only compute $\sigma_{1,i}$ every couple of steps instead of every step, saving costs. Lastly note computing $e$ doesn't require us to have applied our unlearning method first, we can preemptively know what the unlearning error $e$ will be.

\paragraph{Is the approximation Good} Though we have a mathematical backing for our proposed unlearning error \ref{eq:unl_err} which approximates the verification error for our unlearning method, it is still an approximation, and that too one that includes extra terms. Thus the question is whether it does in fact accurately capture the behaviour of the true verification error. However to empirically to check this, which would be to look at correlations under different scenarios, we first need to know how we can change this unlearning error. What follows is first how we can reduce the unlearning error, and then whether when we reduce unlearning error we in fact reduce the verification error (and thus whether we can conclude unlearning error is a good proxy metric).


% , and so this is our measure for the discrepancy between trying to forget the effect of some $\mathbf{x}^*$ from the first sum of Equation~\ref{eq:approx} and what a truly unlearnt model (i.e $M'$ which was retrained without $\mathbf{x}^*$) achieves for its final weights.


%This means trying to properly compute all these $\hat{\mathbf{x}}_{i^*}$ terms to remove them is infeasible, or at least if you were to do so, you might as well simply properly retrain to unlearn.


% Our goal now, having a way to unlearn (albeit for only a part of our expression), is to minimize this second sum as to more effectively forget the effect of $\mathbf{x}^*$, which will be the focus for a later section. The question now is just how good our approximation of this discrepency between the ideal $M'$ and the model we obtain we obtain by removing the effect on the first sum, $M''$ is (which we'll call our "unlearning error"), which is what we discuss in the following section.

%\todo{np you should expand discussion here to say whether there are valuable uses to computing an approximation of the hessian instead}


==> Contents/Unused/6_Reducing_Unlearning_Error.tex <==
\section{Reducing the Unlearning Error}

%\anvith{For me: brief blurb on why we want to reduce the unlearning error, i.e to make our method of unlearning more true}

As we now have a metric capturing the error associated with our unlearning scheme, which is simply adding back the gradient from the first sum in equation \ref{eq:approx}, the question now is whether we can possibly reduce it.

In section~\ref{ssec:pretraining} and~\ref{ssec:std loss}, we propose two methods to reduce the unlearning error. The following section describes our experimental setup.

\subsection{Experimental Setup}
\label{ssec:experimental setup}


We investigate unlearning for 2 classic computer vision models, ResNet-18 and VGG-19 on 2 vision datasets, CIFAR10 (10 classes) and CIFAR100 (100 classes). We refer to the 4 possible model and dataset combinations as 4 settings in the following section. The notation we will be using is the following: for a dataset $D$, we train a model $\model_{0}$ on $D$ \varun{dataset $D$ comprises of how many batches? is it $N$?} \anvith{no N is just some number finetuning steps; the number batches can change and isn't actually completely relevant for this I don't think (later when we give specific numbers we mention the epochs of training)} for $T$ training steps (on some batch ordering) to get to model $\model_{T}$. We can represent $\model_{0}$ and $\model_{T}$ by their parameters $w_0$ and $w_{T}$, respectively. The general experimental setup is as follows:
\begin{enumerate}
    \item Pretrain $\model_{0}$ by training $\model_{0}$ using all of $D$ (and not some partition) for N training steps until we reach $\model_{N}$. \varun{what's the difference b/w steps and iterations?} \anvith{no differnce, I'm chaing anywehere interations are mentioned to mean training steps}
    \item Train $\model_{N}$ for some number of finetuning steps $T$ on batches of data $\{x_1,x_2,\dots,x_T\}$ to get $\model_{N+T}$. \varun{is $T<N$?} \anvith{generally yes, but there are some cases we'll put in the appendix where N is 0. I've changed it to just say some number of finetuning steps}
    \item Compute the unlearning error of $M_{N+T}$ starting from $M_N$, i.e compute eq \ref{eq:error bound} except here $w_t$ is the weights of $M_{N+T}$ and $w_{0}$ are the weights of $M_N$ \varun{what has been unlearned in $M_{N+T}$? can you also explain what is being calculated mathematically?} \anvith{unlearning error actually is agnostic of what were unlearning; whatever we unlearn, the metric is the same, so when we compute it we don't unlearn anything, we just preemptively know what our error will be. I've added this to final paragraph in section 3.2 on unlearning error}
\end{enumerate}

\varun{what is the rationale for this setup?} \anvith{added below}
The reasoning for this setup is we want to understand how we can reduce unlearning error, but also be able to see the effect it has on performance; pretrain too much and we'll have converged and there won't be much we can change, pretrain too little and we won't be able to properly guage the impact a method has on performance as the performance will be poor across the board. In the appendix \anvith{@gabe we're putting all the extra results in the appendix right?} \gabe{I want to get Nicolas and Varun's feedback on this. I think to show that we have done our work, let's put it} we've put related results to what we present in this section for different pretraining amount for the interested reader who would like to see this relation.


Depending on the experiment, we compute the unlearning error at regular intervals during the finetuning process or simply record the final error; what we do will be apparent in context and the figure.

\subsection{Pretraining}
\label{ssec:pretraining}
%\anvith{For me: brief blurb on why this should theoretically work, i.e reduce the t}

Recall that Equation~\ref{eq:error bound}, which defines our unlearning error $e$, depends on t, so a simple method to reduce our unlearning error would seem to be simply training for less steps; however this would generally come at a cost to performance, and so an alternative is to simply pretrain on some public dataset that won't need to be unlearned (there is the question of whether such a dataset is available, and we address this and other question in the section for the next method) \varun{is it clear that for all tasks, there exists such a public dataset?} \anvith{nope, hence why we have the latter discussion on the drawbacks (just added this question preemptively now to above)}, and fine-tune on the data that might possibly need to be unlearned (and this fine-tuning will mean less steps on the part of the dataset that needs to be unlearned, so smaller t). However the other variables in $e$ also change with $t$, and so the fact $e$ increases with $t$ isn't self-evident from the formula (as it could be the other variables decrease faster than $t$ increases).

To verify this experimentally, we consider measuring the unlearning error of a model as a function of the number of SGD steps it takes; that is we record the unlearning error at regular intervals during fine-tuning. Specifically, we record the unlearning error of a model over 4000 finetuning steps (i.e $T=4000$). \varun{so does 4000 refer to $T$? in which case, what is the value of $N$?} \anvith{yes to the first, @gabe I can't remember what N is here, for consistency can we do the N=10 epochs} \varun{figure is grey -- make it white?} \anvith{@gabe} \gabe{Fixed, I added in the actual value of N, 15630 in the caption of figure 1.}.

As we see in figure~\ref{fig:unl_t}, the unlearning error does increase with $t$ (practically linearly), and thus by cutting $t$ down with pre-training, we in effect decrease $e$ almost proportionally.

\begin{figure}
    \centering
    \includegraphics[width = 3.2in]{plots/unl_t.png}
    \caption{Unlearning error for 4 different sections as a function of the number of finetuning steps. Across all 4 settings, the unlearning error increases as a function of $t$. Each model was pretrained for 10 epochs with a batch size of 32 (Hence $N = 15630$).}
    \label{fig:unl_t}
\end{figure}

\varun{move discussion below to next subsection} \anvith{done}

%There is one main issue with pretraining, which is that it might not always be possible to pretrain on a public dataset or implement it with the pipeline being used. You also seemingly have to make a big change to get a big decreases in error (i.e training for half as many steps, which could be several thousand steps less, in order to decrease the unlearning error by half). So what follows is our primary contribution to the problem of decreasing unlearning error, a novel loss function that reduces the unlearning error significantly; the benefit of simply having a loss function is it's non-invasive to the pipeline (i.e can be used in practically all scenarios), as it just requires training on it.

\subsection{Standard Deviation Loss}
\label{ssec:std loss}
%\anvith{For me: brief blurb on motivation for the loss, i.e the paper which links it to singular values, introdue the exact formula}


\varun{re-iterate what the downsides were with pre-training; also re-iterate that this is the primary contribution of your work (i.e. new loss function)} \anvith{added to the end of the previous section on pretraining}

There is one main issue with pretraining, which is that it might not always be possible to pretrain on a public dataset or implement it with the pipeline being used. One also has to make a big change to get a big decreases in error (i.e training for half as many steps, which could be several thousand steps less, in order to decrease the unlearning error by half). So what follows is our primary contribution to the problem of decreasing unlearning error, a novel loss function that reduces the unlearning error significantly; the benefit of simply having a loss function is it's non-invasive to the pipeline (i.e can be used in practically all scenarios), as it just requires training on it.

To understand the motivation for this loss function, let's look at the other variables in \ref{eq:error bound} and in particular $\sigma$. Based on the work done by Fort et al.~\cite{fort2019emergent}, it has been seen that various properties of the spectrum of the hessian during training can be accurately modeled by treating the logits of a neural network as zero mean gaussian variables, where the standard deviation grows during training. In particular it was noted that as the standard deviation grows, the top singular value grows to a peak and then goes back down. 

Inspired by this model for the singular values, we propose the \textit{Standard Deviation Loss} (or SD Loss for short) which adds to normal cross entropy loss a regularizing term for the standard deviation of all the logits:

\begin{multline}
\label{eq:SD_Loss}
SDL(\model(x),y) = - \sum_{i=1}^{c} y_{i}\log(\model(x)_{i}) \\ + \gamma~\sqrt{(\sum_{i=1}^{c}(\model(x)_{i}-\mu)^{2})/c}
\end{multline}

where here $c$ is the output dimension, $\gamma$ is the regularization strength, and $\mu$ is the average value of the output logits $M(x)$ for the specific datapoint $x$ \varun{what is $M(x)_i$?, how is $\mu$ calculated? is it the running average or the average for that particular batch of data? $\gamma$ undefined} \anvith{added now to the sentence}. The motivation for this loss is to keep the standard deviation low, and so keep the singular values low and thus reduce the unlearning error. As we'll see shortly, it doesn't actually affect the singular values meaningfully (showing a disparity between the model presented in Fort et al work \cite{fort2019emergent} and what happens in practice, though not contradictory to what they claimed as it was simply a model), but significantly decreases the change in weights during training.

\varun{explain the experimental setup to obtain Fig.~\ref{fig:SD_loss}}\anvith{added below}
To test the effectiveness of the SD Loss, we compute the unlearning error over 8000 finetuning steps (5 epochs) after pretraining 10 epochs (as to reach a suitable accuracy to understand drops to performance though not so much as to have already converged) for different regularization strengths, which are plotted in figure~\ref{fig:SD_loss}, and the final unlearning error and accurcaies of the models trained on Cifar-10 for the various regularization values after training the 15 epochs in total are listed in \ref{tb:SD_loss_unl_err}, and the percent drops are listed in \ref{tb:SD_loss_unl_percent}. 

As we see from figure \ref{fig:SD_loss} strengthening the regularization of SD Loss consistently drops the unlearning error for ResNet-18 and VGG-19 on both Cifar-10 and cifar-100, and we see from table \ref{tb:SD_loss_unl_percent} incurring a $5\%$ drop to accuracy one can drop the unlearning error by roughly $25\%$, and allowing for larger drops to accuracy one can keep dropping the unlearning error; it should be noted that this drop in accuracy is only over 5 epochs (with 15 epochs of total training), and continuing to train we see the effect on performance becomes less. Lastly note the regularization strengths in \ref{fig:SD_loss} were chosen after some hyper parameter tuning (mainly that we need to work on a scale of $5-25$ for CIFAR10 and $50-250$ for CIFAR100), and generally, if you scale the output dimension by say $10$ (i.e from having $10$ outputs to $100$ outputs) you need to also scale the regularization strength accordingly; this makes sense as we divide by c (the output dimension) in eq \ref{eq:SD_Loss}. \varun{why did you choose these particular values?} \anvith{added sentence above}

%However based on \ref{fig:SD_loss} we see for Cifar-100 the SD Loss wasn't able to make a difference; we hypothesize that the large output dimension makes it hard for the SD Loss to optimize, and it's an interesting direction for future work to adapt to build loss functions that work for high dimensional outputs.

Lastly, in attempt to understand what variables our SD Loss is decreasing in order to decrease the unlearning error, we separately computed the singular values \ref{fig:std_sigma} and change in weights \ref{fig:std_delta_weights} for over 16000 finetuning steps for ResNet-18 on CIFAR-10. As mentioned previously and seen in \ref{fig:SD_loss} the SD regularization barely affects the largest singular value, and in fact for large regularization values increases it, despite the original motivation based on Fort et al.~\cite{fort2019emergent} to see if the relation between standard deviation and singular values can be pushed. 

Nevertheless as seen in \ref{fig:std_delta_weights} it decreases the change in weights significantly, which is how it is able to reduce the unlearning error. This loss function may be of interest for other applications where reducing the change in weights is of interest. \anvith{@Gabe hopefully not too hard to find the old results when we tested with l2-regularization} In the appendix we added similar experimental results for ResNet-18 when trained with l2-regularization, and note though it's goal is to reduce the overall magnitude of the weights, it doesn't have a significant impact on the change in weights nor the unlearning error (and in fact increases it).

%that this new loss does significantly decrease the unlearning error as $\gamma$ increases across all 4 settings. Evidently, $\gamma$ must not be too large to not hinder actual learning of the models. Across all 4 settings, we see that we are able to decrease the unlearning error by on average 47.6\% at $\gamma=5.0$ while only decreasing in testing accuracy by X\% (from X\% to X\%). Changes in testing accuracy and unlearning error as a function of $\gamma$ for all 4 settings is shown in table~\ref{table:SD_loss} in appendix~\ref{appendix:A}. These results show that the standard deviation loss is an effective way to decrease the unlearning error while having limited effect on the performance of models.

\begin{figure*}[htp]
  % Fixed length
  \centering
 \subcaptionbox{ResNet18 - CIFAR10\label{fig2:a}}{\includegraphics[width=1.63in]{plots/rolling unlearning error_resnet_cifar10.png}}\hspace{1em}%
  \subcaptionbox{VGG19 - CIFAR10\label{fig2:b}}{\includegraphics[width=1.63in]{plots/rolling unlearning error_vgg_cifar10.png}}\hspace{1em}%
  \subcaptionbox{ResNet18 - CIFAR100\label{fig2:c}}{\includegraphics[width=1.63in]{plots/rolling unlearning error_resnet_cifar100.png}}\hspace{1em}%
  \subcaptionbox{VGG19 - CIFAR100\label{fig2:d}}{\includegraphics[width=1.63in]{plots/rolling unlearning error_vgg_cifar100.png}}
 \caption{Unlearning error of 4 setups trained with the standard deviation loss with increasing levels of SD regularization. Across all 4 setups, a stronger regularization decreases the unlearning error at a (minimal) cost of the performance of the model.}
\label{fig:SD_loss}
\end{figure*}

%Looking specifically at the singular values, we see in figure~\ref{fig:std_sigma} it seems that the largest singular value blows up at the very beginning of training and increases as a function of of the regularization strength. Although this should increase the unlearning error, we see in figure~\ref{fig:std_delta_weights} that the change in weights decreases as a function of the regularization strength. As supported by the values on the y-axis of figure~\ref{fig:std_sigma} and~\ref{fig:std_delta_weights}, the decrease in the change in weights outweights the increase in the largest singular value which results into the net decrease in unlearning error shown in figure~\ref{fig:SD_loss}. This is counterintuivite to our theoertical justification regarding the SD loss which aims at decreasing the largest singular value. However, these results are understandable: sigma is a function of the loss function which means that if we modify the loss function to decrease sigma,sigma will change accordingly. \gabe{I might have worded this wrong. basically this phenomenon appears in physics where the moment you read a measurement from a system, you break the system. In the same vein, if we try to optimize for sigma by changing the loss function, since sigma is a function of the loss function, you have this nested definition which will lead to unintended results}. \anvith{going to go over this once the figures are updated a bit}

\begin{figure}
    \centering
    \includegraphics[width = 3.2in]{plots/sigma_resnet_cifar10.png}
    \caption{Largest Singular value over training for different regularization strengths for ResNet-18 on CIFAR-10}
    \label{fig:std_sigma}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = 3.2in]{plots/delta weights_resnet_cifar10.png}
    \caption{Change in weights over training for different regularization strengths for ResNet-18 on CIFAR-10}
    \label{fig:std_delta_weights}
\end{figure}



%subsection{Evaluating Methods}

%\subsubsection{Pretraining}

    %\anvith{for gabe: basically just show the finetuning results for different models and datasets, i.e that unlearning error increases with t, so clearly having the finetune less steps works}
    
%\anvith{I'll move the discussion for change in weights to the above, ideally here is where you present/explain the experiments and the main takeaways (assuming we are going to present this aspect), for now I've commented it out}

%As the derived unlearning error in equation~\ref{eq:error bound} is a function of the number of SGD steps $t$ and the change in weights $||\mathbf{w}_{t} - \mathbf{w}_{0}||_{2}$, if a model is pretrained for a certain number of steps $N$ on a dataset that is never unlearned, both of these terms will be decreased. It is important that this dataset represents data that will be never be unlearned (ie: could be publicly available data). Pretraining effectively changes the intial weights $\mathbf{w}_{0}$ in  $||\mathbf{w}_{t} - \mathbf{w}_{0}||_{2}$ to $\mathbf{w}_{N}$ if the model was pretrained for $N$ steps. This is because after $N$ steps of pretraining, the pretrained model is much close to it's final minima than the originally initialized weights $\mathbf{w}_{0}$. Additionally, instead of training for a total number of steps $t = T$ and hence needing to consider $T$ steps in the derivation of the unlearning error, pretraining for $N$ steps means that we only need to consider $t = T - N$ steps in the derivation of the unlearning error (ie: $N-T$ is the number of finetuning steps). 

%\gabe{Should I have a paragraph of how pretraining is actually an incredibly common thing in NLP and CV and effectively reduces the individual effect of your small set of private data points by having trained on millions/billions of public data points?}
%\subsubsection{Standard Deviation Loss}

%\anvith{for gabe: basically show the results for SD loss for the different model and datasets, and different settings}

%\anvith{for me and gabe: add some figures showing it does indeed reduce the standard deviation, and if true, show it reduces singular values, and thus supports our hypothetical reasoning}


==> Contents/Unused/6_STD_Loss_mem_inf.tex <==
\section{SD Loss and Membership Inference}
\label{sec:SD_Loss_MI}

%\anvith{present this as a curiosity: does this in fact reduce membership inference, i.e also achieve definition (b)?}

Reflecting on what we're really doing with our SD Loss, we're essentially making all the logits always be very close together (i.e low standard deviation), and so intuitively this might mean that it would be harder for a membership inference attack to work for a model trained with our SD Loss. There is a more mathematical (and less intuitive) reason which we present in the next section relating unlearning error to distribution shifts, but for now the question is, does SD Loss break membership inference attacks?

\varun{i was hoping for one more result, which is implementing a bunch of different unlearning techniques (not sisa, but things like linear filtration) etc. and measuring the unlearning error. is this doable? }
\anvith{It depends, our unlearning error is basically a property of the training procedure, and doesn't change with what people do after the fact, so for all the examples (except for my knowledge dp which does change the training procedure, but I believe we saw it didn't really work @gabe) we'd just be getting the results with sd reg =0, which isn't very interesting. We could possibly mention this somewhere, I could add this to the paragraph in section 3.2 on unlearning error, and state that this is a property of the training procedure, and so if an unlearning method doesn't change the training procedure, they won't have changed the unlearning error. This is not to say those unlearning methods are ineffective, they mostly rely on a different defintion of unlearning or metric, but the main benefit of our work is that our metric is easily computed (and not like DP and KL divergence which need you to use a specific training procedure or retrain several times to get a distribution) and our cheap unlearning procedure can be very effective. I was thinking this is more of a conclusion thing.}

\subsection{Privacy Risk Score}

%Deciding on what membership inference attack to implement, it should be noted that most attack are very specific about what scenarios they can be applied; they often require a high degree of over-fitting \cite{} or sort of analogously training with a small dataset \cite{} to be non-trivially effective (i.e better than $50\%$).

\anvith{@Varun if we agree with the above statement/justification for focusing on privacy risk score I'll find citations} \varun{jump directly to this description + scrap the above.} \anvith{done}

Recently, Song et al \cite{song2021systematic} introduced the privacy risk score, which they showed accurately captures the likelihood a data-point is a training point (i.e has a strong correlation with the likelihood a data-point is a training point). They showed this method works even when the model employs membership inference defences such as Memguard~\cite{jia2019memguard} and Adversarial Regularization~\cite{nasr2018machine}. Fundamentally, the PRS score gives a value between 0 and 1, where 0 (based on their experimental evidence) means not likely to be a training point, and 1 is very likely to be a training point. \varun{you wanna describe how this score should be interpreted i.e. what is a score of 0 mean; what does a score of 1 mean} \anvith{added above}


As seen in figure \ref{fig:Resnet_SD_loss_Priv_Score} and \ref{fig:VGG_SD_loss_Priv_Score} we are able to reproduce the typical behaviour of privacy risk score when training models with typical Cross Entropy Loss \varun{is this the baseline/reference performance?} \anvith{yes, added statement to emphasize this below}, where the fraction of training points increases with the risk score; this serves as our baseline to compare against. As we also see in those figures, when the models are trained with our SD Loss (incurring a marginal drop in accuracy described in table \ref{tb:PRS_SD_Loss} alongside correlation values) the linear relation is broken, and we see that what was once a strong correlation of $1.0$ and $0.8$ for Resnet-18 and VGG-19  respectively with normal Cross Entropy Loss, drops to $0.2$ and $-0.3$ respectively with an SD regularization of just $1.0$.

So we see that our SD loss defends against the privacy risk score. We leave it to future work to test other attacks against it.

\begin{figure*}[htp]
  % Fixed length
  \centering
 \subcaptionbox{ResNet18 - CIFAR10- Regular Loss\label{fig4:a}}{\includegraphics[width=2.63in]{plots/prs_plots/resnet_cifar10_0.0.png}}\hspace{1em}%
  \subcaptionbox{ResNet18- CIFAR10 - SD Loss (reg = 1.0)\label{fig4:b}}{\includegraphics[width=2.63in]{plots/prs_plots/resnet_cifar10_1.0.png}}\hspace{1em}%
  
 \caption{The training fraction as a function of the privacy risk score for ResNet18 trained with and without the SD Loss}
\label{fig:Resnet_SD_loss_Priv_Score}
\end{figure*}

\begin{figure*}[htp]
  % Fixed length
  \centering
 \subcaptionbox{ResNet18 - CIFAR10- Regular Loss\label{fig4:a}}{\includegraphics[width=2.63in]{plots/prs_plots/vgg_cifar10_0.0.png}}\hspace{1em}%
  \subcaptionbox{ResNet18- CIFAR10 - SD Loss (reg = 1.0)\label{fig4:b}}{\includegraphics[width=2.63in]{plots/prs_plots/vgg_cifar10_1.0.png}}\hspace{1em}%
  
 \caption{The training fraction as a function of the privacy risk score for VGG-19 trained with and without the SD Loss}
\label{fig:VGG_SD_loss_Priv_Score}
\end{figure*}

%\anvith{present results for privacy risk score, i.e show we can reproduce it, then show std_loss breaks it}

%\anvith{present results for privacy risk score, i.e show we can reproduce it, then show sd loss breaks it}


\anvith{I've commented out now the label-only part as reproducing seems to not be something I can reasonably get done today... or ever... I'll have to bug Chris a lot more, but that said I think the above is enough to worth mentioning especially since it was a viable attack against previous defences}

%\subsection{Results for Label-only}

%\anvith{present results for label-only attacks, i.e reproduce and break with std loss}

==> Contents/Unused/7_new_anvith.tex <==
%\section{Evaluation of SD loss and Unlearning Error}
\section{Evaluation}

%\anvith{@Nicolas I don't understand exactly what is being said in this paragraph, but I added the enumeration below which hopefully helps}

\varun{@VC: re-write blurb below}
We now evaluate how well our SD loss facilitates approximate unlearning by decreasing the unlearning error. Because we are now evaluating both our unlearning error (i.e., the metric for unlearning) and our SD loss (i.e., the approach to unlearning), we also measure verification error in our experiments. In other words, verification error serves as the ground truth metric, or baseline, because it measures how far our approximate unlearning approach is from exact unlearning through naive retraining. 
%\varun{In this section, we wish to answer the following questions: (1), ... (2),... (3),....}\anvith{done}

In this section, we wish to answer the following questions:
\begin{enumerate}
\itemsep0em
\item Does SD loss decrease unlearning error? 
\item How are the various components of the unlearning error ($t$, $\sigma_{avg}$, $\mathbf{w}_t$) affected by training with SD loss?
%and if so, what variables is it decreasing?
\item Does decreasing unlearning (either by our loss or changing t) mean decreasing unlearning error, that is, is unlearning error a good proxy? \varun{@AT: is this right?}
\end{enumerate}

All of the experiments (including those done in \S~\ref{sec:Strawman Results}) were done using T4 Nvidia GPUs with 16 GB of dedicated memory. We used Intel Xeon Silver 4110 CPUs with 8 cores each and 32GB of Ram. The underlying OS is Ubuntu 18.04.2 LTS 64 bit. We use PyTorch v1.8.1 with CUDA 10.2 and \texttt{python 3.7}. \varun{Our experiments suggest that: <enter summary of results here>}


\varun{move this blurb later}
Furthermore, as we can calculate the unlearning error with respect to different stages of training (which we'll describe shortly), we also illustrate a more nuanced view of how it works during different stages of training (that is with respect to different weights obtained during training); over the first few epochs unlearning error decreases sharply due to the regularization, with the impact for a given regularization value diminishing during the later intervals of training (though by increasing the regularization we can keep decreasing significantly). What this says is that the benefit of training with SD loss is concentrated during the earlier stages of training, with the need for stronger regularization later, a result that can inform how an entity might employ a regularization scheduler during training to maximize performance and unlearning error.

\subsection{SD loss Decreases Unlearning Error}
\label{sec:Evaluating SD loss}

%\anvith{@Nicolas and @Varun: I've revamped this section, but left the old comments though they might be slightly irrelevant now}

%The question we wish to answer here is the following: does SD loss decrease unlearning error, and if so how? What we'll show is that unlike the strawman examples, SD loss does decrease unlearning error, and it does so by decreasing the final change in weights as predicted by our analysis (while not affecting the singular values). 


%\paragraph{Experimental Setup.} Recall that our setup for using SD loss to decrease unlearning error is simply training with it (where the unlearning method then applies to the final weights a gradient update with respect to the initial weights), and in \S~\ref{sec:Strawman Results} we introduced the setup to compute unlearning error. We modify this setup to have an extra variable $N$ so we can control with respect to what weights during training we're computing the unlearning error to understand how the impact changes during training.

Recall that we introduce the SD loss as a method to reduce the unlearning error as training commences. We wish to empirically validate if this occurs. To this end, we utilize the same datasets and model combinations from \S~\ref{}, and the following setup:

\begin{enumerate}
\itemsep0em
\item Train $M_{0}$ on $D$ with SD loss for $N$ training steps to obtain $M_{N}$.
\item Train $M_{N}$ for and additional $t$ steps on batches of data $\hat{\mathbf{x}}_1,\hat{\mathbf{x}}_2,\cdots,\hat{\mathbf{x}}_t$ (from $D$) to get $M_{N+t}$. 
\item Compute the unlearning error (Equation~\ref{eq:unl_err}) of $M_{N+t}$ starting from $M_N$, except here $\weights_t$ is the weights of $M_{N+t}$ and $\weights_{0}$ are the weights of $M_N$.
\end{enumerate}

In this setup, $N$ is a configurable parameter which allows us to understand more fine-grained effects (\S~\ref{}) associated with training with SD loss. We utilize $N=0,10,20,30,40,50$ and regularization strength $\gamma = 0,1,5,10,15,20$ for CIFAR10 and $\gamma = 0,50,100,150,200,250$  for CIFAR100 in our experiments\footnote{$\gamma = 0$ means we just train with CE Loss (which acts as our baseline)}. For the results we discuss, we choose values of $N=10$ epochs (or $\approx 160000$ steps) and $t \approx 8000$ steps, as for smaller values of $N$ (for the fixed value of $t$ we consider), the model does not learn sufficiently. In Figure~\ref{fig:SD_loss}, we plot the unlearning error as a function of training duration $t$. Observe that, as expected, the unlearning error grows as the training duration increases. However, increasing the regularization parameter $\gamma$ (from 0 which is regular CE loss, to $>0$ values which are SD loss) reduces the rate or growth, and the unlearning error. The influence of SD loss on the accuracy of the final model is presented in Table~\ref{tb:SD_loss_unl_err} in Appendix~\ref{}; refer the row for $N=10$. Note that as we increase the value of $\gamma$, the accuracy of the classifier learnt decreases. The decrease is within 5 percentage points for values of $\gamma \leq 5$. For values of $\gamma > 5$, the drop in accuracy is larger. The same results are presented in Table~\ref{tb:SD_loss_unl_percent} (in Appendix~\ref{}) {\em relative} to the baseline ($N=0$ case).


\subsection{An Ablation Study}
%What Variables is SD loss Decreasing?}

%The follow up question is what variables does SD loss change to decrease unlearning error; our analysis of a binary linear classifier predicted it would decrease the final change in weights $||w_t - w_0||_{\ell_2}$, but does this hold for the more general models we now considered?

Recall that the unlearning error is dependent on $t$, $\sigma_{avg}$, $\mathbf{w}_t$, and also the value of $N$. We discuss how these factors influence the unlearning error. As earlier, the results are plotted for $N=10$ epochs, and $t \approx 8000$ steps.

\noindent{\bf Singular Values \& Change in Weights:} The impact of SD loss on $\sigma_{avg}$ and the final change in weights is presented in Figure~\ref{fig:std_delta_weights} and Figure~\ref{fig:std_sigma} respectively. As we see from Figure~\ref{fig:std_sigma}, the impact to the singular values is {\em minimal and not consistent}. After some initial oscillation, SD loss leaves $\sigma_{avg}$ unchanged. From Figure~\ref{fig:std_delta_weights}, we can see that SD loss {\em does decrease} the change in weights $||\mathbf{w}_t - \mathbf{w}_0||_{2}$ significantly, where increasing $\gamma$ consistently decreases $||\mathbf{w}_t - \mathbf{w}_0||_{2}$\footnote{Note that $w_t$ are the weights of the model $M_{N+t}$, and $w_0$ are the weights of the model $M_N$.}.

% So to conclude, how SD loss decreases unlearning error is by decreasing $||w_t - w_0||_{\ell_2}$ while keeping $\sigma_{avg}$ unchanged.
\vspace{1mm}
\noindent{\bf Influence of $N$:} We wish to answer a more nuanced question: {\em how does the impact on SD loss vary as training progresses i.e., as $N$ increases?} The results are presented in Tables~\ref{tb:SD_loss_unl_err} and Table~\ref{tb:SD_loss_unl_percent} in Appendix~\ref{}. We observe that as $N$ increases, the decrease in unlearning error caused by a given regularization diminishes (with the exception of ResNet18 on CIFAR10). For example, looking at VGG19 on CIFAR10 in Table~\ref{tb:SD_loss_unl_percent}, we see with respect to $N=10$ epochs of training, $\gamma=5$ decreases the unlearning error by $20\%$ relative to the baseline ($\gamma=0$). With respect to $N=30$ epochs of training, $\gamma=5$ results in a $4\%$ drop relative to the baseline ($\gamma=0$). \varun{why do we observe this effect?} 

% The exception to this trend is ResNet18 on CIFAR10, which continues to drop unlearning error significantly for the same regularization strength even during the late stages of training (this perhaps speaks to something special about the architecture ans setup which future work might want to look into). 

% Note that performance also degrades with stronger regularization strengths (which allow one to keep dropping unlearning error by more than $50\%$), but the rate at which it does varies with each setup and also the stage of training, speaking to possible hyper parameter tuning or regularization strength scheduling an entity could employ to best maximize performance and unlearning error for a specific model.


%To see how SD loss generalizes for the settings stated in Section~\ref{sec:Strawman Results}, we computed the unlearning error over 8000 finetuning steps (5 epochs) for various amounts of pretraining with different regularization strengths. The final unlearning error and accuracies for all the different setting (pretraining amounts $N=0,10,20,30,40,50$ epochs, and varying regularization strengths) are listed in Table \ref{tb:SD_loss_unl_err}, and the percent drops version of that table is Table \ref{tb:SD_loss_unl_percent}. We plotted the $N=10$ epochs case in Figure~\ref{fig:SD_loss}, as it represents the general impact of the loss function (not so much pretraining as to have already converged, but enough that impacts to performance are noticeable).

%As we see from Figure \ref{fig:SD_loss} strengthening the regularization of SD loss consistently drops the unlearning error for ResNet-18 and VGG-19 on both CIFAR10 and CIFAR100, and we see from Table \ref{tb:SD_loss_unl_percent} incurring a $5\%$ drop to accuracy one can drop the unlearning error by roughly $25\%$ in general for all the settings, and allowing for larger drops to accuracy one can keep dropping the unlearning error. It should be noted that this drop in accuracy is for the $N=10$ epochs case, and continuing to train we see the drop on performance becomes less, which is particularly apparent with ResNet 18 on CIFAR10 as for $N=40$ epochs we can drop unlearning error by $44.61\%$ by only incurring a $0.97\%$ drop to accuracy as seen in Table \ref{tb:SD_loss_unl_percent}. More generally it should be noted that ResNet18 responds better to SD loss than VGG-19 (continuing to drop unlearning error significantly even after large amount of pretraining with little drops to accuracy). \varun{why does resnet respond better? if you can't explain it -- i wouldn't point it out. or provide some theory/guess?} 

%\nj{do you have an intuition/explanation why this is the case?} \anvith{no, we added this remark to the final discussion as it could be that some architectures are just better than others}

%Lastly note the regularization strengths in Figure~\ref{fig:SD_loss} were chosen after some hyperparameter tuning (mainly that we need to work on a scale of $5-25$ for CIFAR10 and $50-250$ for CIFAR100), and generally, if the output dimension scales by say $10$ (i.e., from having $10$ outputs to $100$ outputs) one needs to also scale the regularization strength accordingly; this makes sense as we divide by $c$ (the output dimension) in equation \ref{eq:SD_Loss}. %\varun{why did you choose these particular values?} \anvith{added sentence above}

%However based on \ref{fig:SD_loss} we see for Cifar-100 the SD loss wasn't able to make a difference; we hypothesize that the large output dimension makes it hard for the SD loss to optimize, and it's an interesting direction for future work to adapt to build loss functions that work for high dimensional outputs.
%\nj{suggestion: use Figure~\ref{} instead of \ref{} when you refer to a figure}

%\varun{nicolas is right; this can be made a separate subsection and the corresponding question can be added in the blurb at the beginning of s7; you also want to make "what" you're evaluating for clear (again) -- establish what are the variables that can influence the SD loss and how you plan on measuring these individual effects; also, the choice of $t$ seems to be arbitrary, any particular reason for 16k?; also follow the same protocol to describe the results. this bit is a little thin but we can maybe re-write it more densely after something is written first}

%In an attempt to understand what variables our SD loss is decreasing in order to decrease the unlearning error, we separately computed the singular values (Figure~\ref{fig:std_sigma}) and change in weights (Figure~\ref{fig:std_delta_weights}) for over 16000 finetuning steps for ResNet-18 on CIFAR10. As seen in Figure~\ref{fig:SD_loss} the SD regularization barely affects the largest singular value, and in fact for large regularization values increases it slightly. 

%Nevertheless as seen in Figure~\ref{fig:std_delta_weights} increasing the regularization strength decreases the final change in weights significantly, which is what we predicted in our previous analysis of a binary linear classifer in Section~\ref{sec:A Simple Binary Classifer} and now see generalizes to deep neural networks. This is ultimately how it is able to reduce the unlearning error. This loss function may be of interest for other applications where reducing the final change in weights is of interest.  
%\vspace*{-\baselineskip}

%\varun{scrap below}\anvith{done}
%\paragraph{Conclusion of SD loss} Thus, in constrast to the strawman examples considered in Section~\ref{sec:Strawman Results}, we have that SD loss can reduce $e$ significantly. The reason is that it decreases the final change in weights, with stronger $\gamma$ meaning a stronger drop in change in weights, just as we predicted. 

%\anvith{@varun or @gabe, anyone know how to fix the big gap that appears in the pdf before the paragraph?} \nj{vspace, but leave this as the last thing to do} \gabe{fixed with "\ vspace*{-\ baselineskip}}
%In the appendix we added similar experimental results for ResNet-18 when trained with $\ell_2$-regularization, and note though it's goal is to reduce the overall magnitude of the weights, it doesn't have a significant impact on the change in weights nor the unlearning error (and in fact increases it).
%that this new loss does significantly decrease the unlearning error as $\gamma$ increases across all 4 settings. Evidently, $\gamma$ must not be too large to not hinder actual learning of the models. Across all 4 settings, we see that we are able to decrease the unlearning error by on average 47.6\% at $\gamma=5.0$ while only decreasing in testing accuracy by X\% (from X\% to X\%). Changes in testing accuracy and unlearning error as a function of $\gamma$ for all 4 settings is shown in table~\ref{table:SD_loss} in appendix~\ref{appendix:A}. These results show that the standard deviation loss is an effective way to decrease the unlearning error while having limited effect on the performance of models.
\begin{figure*}[htp]
  % Fixed length
  \centering
  \includegraphics[width=7in]{plots/new_fig10.png}
 \caption{Unlearning error of 4 setups trained with the standard deviation loss with increasing levels of SD regularization. Across all 4 setups, a stronger regularization decreases the unlearning error at a (minimal) cost of the performance of the model. \gabe{@Varun N=10 epochs, T= 5 epochs -> ~7000 steps}}
\label{fig:SD_loss}
\end{figure*}
%Looking specifically at the singular values, we see in figure~\ref{fig:std_sigma} it seems that the largest singular value blows up at the very beginning of training and increases as a function of of the regularization strength. Although this should increase the unlearning error, we see in figure~\ref{fig:std_delta_weights} that the change in weights decreases as a function of the regularization strength. As supported by the values on the y-axis of figure~\ref{fig:std_sigma} and~\ref{fig:std_delta_weights}, the decrease in the change in weights outweights the increase in the largest singular value which results into the net decrease in unlearning error shown in figure~\ref{fig:SD_loss}. This is counterintuivite to our theoertical justification regarding the SD loss which aims at decreasing the largest singular value. However, these results are understandable: sigma is a function of the loss function which means that if we modify the loss function to decrease sigma,sigma will change accordingly. \gabe{I might have worded this wrong. basically this phenomenon appears in physics where the moment you read a measurement from a system, you break the system. In the same vein, if we try to optimize for sigma by changing the loss function, since sigma is a function of the loss function, you have this nested definition which will lead to unintended results}. \anvith{going to go over this once the figures are updated a bit}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{plots/fig8.png}
    \caption{Largest Singular value over training for different regularization strengths for ResNet-18 on CIFAR10 \gabe{@Varun N=10 epochs, T= 5 epochs -> ~7000 steps}}
    \label{fig:std_sigma}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{plots/fig9}
    \caption{Change in weights over training for different regularization strengths for ResNet-18 on CIFAR10 \gabe{@Varun N=10 epochs, T= 5 epochs -> ~7000 steps}}
    \label{fig:std_delta_weights}
\end{figure}
%subsection{Evaluating Methods}
%\subsubsection{Pretraining}

    %\anvith{for gabe: basically just show the finetuning results for different models and datasets, i.e that unlearning error increases with t, so clearly having the finetune less steps works}
%\anvith{I'll move the discussion for change in weights to the above, ideally here is where you present/explain the experiments and the main takeaways (assuming we are going to present this aspect), for now I've commented it out}
%As the derived unlearning error in equation~\ref{eq:error bound} is a function of the number of SGD steps $t$ and the change in weights $||\mathbf{w}_{t} - \mathbf{w}_{0}||_{2}$, if a model is pretrained for a certain number of steps $N$ on a dataset that is never unlearned, both of these terms will be decreased. It is important that this dataset represents data that will be never be unlearned (ie: could be publicly available data). Pretraining effectively changes the intial weights $\mathbf{w}_{0}$ in  $||\mathbf{w}_{t} - \mathbf{w}_{0}||_{2}$ to $\mathbf{w}_{N}$ if the model was pretrained for $N$ steps. This is because after $N$ steps of pretraining, the pretrained model is much close to it's final minima than the originally initialized weights $\mathbf{w}_{0}$. Additionally, instead of training for a total number of steps $t = T$ and hence needing to consider $T$ steps in the derivation of the unlearning error, pretraining for $N$ steps means that we only need to consider $t = T - N$ steps in the derivation of the unlearning error (ie: $N-T$ is the number of finetuning steps). 
%\gabe{Should I have a paragraph of how pretraining is actually an incredibly common thing in NLP and CV and effectively reduces the individual effect of your small set of private data points by having trained on millions/billions of public data points?}
%\subsubsection{Standard Deviation Loss}
%\anvith{for gabe: basically show the results for SD loss for the different model and datasets, and different settings}
%\anvith{for me and gabe: add some figures showing it does indeed reduce the standard deviation, and if true, show it reduces singular values, and thus supports our hypothetical reasoning}

\subsection{Unlearning Error \& Verification Error}
\label{sec:Comparing Unlearning Error and Verification Error}

The question we now wish to answer is whether unlearning error is a good proxy metric for verification error; that is, when we decrease unlearning error by our SD loss or changing t, do we in fact decrease the verification error (i.e, are unlearning error and verification error strongly correlated)? We proceed to do this with an ablation study where we:

\begin{enumerate}
    \item Show that with t as our only variable, unlearning error and verification error are strongly correlated; that is decreasing unlearning error means decreasing verification error
    \item Show that with SD loss regularization strength as our only variable, unlearning error and verification error are strongly correlated
    \item Show that irrespective of architecture and combination of changing t and loss function unlearning error and verification error are correlated
\end{enumerate}

Together these three observations allow us to make the claim that unlearning error truly proxies verification error, and that with little loss to generality we can simply focus on decreasing unlearning error (at least with the methods we discussed and varied).

%Recall that the design of our SD loss was informed by our definition of unlearning error $e$. Having established that the SD loss is effective in decreasing $e$, we now circle back to our original motivation which is to obtain an approximate unlearning approach with minimal verification error; that is our approximately unlearned model should be close from beign a model we could have obtained through naive retraining. We now  confirm that decreasing the unlearning error also decreases the verification error. In particular, we verify that both are correlated through an ablation study which isolates the impact of the number of steps $t$, the regularizer strength $\lambda$, and the model architecture. 

\varun{not clear why you need an ablation study to show the correlation effects. can you make that a bit more precise please?; also, please motivate why you do each of the steps below. what is the hypothesis that you are validating that requires this specific setup?} \anvith{revamped, better?}

% At this point, with our SD loss, we see we can significantly reduce $e$, and similarly we see changing $t$ (i.e., by pretraining) is also a viable option though not ideal. Together these two give us an option to vary the unlearning error and see if reducing unlearning error also reduces verification error (i.e., that they are correlated under these methods), which we proceed to do by an ablation study (controlling our variables). The main takeaway from this section will be that they are indeed strongly correlated, and that when we reduce unlearning error with the methods we've considered we in fact also reduce verification error. This shows unlearning error is a viable alternative to verification error.

\paragraph{Experimental Setup} To test the correlations between unlearning error and verification we need to compute both for a given model; we detailed in \S~\ref{sec:Evaluating SD loss} how we compute unlearning error, and what follows are the additional steps we add on to compute the verification error:

%To experimentally test this we add the following steps to the experimental setup stated in \S~\ref{sec:Evaluating SD loss} to compute the verification error:

\begin{enumerate}
    \item Train $\model_{N}$ for $t-1$ steps on batches $\mathbf{x}_2,\dots,\mathbf{x}_t$. The resulting model is the naively retrained model $M'$ without batch $\mathbf{x}_{1}$, with weights $\weights'$.
    \item Get $M''$, in particular $\weights''$, by our unlearning method:
    $$ \weights'' = \weights_{N+t} + \frac{\eta}{b}\frac{\partial L}{\partial w}|_{\weights_{n+t},x_1}$$ where $\weights_{N+t}$ were the weights of $\model_{N+t}$ from before in \S~\ref{sec:Strawman Results}
    \item Compute the verification error ($||\weights' -\weights''||_{2}$).
\end{enumerate}

\subsubsection{Changing t}

%The main underlying assumption for pretraining is that varying t varies the unlearning error $e$ proportionally; thus, with $t$ being our only variable, we'd like to see that the true discrepency and unlearning error are positively correlated, meaning that with pretraining we are in fact reducing the true discrepency when we are reducing the unlearning error (which is what we can relatively cheaply measure).

What we saw from Figure~\ref{fig:unl_t} is that unlearning error increases with t; the follow up question is now whether verification error does in fact increase with t, or more generally, with t as our only variable, is unlearning error and verification error $||\weights' - \weights''||_{\ell_2}$ correlated.

\varun{here, you want to remind the reader how verification error is computed; also in this setting -- why do you need to pretrain? } \anvith{1) added, 2)don't need to we just did lol, @Gabe can we try a $N=0$ plot, shouldn't make a big difference}

Figure~\ref{fig:pretrain} shows the relationship between the verification error and the unlearning error as a function of the number of SGD steps taken (i.e,\nj{i.e.,}\anvith{done} $t$), for $t=14000$ steps (about 5 epochs) after $N = 80$ epochs of training for ResNet-18 on CIFAR10. The main takeaway here is that the verification error and unlearning error have a strong correlation of $0.9668$, and thus when we reduce the unlearning error by training for less $t$ (say because we pretrained), we reduce the verification error. The choice of $N$ here was arbitrary, and we see similar results for $N = 0$ in Figure~\ref{fig:pretrain} \anvith{@Gabe please add}\gabe{do you mean a second version of figure 7 but with a different pretraining amount in the appendix?}.

%\anvith{reworeded the above based on comments left for old paragraph- commented out below}


%The model is a ResNet-18 pretrained for 80 epochs on CIFAR10 and then performs the experimental steps we've detailed earlier in Sections \ref{sec:Evaluating SD loss},\ref{sec:Comparing Unlearning Error and Verification Error} \nj{broken reference}\anvith{fixed} for $t=14000$ steps, or approximately 5 epochs of training.\gabe{previous sentence is weird, also unsure why there are 2 references to sections}\anvith{yeah, I added some missing words- the two refrences are for the steps in 7.1 and 7.2} The main takeaway here is that the verification error and unlearning error have a strong correlation of $0.9668$, and thus when we reduce the unlearning error by training for less $t$ (say because we pretrained), we reduce the verification error.

%Furthermore, We also see that both verification and unlearning error are a similar function of $t$, and so we can conclude that when varying $t$, if we decrease unlearning error, we also decrease the true discrepancy; thus our assumption for pretraining . 

%\gabe{does this make sense? I think it's poorly worded, need to fix IMO} \anvith{I've reworded it a bit, basically the point is we want to state first the assumption for pretraining was varying t proportionally affect unlearning error, and we want to show that with this as our only variable, we have a strong correlation between verification error and unlearning error, which is what that figure shows; thus we conclude that our assumption for pretraining was correct, and thus pretraining is applicable}.

%\anvith{Slight issue with the below statement is that verification error is the difference between $M''$ and $M$, and so increasing verification error does necessarily mean increasing difference of $M$ and $M'$}

\varun{the phrasing is not the best; also -- zero intuition provided for why the model paths must diverge (this is where you might repeat that analysis you did with nick in the pol paper)} \anvith{honestly I think we can drop the below stuff, I'm commenting it out}
%As another takeaway, these results also agree with the intuition behind why unlearning deep neural networks trained with iterative methods such as SGD is difficult. Even though $\model$ and $\model^{'}$ differ by a single batch, once the differing batch occurs during training, $\model$ and $\model^{'}$ begin to take two different sequences of updates and begin to diverge. As the model trains for more steps, the model is left to continue to diverge further and further, which is shown by the verification error increasing as a function of $t$ (note verification error measures the difference between $M''$ and $M'$, but note $M''$ and $M$ only differ by a constant vector, our unlearning update, so is indicative of an increase in the difference between $M'$ and $M$).

\begin{figure}[h]
  % Fixed length
  \centering
 \includegraphics[width=0.99\columnwidth]{plots/During_training_corr.pdf}
 \caption{Unlearning error and verification error as a function of the finetuning steps (indicated by the color gradient) for ResNet-18 on CIFAR10 for $N=0$ and $N=80$ pretraining amounts. Unlearning error and verification error are measured every 400 and 100 SGD updates for a total of 14000 SGD updates, respectively. The correlation between unlearning error and verification error as a function of $T$ is \textbf{0.934} and \textbf{0.9668},respectively. Both unlearning error and verification error increase as a function of the number of finetuning steps.}
\label{fig:pretrain}
\end{figure}

\subsubsection{Changing SD loss Strength}

\varun{could you explain, with the pearson coefficient values, why the correlation is strong in the text description as well?} \anvith{added}

As seen in Figure~\ref{fig:corr_std_loss} when varying the strength of our SD regularization we have a strong correlation between unlearning error and the verification error for ResNet-18 and VGG-19 on CIFAR10 of 0.96 and 0.81 respectively; in fact for VGG-19 we see the relation between verification error and the regularization is stronger than that for unlearning error (note that as the point get bluer, i.e stronger regularization strength, they constantly decrease on the y-axis where as the x-axis has some noise). \varun{this explanation does not make sense to me; probably because the third axis (strength) is not easy to visualize; do we wanna make the plot a 3d plot?}\anvith{reworded to make a bit clearer- refrenced what you should be looking at- is it better? I think a 3d plot would be a bit much but we can if we want to I think @Gabe}

%Thus the main takeaway here is that only changing the SD regularization, when we decrease the unlearning error we also decrease the verification error, and so we were justified in looking solely at the unlearning error (which is easier to compute).

This is a strong result, as only reasoning with the verification error, it is not clear how one might have come to the SD loss to reduce it. This also shows more generally that the unlearning error accurately proxies the verification error when varying our loss function.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{plots/std_loss_correlation-2.png}
 \caption{Correlation between unlearning error and verification error for ResNet-18 and VGG-19 on CIFAR10 as a function of the regularization strength. The correlations are both high at 0.96 and 0.81 for ResNet-18 and VGG-19, respectively. Notice that the stronger the regularization (more blue) the more the verification and unlearning error decrease in both settings.}
\label{fig:corr_std_loss}
\end{figure}


\subsubsection{Considering all Models}
\label{sec:Considering all Models}

\varun{what are the parameters you vary in fig~\ref{fig:big_final_corr}?} \anvith{@gabe can you add it somewhere in the text: I believe it was just loss, regularization strength, finetuning steps, pretraining amount, model, and datasets}\gabe{Added in the text below, we can be more specific in the appendix if need be}.

\todo{more details please yes. just say range of batch sizes, training amounts. etc}\anvith{@Gabe}\gabe{added as a footnote}
Lastly as seen in Figure~\ref{fig:big_final_corr} where we consider 160 different training setups\footnote{We consider different amounts of pretraining $N = \{10,20, \dots, 80\}$, batch sizes $\{32,64,128\}$,  SD regularization strength (values between the ranges shown in Figure~\ref{fig:SD_loss}), models (ResNet-18 and VGG-19) and batch size over which the Hessian is calculated.} , we see that in general, regardless of architecture, when a model with a specific setup (one of the ones we've been considering) has lower unlearning error, it has lower verification error, as we see by the strong positive correlation between unlearning error and the verification error across the different settings and architecture considered.

The fact that unlearning error is a good proxy for the verification error serves as evidence that the mathematical basis for unlearning error presented in Section~\ref{sec:approximation} holds for the different architectures and datasets we considered---despite the several approximations we made to arrive at the definition of unlearning error. 
Another takeaway from this result, and the fact that the correlations stand across different architectures, is that unlearning error can be used to compare how well different models with potentially different architectures unlearned, leading to the possible study of what architectures unlearn better.\todo{check if true}\anvith{I believe, based on that data, that we can make the stronger claim that it holds across architectures}

\todo{I removed the sentence in the latex comment below this line because I don't see why we are consistently bringing training less longer as a baseline now. it seems like a pretty weak baseline so I don;t think it's worth expanding on it here}\anvith{agreed, only addeed because I though it illustrated how non-trivial being able to make this conclusions across architectures, loss functions, etc is}

% This result is highly non-trivial, as simply using the number of training steps as a proxy for verification error (with the rather intuitive reasoning behind pretraining that error increases with steps), we would not be able to tell if one model had a higher error than another when trained the same number of steps, nor how a loss function might change this error.

%\anvith{@varun added this to reiterate why this works, going back to the opening paragraphs for section 5}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\columnwidth]{plots/final_fig.png}
 \caption{Unlearning and verification error for 160 settings across CIFAR10 and CIFAR100. The correlation between unlearning error and verification error for CIFAR10 and CIFAR100 are \textbf{0.9028} and  \textbf{0.8813}, respectively. Settings trained with SD loss (green) for both datasets have lower unlearning and verification error then those trained with regular cross entropy (red).}
\label{fig:big_final_corr}
\end{figure}

%Where we repeat for different regularization strengths and different $N$\nicolas{first define N , second I thought we were not using pretraining but following still uses it}; our objective is to better understand how our SD loss performs at reducing unlearning when starting from different stages in training. Varying the amount of pretraining done reduces to taking snapshots at different points during training and helps us understand how the dynamics change.


==> Contents/Unused/7_unl_err_is_good.tex <==
\section{Evaluation of SD Loss and Unlearning Error}

% At this point we have a promising method to reduce unlearning error, our SD Loss, though how it generalizes to more general deep neural networks is still up to debate. 
\anvith{@Nicolas I don't understand exactly what is being said in this paragraph, but I added the enumeration below which hopefully helps}
We now evaluate how well our SD loss facilitates approximate unlearning by decreasing the unlearning error. Because we are now evaluating both our unlearning error (i.e., the metric for unlearning) and our SD loss (i.e., the approach to unlearning), we also measure verification error in our experiments. In other words, verification error serves as the ground truth metric, or baseline, because it measures how far our approximate unlearning approach is from exact unlearning through naive retraining. 



\varun{In this section, we wish to answer the following questions: (1), ... (2),... (3),....}\anvith{done}

In this section, we wish to answer the following questions:
\begin{enumerate}
    \item Does SD Loss decrease unlearning error, and if so, what variables is it decreasing?
    \item Does decreasing unlearning (either by our loss or changing t) mean decreasing unlearning error, that is, is unlearning error a good proxy?
\end{enumerate}
%
% We also have yet to verify whether unlearning error truly captures verification error, as it's just an approximation so far. 
% We answer these questions in this following section; 
%To be specific what we show is that
%We now move onto evaluating our method of decreasing unlearning error (our SD Loss) for general neural networks, and then evaluating whether unlearning error is correlated with verification error in the scenarios we've so far considered that do change unlearning error (i.e changing with the strength of our SD regularization or changing by changing $t$). To be specfic we answer the following questions in this section:
%\nj{again you could use \ itemsep0em to save space}
%\begin{itemize}
    %\item the SD Loss effectively reduces unlearning error for the 4 settings we evaluated the strawman examples on in Section \ref{sec:Strawman Results}. This reduction in unlearning error is achieved at a minimal cost to performance for deep neural networks we evaluated.
    %\item Our unlearning error is strongly correlated to verification error as training progresses (i.e., the number of steps $t$ increases). This holds as we vary the strength of our regularization, and the combination of model architectures an dataset.
%\end{itemize}


All of the experiments (including those done in Section \ref{strawman results}) were done using T4 Nvidia GPUs with 16 GB of dedicated memory. We used Intel Xeon Silver 4110 CPUs with 8 cores each and 32GB of Ram. The underlying OS is Ubuntu 18.04.2 LTS 64 bit. We use PyTorch v1.8.1 with CUDA 10.2 and Python 3.7. 

%\nj{this paragraph could go to appendix if you need more space}

\subsection{SD Loss decreases Unlearning Error}
\label{sec:Evaluating SD Loss}

\anvith{below also doesn't make much sense, I'm going to comment out and write a new section 7 where I mainly just change 7.1}
We first evaluate the impact of our SD loss on the different terms defining our unlearning error: most importantly the difference in weights\todo{add latex}\anvith{not sure what add latex means}, but also the singular values.  Unlike the strawman approaches considered previously, we show that the SD loss decreases the difference in weight while keeping other terms (e.g., singular values) mostly constant. Our hypothesis is that SD Loss will decrease unlearning error by decreasing the change in weights (while having little to no impact on the singular values). 





\varun{before you delve into the experimental setup, you might wanna specify what your hypothesis is: this will help you set up why you need to perform pre-training; also remember that $M_0$ was not defined earlier so you got to do it now}

\paragraph{Experimental Setup.} The experimental setup we follow for our SD Loss results is the following:

\begin{enumerate}
\itemsep0em
\item Pretrain $M_{0}$ by training $M_{0}$ using all of $D$ (and not some partition) for $N$ training steps until we reach $M_{N}$.
\item Train $M_{N}$ for $t$ finetuning steps on batches of data $\hat{\mathbf{x}}_1,\hat{\mathbf{x}}_2,\cdots,\hat{\mathbf{x}}_t$ (from $D$) to get $M_{N+t}$.
\item Compute the unlearning error of $M_{N+t}$ starting from $M_N$, i.e., compute Equation~\ref{eq:unl_err} (\varun{not eq 8?})\anvith{fixed to refer to unlearnin error definition} except here $\weights_t$ is the weights of $M_{N+t}$ and $\weights_{0}$ are the weights of $M_N$.
\end{enumerate}

\varun{you wanna highlight the part we discussed; the ambiguity in part stems from the fact that thus far, the concrete mechanism to unlearn has not been discussed i.e., train with SD loss + perform amnesiac style deletion. once this is established, you can argue that pre-training to varying degrees allows you to understand the influence of the error at various stages of the training process. why this knowledge is useful is still unclear to me. also, have you folks thought of a scenario where you pretrain for N epochs with SD loss, and then fine-tune for t epochs with regular cross entropy? or vice-versa? might be good to discuss since the regular loss (CE) might help make up any lost accuracy?}

Where we repeat for different regularization strengths and different $N$\nicolas{first define N , second I thought we were not using pretraining but following still uses it}; our objective is to better understand how our SD Loss performs at reducing unlearning when starting from different stages in training. Varying the amount of pretraining done reduces to taking snapshots at different points during training and helps us understand how the dynamics change.

\paragraph{Results.}\nicolas{ask Varun to help rewrite. ideas our out of order. state high level method of experiment, then go into details of how experiment is ran and results. surface back with takeaways. explore possibility of separating experiment on singular values to another subsection} 

\varun{if you wanna see if SD loss impacts the unlearning error, you should be considering the N=0 case. $N>0$ can be used to dissect the effect of the loss. as NP states earlier, follow this template: (a) recall that the objective of our experiment is to.., (b) to this end, we use the same setup as in \S~\ref{} (datasets used + models used), where we vary the number of training steps $t$ and measure its influence on the unlearning error $e$ (also add discussion of hyperparam tuning here); (c) our results are summarized in fig. observe that (here you can highlight the key observations i should make + the reasons why they occur). also please make the clear distinction between percentage and percentage point -- they are not the same.}
To see how SD Loss generalizes for the settings stated in Section~\ref{sec:Strawman Results}, we computed the unlearning error over 8000 finetuning steps (5 epochs) for various amounts of pretraining with different regularization strengths. The final unlearning error and accuracies for all the different setting (pretraining amounts $N=0,10,20,30,40,50$ epochs, and varying regularization strengths) are listed in Table \ref{tb:SD_loss_unl_err}, and the percent drops version of that table is Table \ref{tb:SD_loss_unl_percent}. We plotted the $N=10$ epochs case in Figure~\ref{fig:SD_loss}, as it represents the general impact of the loss function (not so much pretraining as to have already converged, but enough that impacts to performance are noticeable).

As we see from Figure \ref{fig:SD_loss} strengthening the regularization of SD Loss consistently drops the unlearning error for ResNet-18 and VGG-19 on both CIFAR10 and CIFAR100, and we see from Table \ref{tb:SD_loss_unl_percent} incurring a $5\%$ drop to accuracy one can drop the unlearning error by roughly $25\%$ in general for all the settings, and allowing for larger drops to accuracy one can keep dropping the unlearning error. It should be noted that this drop in accuracy is for the $N=10$ epochs case, and continuing to train we see the drop on performance becomes less, which is particularly apparent with ResNet 18 on CIFAR10 as for $N=40$ epochs we can drop unlearning error by $44.61\%$ by only incurring a $0.97\%$ drop to accuracy as seen in Table \ref{tb:SD_loss_unl_percent}. More generally it should be noted that ResNet18 responds better to SD Loss than VGG-19 (continuing to drop unlearning error significantly even after large amount of pretraining with little drops to accuracy). \varun{why does resnet respond better? if you can't explain it -- i wouldn't point it out. or provide some theory/guess?} 

%\nj{do you have an intuition/explanation why this is the case?} \anvith{no, we added this remark to the final discussion as it could be that some architectures are just better than others}

Lastly note the regularization strengths in Figure~\ref{fig:SD_loss} were chosen after some hyperparameter tuning (mainly that we need to work on a scale of $5-25$ for CIFAR10 and $50-250$ for CIFAR100), and generally, if the output dimension scales by say $10$ (i.e., from having $10$ outputs to $100$ outputs) one needs to also scale the regularization strength accordingly; this makes sense as we divide by $c$ (the output dimension) in equation \ref{eq:SD_Loss}. %\varun{why did you choose these particular values?} \anvith{added sentence above}

%However based on \ref{fig:SD_loss} we see for Cifar-100 the SD Loss wasn't able to make a difference; we hypothesize that the large output dimension makes it hard for the SD Loss to optimize, and it's an interesting direction for future work to adapt to build loss functions that work for high dimensional outputs.
%\nj{suggestion: use Figure~\ref{} instead of \ref{} when you refer to a figure}

\varun{nicolas is right; this can be made a separate subsection and the corresponding question can be added in the blurb at the beginning of s7; you also want to make "what" you're evaluating for clear (again) -- establish what are the variables that can influence the SD loss and how you plan on measuring these individual effects; also, the choice of $t$ seems to be arbitrary, any particular reason for 16k?; also follow the same protocol to describe the results. this bit is a little thin but we can maybe re-write it more densely after something is written first}

In an attempt to understand what variables our SD Loss is decreasing in order to decrease the unlearning error, we separately computed the singular values (Figure~\ref{fig:std_sigma}) and change in weights (Figure~\ref{fig:std_delta_weights}) for over 16000 finetuning steps for ResNet-18 on CIFAR10. As seen in Figure~\ref{fig:SD_loss} the SD regularization barely affects the largest singular value, and in fact for large regularization values increases it slightly. 

Nevertheless as seen in Figure~\ref{fig:std_delta_weights} increasing the regularization strength decreases the final change in weights significantly, which is what we predicted in our previous analysis of a binary linear classifer in Section~\ref{sec:A Simple Binary Classifer} and now see generalizes to deep neural networks. This is ultimately how it is able to reduce the unlearning error. This loss function may be of interest for other applications where reducing the final change in weights is of interest.  
%\vspace*{-\baselineskip}

\varun{scrap below}
\paragraph{Conclusion of SD Loss} Thus, in constrast to the strawman examples considered in Section~\ref{sec:Strawman Results}, we have that SD Loss can reduce $e$ significantly. The reason is that it decreases the final change in weights, with stronger $\gamma$ meaning a stronger drop in change in weights, just as we predicted. 

%\anvith{@varun or @gabe, anyone know how to fix the big gap that appears in the pdf before the paragraph?} \nj{vspace, but leave this as the last thing to do} \gabe{fixed with "\ vspace*{-\ baselineskip}}
%In the appendix we added similar experimental results for ResNet-18 when trained with $\ell_2$-regularization, and note though it's goal is to reduce the overall magnitude of the weights, it doesn't have a significant impact on the change in weights nor the unlearning error (and in fact increases it).
%that this new loss does significantly decrease the unlearning error as $\gamma$ increases across all 4 settings. Evidently, $\gamma$ must not be too large to not hinder actual learning of the models. Across all 4 settings, we see that we are able to decrease the unlearning error by on average 47.6\% at $\gamma=5.0$ while only decreasing in testing accuracy by X\% (from X\% to X\%). Changes in testing accuracy and unlearning error as a function of $\gamma$ for all 4 settings is shown in table~\ref{table:SD_loss} in appendix~\ref{appendix:A}. These results show that the standard deviation loss is an effective way to decrease the unlearning error while having limited effect on the performance of models.
\begin{figure*}[htp]
  % Fixed length
  \centering
  \includegraphics[width=7in]{plots/new_fig10.png}
 \caption{Unlearning error of 4 setups trained with the standard deviation loss with increasing levels of SD regularization. Across all 4 setups, a stronger regularization decreases the unlearning error at a (minimal) cost of the performance of the model.}
\label{fig:SD_loss}
\end{figure*}
%Looking specifically at the singular values, we see in figure~\ref{fig:std_sigma} it seems that the largest singular value blows up at the very beginning of training and increases as a function of of the regularization strength. Although this should increase the unlearning error, we see in figure~\ref{fig:std_delta_weights} that the change in weights decreases as a function of the regularization strength. As supported by the values on the y-axis of figure~\ref{fig:std_sigma} and~\ref{fig:std_delta_weights}, the decrease in the change in weights outweights the increase in the largest singular value which results into the net decrease in unlearning error shown in figure~\ref{fig:SD_loss}. This is counterintuivite to our theoertical justification regarding the SD loss which aims at decreasing the largest singular value. However, these results are understandable: sigma is a function of the loss function which means that if we modify the loss function to decrease sigma,sigma will change accordingly. \gabe{I might have worded this wrong. basically this phenomenon appears in physics where the moment you read a measurement from a system, you break the system. In the same vein, if we try to optimize for sigma by changing the loss function, since sigma is a function of the loss function, you have this nested definition which will lead to unintended results}. \anvith{going to go over this once the figures are updated a bit}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{plots/fig8.png}
    \caption{Largest Singular value over training for different regularization strengths for ResNet-18 on CIFAR10}
    \label{fig:std_sigma}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{plots/fig9}
    \caption{Change in weights over training for different regularization strengths for ResNet-18 on CIFAR10}
    \label{fig:std_delta_weights}
\end{figure}
%subsection{Evaluating Methods}
%\subsubsection{Pretraining}

    %\anvith{for gabe: basically just show the finetuning results for different models and datasets, i.e that unlearning error increases with t, so clearly having the finetune less steps works}
%\anvith{I'll move the discussion for change in weights to the above, ideally here is where you present/explain the experiments and the main takeaways (assuming we are going to present this aspect), for now I've commented it out}
%As the derived unlearning error in equation~\ref{eq:error bound} is a function of the number of SGD steps $t$ and the change in weights $||\mathbf{w}_{t} - \mathbf{w}_{0}||_{2}$, if a model is pretrained for a certain number of steps $N$ on a dataset that is never unlearned, both of these terms will be decreased. It is important that this dataset represents data that will be never be unlearned (ie: could be publicly available data). Pretraining effectively changes the intial weights $\mathbf{w}_{0}$ in  $||\mathbf{w}_{t} - \mathbf{w}_{0}||_{2}$ to $\mathbf{w}_{N}$ if the model was pretrained for $N$ steps. This is because after $N$ steps of pretraining, the pretrained model is much close to it's final minima than the originally initialized weights $\mathbf{w}_{0}$. Additionally, instead of training for a total number of steps $t = T$ and hence needing to consider $T$ steps in the derivation of the unlearning error, pretraining for $N$ steps means that we only need to consider $t = T - N$ steps in the derivation of the unlearning error (ie: $N-T$ is the number of finetuning steps). 
%\gabe{Should I have a paragraph of how pretraining is actually an incredibly common thing in NLP and CV and effectively reduces the individual effect of your small set of private data points by having trained on millions/billions of public data points?}
%\subsubsection{Standard Deviation Loss}
%\anvith{for gabe: basically show the results for SD loss for the different model and datasets, and different settings}
%\anvith{for me and gabe: add some figures showing it does indeed reduce the standard deviation, and if true, show it reduces singular values, and thus supports our hypothetical reasoning}

\subsection{Comparing Unlearning Error and Verification Error}
\label{sec:Comparing Unlearning Error and Verification Error}



Recall that the design of our SD loss was informed by our definition of unlearning error $e$. Having established that the SD loss is effective in decreasing $e$, we now circle back to our original motivation which is to obtain an approximate unlearning approach with minimal verification error; that is our approximately unlearned model should be close from beign a model we could have obtained through naive retraining. We now  confirm that decreasing the unlearning error also decreases the verification error. In particular, we verify that both are correlated through an ablation study which isolates the impact of the number of steps $t$, the regularizer strength $\lambda$, and the model architecture. 

\varun{not clear why you need an ablation study to show the correlation effects. can you make that a bit more precise please?; also, please motivate why you do each of the steps below. what is the hypothesis that you are validating that requires this specific setup?}

% At this point, with our SD Loss, we see we can significantly reduce $e$, and similarly we see changing $t$ (i.e., by pretraining) is also a viable option though not ideal. Together these two give us an option to vary the unlearning error and see if reducing unlearning error also reduces verification error (i.e., that they are correlated under these methods), which we proceed to do by an ablation study (controlling our variables). The main takeaway from this section will be that they are indeed strongly correlated, and that when we reduce unlearning error with the methods we've considered we in fact also reduce verification error. This shows unlearning error is a viable alternative to verification error.

\paragraph{Experimental Setup} To experimentally test this we add the following steps to the experimental setup stated in Section \ref{sec:Evaluating SD Loss} to compute the verification error:

\begin{enumerate}
    \item Train $\model_{N}$ for $t-1$ steps on batches $\mathbf{x}_2,\dots,\mathbf{x}_t$. The resulting model is the naively retrained model $M'$ without batch $\mathbf{x}_{1}$, with weights $\weights'$.
    \item Get $M''$, in particular $\weights''$, by our unlearning method:
    $$ \weights'' = \weights_{N+t} + \eta  \frac{\partial L}{\partial w}|_{\weights_{n+t},x_1}$$ where $\weights_{N+t}$ were the weights of $\model_{N+t}$ from before in Section \ref{sec:Strawman Results}
    \item Compute the unlearning error of $M_{N+t}$ and the verification error ($||\weights' -\weights''||_{2}$).
\end{enumerate}

\subsubsection{Changing t}

%The main underlying assumption for pretraining is that varying t varies the unlearning error $e$ proportionally; thus, with $t$ being our only variable, we'd like to see that the true discrepency and unlearning error are positively correlated, meaning that with pretraining we are in fact reducing the true discrepency when we are reducing the unlearning error (which is what we can relatively cheaply measure).

What we saw from Figure~\ref{fig:unl_t} is that unlearning error increases with t; the follow up question is now whether verification error does in fact increase with t, or more generally, with t as our only variable, is unlearning error and verification error correlated.

\varun{here, you want to remind the reader how verification error is computed; also in this setting -- why do you need to pretrain? }

Figure~\ref{fig:pretrain} shows the relationship between the verification error and the unlearning error as a function of the number of SGD steps taken (i.e,\nj{i.e.,}\anvith{done} $t$), for $t=14000$ steps (about 5 epochs) after $N = 80$ epochs of pretraining for ResNet-18 on CIFAR10. The main takeaway here is that the verification error and unlearning error have a strong correlation of $0.9668$, and thus when we reduce the unlearning error by training for less $t$ (say because we pretrained), we reduce the verification error.

%\anvith{reworeded the above based on comments left for old paragraph- commented out below}


%The model is a ResNet-18 pretrained for 80 epochs on CIFAR10 and then performs the experimental steps we've detailed earlier in Sections \ref{sec:Evaluating SD Loss},\ref{sec:Comparing Unlearning Error and Verification Error} \nj{broken reference}\anvith{fixed} for $t=14000$ steps, or approximately 5 epochs of training.\gabe{previous sentence is weird, also unsure why there are 2 references to sections}\anvith{yeah, I added some missing words- the two refrences are for the steps in 7.1 and 7.2} The main takeaway here is that the verification error and unlearning error have a strong correlation of $0.9668$, and thus when we reduce the unlearning error by training for less $t$ (say because we pretrained), we reduce the verification error.

%Furthermore, We also see that both verification and unlearning error are a similar function of $t$, and so we can conclude that when varying $t$, if we decrease unlearning error, we also decrease the true discrepancy; thus our assumption for pretraining . 

%\gabe{does this make sense? I think it's poorly worded, need to fix IMO} \anvith{I've reworded it a bit, basically the point is we want to state first the assumption for pretraining was varying t proportionally affect unlearning error, and we want to show that with this as our only variable, we have a strong correlation between verification error and unlearning error, which is what that figure shows; thus we conclude that our assumption for pretraining was correct, and thus pretraining is applicable}.

%\anvith{Slight issue with the below statement is that verification error is the difference between $M''$ and $M$, and so increasing verification error does necessarily mean increasing difference of $M$ and $M'$}

\varun{the phrasing is not the best; also -- zero intuition provided for why the model paths must diverge (this is where you might repeat that analysis you did with nick in the pol paper)}
As another takeaway, these results also agree with the intuition behind why unlearning deep neural networks trained with iterative methods such as SGD is difficult. Even though $\model$ and $\model^{'}$ differ by a single batch, once the differing batch occurs during training, $\model$ and $\model^{'}$ begin to take two different sequences of updates and begin to diverge. As the model trains for more steps, the model is left to continue to diverge further and further, which is shown by the verification error increasing as a function of $t$ (note verification error measures the difference between $M''$ and $M'$, but note $M''$ and $M$ only differ by a constant vector, our unlearning update, so is indicative of an increase in the difference between $M'$ and $M$).



\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{plots/VER_VS_UNL_61-2.png}
    \caption{Unlearning error and verification error as a function of the finetuning steps (indicated by the color gradient) for ResNet-18 on CIFAR10. Unlearning error and verification error are measured every 100 SGD updates for a total of 14000 SGD updates. The correlation between unlearning error and verification error as a function of $T$ is \textbf{0.9668}. Both unlearning error and verification error increase as a function of the number of finetuning steps.}
    \label{fig:pretrain}
\end{figure}

\subsubsection{Changing SD Loss Strength}


\varun{could you explain, with the pearson coefficient values, why the correlation is strong in the text description as well?} \anvith{added}

As seen in figure~\ref{fig:corr_std_loss} when varying the strength of our SD regularization we have a strong correlation between unlearning error and the verification error for ResNet-18 and VGG-19 on CIFAR10 of 0.96 and 0.81 respectively; in fact for VGG-19 we see the relation between verification error and the regularization is stronger than that for unlearning error (note the y-axis in \ref{fig:corr_std_loss} (b) continually decreases with the strength of the regularization where as the x-axis has some noise). \varun{this explanation does not make sense to me; probably because the third axis (strength) is not easy to visualize; do we wanna make the plot a 3d plot?}

%Thus the main takeaway here is that only changing the SD regularization, when we decrease the unlearning error we also decrease the verification error, and so we were justified in looking solely at the unlearning error (which is easier to compute).

This is a strong result, as only reasoning with the verification error, it is not clear how one might have come to the SD Loss to reduce it. This also shows more generally that the unlearning error accurately proxies the verification error when varying our loss function.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{plots/std_loss_correlation-2.png}
 \caption{Correlation between unlearning error and verification error for ResNet-18 and VGG-19 on CIFAR10 as a function of the regularization strength. The correlations are both high at 0.96 and 0.81 for ResNet-18 and VGG-19, respectively. Notice that the stronger the regularization (more blue) the more the verification and unlearning error decrease in both settings.}
\label{fig:corr_std_loss}
\end{figure}


\subsubsection{Considering all Models}
\label{sec:Considering all Models}

\varun{what are the parameters you vary in fig~\ref{fig:big_final_corr}?} \anvith{@gabe can you add it somewhere in the text: I believe it was just loss, regularization strength, finetuning steps, pretraining amount, model, and datasets}\gabe{Added in the text below, we can be more specific in the appendix if need be}.

\todo{more details please yes. just say range of batch sizes, training amounts. etc}\anvith{@Gabe}

Lastly as seen in Figure~\ref{fig:big_final_corr} where we consider 160 different training setups (ie: different batch sizes, training amounts, regularization strength(s) etc), we see that in general, regardless of architecture, when a model with a specific setup (one of the ones we've been considering) has lower unlearning error, it has lower verification error, as we see by the strong positive correlation between unlearning error and the verification error across the different settings and architecture considered.

The fact that unlearning error is a good proxy for the verification error serves as evidence that the mathematical basis for unlearning error presented in Section~\ref{sec:approximation} holds for the different architectures and datasets we considered---despite the several approximations we made to arrive at the definition of unlearning error. 
Another takeaway from this result, and the fact that the correlations stand across different architectures, is that unlearning error can be used to compare how well different models with potentially different architectures unlearned, leading to the possible study of what architectures unlearn better.\todo{check if true}\anvith{I believe, based on that data, that we can make the stronger claim that it holds across architectures}

\todo{I removed the sentence in the latex comment below this line because I don't see why we are consistently bringing training less longer as a baseline now. it seems like a pretty weak baseline so I don;t think it's worth expanding on it here}\anvith{agreed, only addeed because I though it illustrated how non-trivial being able to make this conclusions across architectures, loss functions, etc is}

% This result is highly non-trivial, as simply using the number of training steps as a proxy for verification error (with the rather intuitive reasoning behind pretraining that error increases with steps), we would not be able to tell if one model had a higher error than another when trained the same number of steps, nor how a loss function might change this error.

%\anvith{@varun added this to reiterate why this works, going back to the opening paragraphs for section 5}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\columnwidth]{plots/final_fig.png}
 \caption{Unlearning and verification error for 160 settings across CIFAR10 and CIFAR100. The correlation between unlearning error and verification error for CIFAR10 and CIFAR100 are \textbf{0.9028} and  \textbf{0.8813}, respectively. Settings trained with SD loss (green) for both datasets have lower unlearning and verification error then those trained with regular cross entropy (red).}
\label{fig:big_final_corr}
\end{figure}

==> Contents/Unused/new_3_Unlearning_Taxonomy.tex <==
%\section{Unlearning Taxonomy}
\section{Background \& Related Work}
\label{sec:overview_unlearning}

%\anvith{@gabe this is more or less temporary, and you might be able to use this setup to help with the table}

%\varun{introduce the problem of unlearning here (informally) in one or two sentences.}\anvith{added it as a one line thing below}

We begin by discussing the semantics behind unlearning (\S~\ref{sec:define_unlearning}), which deals with the problem of "forgetting" a datapoint $\mathbf{x}^* \in D$ from a model $M$ which trained on it. We proceed to discuss metrics to measure the efficacy of unlearning (\S~\ref{sec:unlearning_metrics}), and methods to achieve them (\S~\ref{sec:unlearning_methods}). %A more exhaustive taxonomy of all the methods is presented in Figure~\ref{fig:unlearning_table}. 

\begin{figure}
    \includegraphics[width = 3.28in]{plots/unlearning_table.png}
    \caption{\varun{make fonts bigger + caption more informative}\anvith{@gabe}Taxonomy of prior work on post-hoc (post-training) approximate (avoiding retraining) unlearning methods. Unlearning methods within these categories are categorized in two ways: (1) What is the definition of unlearning used to motivate the removal of information (horizontal axis)? (2) How is the success of the unlearning method measured (vertical axis)?}
    \label{fig:unlearning_table}
\end{figure}

\subsection{Defining Unlearning}
\label{sec:define_unlearning}

% in this dataset, or more generally a sample of datapoints $\mathbf{\mathbf{x}^*}$ \varun{again, notational confusion. why $\mathbf{x}^*$? can't simply $\mathbf{x}$ suffice?}
% \anvith{I refer to the unlearning data really often so I was thinking in the later presentation it helps to disinguish the unlearning datapoints from the regular datapoints}, and make the according change to our model; what this represents is the responsibility of an entity to uphold an individual's (in the case when data is personal) right to be forgotten from a corporation's dataset, and thus an entity must modify their model to meet this change.

% , and this is what we will call \textit{naive retraining}. \varun{\textit{emphasize} instead of using quotes} 
% \anvith{thanks, changed}

%\varun{such that? maybe use the same definition as in the unlearning paper (SISA paper)} \anvith{I've added a bit above, but what this forgetting is is what the rest of this section is about, which doesn't necessarily align with the final distribution definition stated in SISA as we're for now still leaving open the choice of just forgetting this in the output space}.

Unlearning is the mechanism of \textit{forgetting} a datapoint $\mathbf{x}^*$ from a trained model $M$ such that it is suitably similar to a model trained without $\mathbf{x}^*$. The task now is to define how this forgetting occurs. The naive (but undebatable) approach to unlearning is to simply train another model $M'$ from scratch on $D'= D \textbackslash \mathbf{x}^*$. However the issue with \textit{naive retraining}~\cite{bourtoule2019machine} is the large computational overhead associated with them, i.e retraining, especially for increasingly popular large models, like GPT-3~\cite{brown2020language}. 
% \anvith{any good references to the costs related to big model like GPT-3}, and so an entity stands to expend valuabe computational resources \varun{expend valuable computational resources} \anvith{changed} if they're required to retrain every time and unlearning request is sent to them. 
%In this vain, there is a need for a computationally-efficient manner to unlearn, which naive retraining doesn't provide; this is the motivation for many 
\textit{Approximate unlearning} methods (i.e., methods that do not perform retraining) try to alleviate these cost-related concerns by not requiring retraining, but rather some computationally less expensive operation on the final weights. For example Graves et al.~\cite{graves2020amnesiac} add back training updates to unlearn (which is significantly cheaper than retraining if the entity stores these updates while training). 


%\varun{unclear what you're hoping to communicate with this last sentence; are you going to propose a new measure of cost?} 
% \anvith{yep agreed it was a bit vague, I've changed it to state this is the motivation for approximate unlearning methods, which perhaps is a restatement of the introduction? I think it's needed to flow into the next paragraph and basic classification of approaches. Opinions?}

% We can broadly classify the various approximate unlearning approaches. To do this it helps to work in reference to what we know is a truly unlearned model, the naively retrained model $M'$ as defined earlier. Relative to the ideal unlearned model $M'$, we can define two approaches to defining whether another model $M''$ obtained through some approximate unlearning process from the original model $M$ has truly unlearned a datapoint $\mathbf{x}^*$, alongside the original definition of unlearning in terms of retraining (which we will stop calling naive as various approaches are more sophisticated despite still being retraining):

% \varun{what is the difference b/w $M'$ and $M''$? $M'$ is obtained through retraining, and $M''$ is obtained using some other mechanism? ; why these 3 below?} 
% \anvith{yes to the first (I added an extra word to emphasize $M''$ is from some approximate unlearning process, and the below are how we can define whether $M''$ has unlearned, I'm going to drop the old third one and replace it with the baseline retraining}

%\anvith{so we actually don't give any examples or have any discussion for this third definition, so I think it's a bit useless defining this here, I think it makes more sense, considering SISA, to make the third definition "general retraining methods to provide $M'$"}

%The vast majority of the literature on this topic of unlearning for deep neural networks fall into considering one of these three categories, where the focus on third definition of retraining is to make obtaining $M'$ cheaper. 

\vspace{1mm}
\noindent{\bf A Taxonomy of Approximate Unlearning Approaches:} Broadly speaking, approximate unlearning tries to make the approximately unlearned model $M''$ and the naively retrained model $M'$ as similar as possible. Here, similarity between models broadly falls into two categories: ({\bf D1}) the weights of $M'$ and $M''$ (or distribution of weights) are similar, ({\bf D2}) the distribution of outputs generated by $M'$ and $M''$ are similar\footnote{Note that we discuss different techniques that measure similarity in \S~\ref{sec:unlearning_metrics}.}. However, models are defined by the data they are trained on, and their final weights. For this reason, we focus on the first definition of approximate unlearning in our work, and understanding the impact $\mathbf{x}^*$ has on the final weights.


% Keeping these broad approaches in mind, what follows are metrics and approaches that we categorize as being one of these. 

% \varun{now that we've established these 3 categories, what next?}
% \anvith{just added a sentence setting up the next bit, this was mainly just to introduce the broad definitions to keep in mind as we won't be particularly interested in (b) for reasons described in the next paragraph}.

%and (c) we simply obtain $M'$ from retraining where similarity is measured using a distance metric (refer \S~\ref{sec:unlearning_metrics}). \varun{now that we've established these 3 categories, what next?}

% \varun{i don't understand category 3} 
% \anvith{yeah the third actually does make any sense under approximte unlearning, I originaly had it as basically the three forms of unlearning, but I like this better, it's less redundant; I've commented mention of the 3rd option out} 

% Ideally all three of these categories would be equivalent, but it's clear that two models can have more or less very similar outputs but not be very similar in weights, which is the case when training high accuracy models, where as the opposite direction is more or less true (as having the same weights means the same outputs), though depending on the various local properties around a neighbourhood of the weights of $M'$, the relation may not be perfectly monotonic. The point here is that the first two definitions aren't interchangeable. 
% \varun{on reading this paragraph, i am missing the crux of the discussion. what do you wish to convey?}



%\anvith{below discussion is perhaps a bit too early, I restate this at the beginning of the sgd section so I don't think we need to state this here}

\subsection{Unlearning Metrics} 
\label{sec:unlearning_metrics}

We provide an overview of the main techniques used to measure \textit{similarity} between $M'$ and $M''$ (in the first two definitions provided in \S~\ref{sec:define_unlearning}). This is broadly categorized by the y-axis of Figure~\ref{fig:unlearning_table}.

%we emphasize this now as one of the contributions of our work will be an analysis of what similarity means and how we can quantify it. 

\vspace{1mm}
\noindent{\bf 1. $\ell_2$ Distance (or Verification Error):} For definition ({\bf D1}), a simple metric is the $\ell_2$ distance between the weights of $M'$ and $M''$. However, this first requires computing $M'$ (through naive retraining), which is expensive. Another issue is that it has widely been seen that one can retrain on the same sequence of data from the same initialization and obtain different terminal weights~\cite{jia2021proof} (which is caused by the build up of slight hardware randomnesses); if $M'$ changes each time it is recomputed, it is difficult to use \textit{any} computed $M'$ as a baseline to compute $\ell_2$ distances with respect to. One solution to this issue is to simply look at smaller retraining intervals, or look at an average, or focus on correlations with proxy metrics (such as what we propose in \S~\ref{sec:approximation}).

% \anvith{just us as far as I'm aware}). 
% \varun{how?} 
% \anvith{commented out, main way is to shift away from $\ell_2$ and look at probability distribution similarity, which is the following}


% but other work have found other ways to work with ({\bf D1}), such as the following. \varun{how?} \anvith{reworded, main way is to shift away from $\ell_2$ and look at probability distribution similarity, like the following}

%\anvith{I changed it to be more concrete what exactly the issue is, is it better?}

%So in general one cannot simply blindly compare the $\ell_2$ distance between the weights of $M'$ and $M''$; this will be an issue we address, but let's move on for now.

%and in fact using it to some degree (by acknowledging training is stochastic, though perhaps in additional ways to just random batching), 

\vspace{1mm}
\noindent{\bf 2. KL Divergence:} Bypassing the issue of hardware randomness in training as mentioned above, for definition ({\bf D1}), Golatkar et al.~\cite{golatkar2020eternal} consider measuring the similarity of the weights of $M''$ with respect to a distribution of weights of $M'$. They achieve this by looking at Kullback-Leiber (KL) divergence of the two distributions (as they consider $M''$ as being the result of another stochastic process on the original model $M$). The drawback to this is that explicitly calculating what the KL divergence is, rather than simply using it abstractly to define a forgetting procedure, requires knowing the final distributions of models trained on $D'$ which would involve sampling many final models trained on $D'.

%$, i.e retraining multiple times yourself (at which point you've already obtained $M'$ and naively retrained). \varun{any issues with this form of measurement?} \anvith{not other than explicitly computing what it is isn't cheap- requires getting enough samples of final models to know what the distributions are. Added this above}

%\varun{is the first metric the 2 norm b/w the weights? if so, state that upfront, maybe in bold?}
%\anvith{yes, changed}

% \varun{grammar incorrect} 
% \anvith{omitted that section because I think it wasn't particularly relevant}

\vspace{1mm}
\noindent{\bf 3. Membership Inference (MI):} For definition ({\bf D2}), a standard method used to measure similarity in the outputs between $M'$ and $M''$ is by comparing the MI prediction for $\mathbf{x}^*$ on $M'$. This approach is used by Graves et al.~\cite{graves2020amnesiac} and Baumhauer et al.~\cite{baumhauer2020machine}. The reasoning here is that as $M'$ was properly retrained without $\mathbf{x}^*$, a MI attack (MIA) should return that it was not trained with $\mathbf{x}^*$; if a MIA on $M''$ also consistently outputs that $M''$ was not trained with $\mathbf{x}^*$, then we could say their outputs are similar (in the sense that their output on $\mathbf{x}^*$ are similar enough that the MIA believe $M''$ has not been trained on $\mathbf{x}^*$). However, such approaches are not \textit{precise}: it is possible a MIA will give a false positive that $M'$ had indeed trained on $\mathbf{x}^*$, in which case simply lowering the MI likelihood of $\mathbf{x}^*$ for $M''$ does not necessarily make it resemble $M'$. \varun{@varun: re-write \& condense}

% \varun{what if there are many points that are (a) exactly equal to $\mathbf{x}^*$ or (b) the value of $\mathbf{x}^*$ can be inferred from other points because of correlations in the dataset?} 
% \anvith{added discussion on it, is it better?}

%\anvith{for the following, I've realized it also fall under ({\bf D1}) as the DP like gurantees they give is in terms of the final model returned after training, i.e in the weight space, so I've actually changed this to be about ({\bf D1}) and (b) and commented the old version out; opinions?}

\vspace{1mm}
\noindent{\bf 4. Privacy Leakage:} For definition ({\bf D1}), another common metric for measuring similarity is in terms of privacy leakage~\cite{}: clearly $M'$ leaks no information about $\mathbf{x}^*$ as it was not trained on it, and so the smaller the privacy leakage of $M''$ in terms of its weights (specifically for $\mathbf{x}^*$), the closer $M''$ is to being unlearned; so here similarity between weights is measured in terms of of how little the privacy leakage (however privacy leakage is defined) of $\mathbf{x}^*$ is from $M''$ when looking at the weights. This sort of reasoning about privacy leakage is commonly presented in terms of differentially private learning~\cite{abadi2016deep} through the calculation of the privacy parameter $\varepsilon$, but also in the work of Sekhari et al.~\cite{sekhari2021remember} and Guo et al.~\cite{guo2019certified}.


% \varun{you want to say auditing privacy (or obtaining the privacy parameter $\epsilon$); differential privacy is a general mechanism right?} 
% \anvith{yes you're right, changed the statement to be about privacy leakage, which is what Nicolas referred to in the introduction, is it better?}

\paragraph{Limitations of Membership Inference.}
\label{sec:Limitations of Membership Inference}

\varun{this discussion is neatly captured in the taxonomy of unlearning approaches. why is it repeated here?} \anvith{agreed commenting out some stuff, going to briefly mention again we prefer metrics focus on weights because that's what the influence of $x^*$}
%As is apparent from the previous examples, there is a tension associated with defining what it means to truly unlearn: does it require similarity between the distribution of weights ({\bf D1}) or the distribution of outputs ({\bf D2})? However, note that what is common to both is understanding the effect of a datapoint $\mathbf{x}^*$ on a model trained on it. The effect of $\mathbf{x}^*$ is viewed through its influence on the sequence of training updates, which in turn changes the weights learned. Thus, the change in outputs can be viewed as a byproduct of the change in weights.

%So then does ({\bf D2}) also accurately capture ({\bf D1}) in practice? More specifically, as membership inference is a common metric used to evaluate ({\bf D2}), is membership inference also generally correlated with a metric for ({\bf D1}), say verification error \varun{why this particular metric?}? The choice of focusing on a comparison with verification error will be more apparent later in the section.

As can be seen in Figure \ref{fig:unlearning_table}, membership inference is the most popular metric for unlearning (tied with a general definition of similarity in final weight distributions). However as mentioned in Section \ref{sec:define_unlearning} it's more intuitive to reason with similarity of weights (as that's what defines a model). So the question is whether membership inference is also related to definition ({\bf D1}). 

Instead of now proceeding to compare with every metric we've seen for definition ({\bf D1}), which is broadly speaking metrics for similarity of distribution of final weights, we note that in fact verification error is related to how similar the distribution of final weights are. Intuitively if the average verification error is 0 then that means the distributions of final weights of $M'$ and $M''$ are more or less the same and thus all the other metrics for definition ({\bf D1}) are 0; it is obviously not completely true that if the mean is the same then the distributions are the same, and we elaborate on this relation in Section \ref{sec:define_unlearning}. However for now it's intuitive that average verification error (or more generally correlations with verification error) is the golden standard we can focus on to understand if Membership Inference is at all related to ({\bf D1})

\paragraph{Privacy Risk Score and Verification Error.} \varun{don't talk about how it can alleviate concerns by other methods; the focus of this para should be (a) what is privacy risk score (provide range of values returned), (b) how it relates to metrics for unlearning, (c) what your experimental setup is and what you wish to validate, (d) what the results are and why MI is not a good metric. then, this whole sub-section can be re-cast as follows: (1) introduce other metrics (modulo MI) + \textit{establish why verification error should be the golden standard in a few sentences (add a forward pointer after)}; the emphasized part is essential and is missing right now, (2) talk about MI as a metric for unlearning, (3) talk about why MI is bad} \anvith{agreed; to the brief blrub above I added an emphasis on why we focus on verification error. Below I trimmed it down to follow the outline for this paragraph you gave}

Recently, Song et al.~\cite{song2021systematic} introduced the privacy risk score, which they showed accurately captures the likelihood a data-point is a training point (i.e has a strong correlation with the likelihood a data-point is a training point). Fundamentally, the PRS score gives a value between 0 and 1, where 0 (based on their experimental evidence) means not likely to be a training point, and 1 is very likely to be a training point. This behaves as a membership inference attack which immediately gives to a datapoint $x^*$ a metric (the PRS score) of the attacks success rate on it, i.e this falls under a membership inference metric for unlearning as discussed in Section \ref{sec:unlearning_metrics}.

%They showed this method works even when the model employs membership inference defences such as Memguard~\cite{jia2019memguard} and Adversarial Regularization~\cite{nasr2018machine}. Fundamentally, the PRS score gives a value between 0 and 1, where 0 (based on their experimental evidence) means not likely to be a training point, and 1 is very likely to be a training point. 

%\varun{you wanna describe how this score should be interpreted i.e. what is a score of 0 mean; what does a score of 1 mean} \anvith{added above}

So now to understand the relation between membership inference and verification error (and thus definition ({\bf D!}) we test the correlation between PRS score (a membership inference metric) and verification error after an approximate unlearning method that was originally evaluated on membership inference, in this case Amnesiac Machine Learning as proposed by Graves et al~\cite{graves2020amnesiac}.

%\anvith{@gabe for you to fill once the results are back}

We train triplets of $M$, the naively retrained model $M^{'}$ and the unlearned model $M^{''}$ obtained via Amnesiac Machine Learning (this triplet being that all of them are trained on the same settings) on the CIFAR-10 and CIFAR-100 dataset and obtain many different triplets by changing the training settings (different amounts of training, batch sizes, learning rates etc). For each triplet we measured the privacy risk score of the unlearned point $x^*$ on $M''$ and the verification error $||M'' - M'||_{\ell_2}$, and the plot of the relation between the privacy risk score and verification error is given in Figure~\ref{fig:amnesiac_prs_vs_ver}.

As can be seen in Figure~\ref{fig:amnesiac_prs_vs_ver} there is little to no correlation between privacy risk score and the verification error; this generally shows that membership inference as a metric doesn't always capture definition ({\bf D1}) in the sense that a membership inference attack isn't necessarily correlated with verification error (as we see privacy risk score isn't correlated with verification error). As definition ({\bf D1}) is the stronger definition for unlearning, this shows the limitations with working with membership inference as a metric for unlearning.


%We would expect that a model M that has undergone an unlearning procedure to unlearn data $x^{*}$ whould have a privacy risk score of 0.5 or below, i.e: Membership Inference does not know if it is a training or testing point or thinks it's a testing point. In such a case, we would expect a verification error close to zero. In the case that a data point has not been fully unlearned, the privacy risk score should be slightly above 0.5 (ie: 0.6 or 0.7) and have a non-zero verification error as $M^{'}$ and $M^{''}$ should differ due $\mathbf{x}^*$ not being unlearned in it's entirety. However, in Figure~\ref{fig:amnesiac_prs_vs_ver}, we see that privacy risk score and verification error are not correlated and do not follow this relationship. This results motivates the need for further investigation of unlearning metrics to truly capture unlearning which we will discuss in future sections.

\begin{figure}
    \centering
    \includegraphics[width = 3.2in]{plots/fig2.png}
 \caption{Correlation between privacy risk score and verification error in different training setups for CIFAR10 and CIFAR100. The correlations are -0.29 and -0.02, respectively.}
 \label{fig:amnesiac_prs_vs_ver}
\end{figure}



\subsection{Unlearning Methods}
\label{sec:unlearning_methods}

\varun{@varun: condense}

We turn our attention to the following question: \textit{how exactly does one unlearn}? What follows are some examples. The specific things these approximate unlearning methods change is broadly categorized by the x-axis of Figure~\ref{fig:unlearning_table}

\vspace{1mm}
\noindent{\bf 1. SISA Training:} The SISA framework by Bourtoule et al.~\cite{bourtoule2019machine} works by partitioning the data between different smaller models so that one never has to truly retrain the entire model; only a smaller model is impacted by a request to unlearn a datapoint. This is an example of naive retraining, where the authors still perform retraining to obtain $M'$ from $D'$, but in a cost effective manner.

\vspace{1mm}
\noindent{\bf 2. Scrubbing:} The scrubbing procedure by Golatkar et al.~\cite{golatkar2020eternal} is an example of ({\bf D1}) of approximate unlearning. Here, the authors provide a stochastic method applied to a given $M$ to output a model $M''$ whose weights are in the distribution of the ideal retrained model $M'$, which they accomplished by minimizing a "forgetting Lagrangian" which introduced a weighted term measuring the KL-divergence of the the distribution outputted by this stochastic method and $M'$. 

% \varun{you want to give a little bit more info on the method; look at the explanation for sisa} 
% \anvith{added a bit more}

%the metric they use to measure the discrepancy in the distributions of weights is KL-divergence, as discussed in the previous section. 

% \varun{repetetive; you've explained this before.} \anvith{yep, I commented it out and am just leaving the statement of what they do, before we were talking about how they measure the effectiveness of what they do}

\vspace{1mm}
\noindent{\bf 3. Amnesiac Unlearning:} Amnesiac unlearning~\cite{graves2020amnesiac} works by removing training updates that use $\mathbf{x}^*$ (that is adding back all the gradient updates with $\mathbf{x}^*$ during training) to obtain an unlearnt model $M''$. As a preface, this is quite different from what we'll propose, as all we need is to compute a single gradient update with respect to the initial weights (and train on a specific loss function to get good results) and don't need to store anything but the initial weights, as compared to storing all the updates with amnesiac unlearning. However the idea of adding back gradients (though different gradients in our case) is similar.

% In their work, they measure the effectiveness of this procedure by following ({\bf D2}), by comparing the outputs of MIA on $M''$, however, with the work we will do, we see we can also analyze the effectiveness of this method in terms of the first definition of unlearning. 
% \varun{do they add training updates or remove them?} 
% \anvith{yeah sorry, I was thinking about how you add back gradients, but it's more correct to just say they remove the training updates}

\vspace{1mm}
\noindent{\bf 4. Differentially Private Learning} Lastly, DP naturally allows one to approximately forget a data point by doing nothing as it gives bounds on how indistinguishable a given model is to one not trained on a data point (so is an approximate unlearning method under ({\bf D1}) as we look at the distribution of final models in the weight space). However Sekhari et al.~\cite{sekhari2021remember} show that DP learning only allows one to delete $O(\frac{n}{\sqrt{d}})$ data points while retaining meaningful bounds, and propose an unlearning algorithm for convex and strongly convex losses that improves the number of datapoints one can delete by adding a hessian update and noise to the final weights. 


\subsection{Many Different Metrics}

\varun{1. can you summarize why verification error is the gold standard? so far, i can see (a) simple and intuitive. that's it. everything else is left as a forward pointer, which is not a good idea -- you want to establish it right here (Without too much technical detail); 2. also check for grammar -- it's vs. its } \anvith{1. reworded and added to paragraph 3 to make it clearer why it's the gold standard, 2. fixed (was only in the last paragraph?)}

Looking at the taxonomy, one of the main issues we see is the diversity of different metrics used; it is fair to say the field has diversified into many different branches. It is a benefit for the field to look into relating these metrics in order to understand them holistically, and possibly understand the benefits that one metric might have compared to another.  

From our discussion of Membership Inference and ({\bf D2}) from Section \ref{sec:unlearning_metrics} (one of the current favourite metrics) we see that ({\bf D2}) doesn't imply ({\bf D1}), though the opposite is inherently true (as if the weights of $M''$ approach those of $M'$, so will the outputs under continuity).

So we focus on trying to unify the metrics for ({\bf D1}) and thus all the metrics. The simplest and yet strongest is Verification Error; when we earlier said that ({\bf D1}) implies ({\bf D2}), we're talking about the limit as the verification error approaches 0 (what is used for continuity). Furthermore, as also mentioned in Section \ref{sec:unlearning_metrics} when discussing the limitations of membership inference, we note that if average verification error is 0 then the distirbutions of $M'$ and $M''$ are, informally speaking, practically the same (Section \ref{sec:Focusing on Verification Error} makes this relation, and its dependencies, more explicit). Thus we see verification error captures all the general metrics stated on the y-axis of Figure~\ref{fig:unlearning_table} and can be used as our unifying metric.

%will be showing how verification error also captures differences in distribution of weights between $M''$ and $M'$, unifying the other pursuit others have taken for measuring ({\bf D1}); we also see verification error is important for the concept of a \textit{proof of unlearning}

However verification error has its own issues hindering its use as a metric: it's expensive to compute as it requires computing $M'$ and is subject to the randomness of training. Solving these issues, while also introducing a method to reduce verification error (our standard deviation regularizer) will be the focus of the latter part of the paper, Sections \ref{sec:A Closed Form Approximation of SGD}, \ref{sec:Reducing the Unlearning Error}, \ref{sec:Comparing Unlearning Error and Verification Error}.


%\subsection{TEMPORARY (will migrate after results are added):Issues with Membership Inference}
%\anvith{Emphasizing this is temporary, to be moved to a subsubsection at the end of 3.2 Titled "Limitations of Membership Inference"}
%As is apparent from the previous examples, there is a tension associated with defining what it means to truly unlearn: does it require similarity between the distribution of weights (({\bf D1})) or the distribution of outputs (({\bf D2}))? However, note that what is common to both is understanding the effect of a datapoint $\mathbf{x}^*$ on a model trained on it. The effect of $\mathbf{x}^*$ is viewed through its influence on the sequence of training updates, which in turn changes the weights learned. Thus, the change in outputs can be viewed as a byproduct of the change in weights.

%So then does ({\bf D2}) also accurately capture ({\bf D1}) in practice? More specifically, as membership inference is a common metric used to evaluate ({\bf D2}), is membership inference also generally correlated with a metric for ({\bf D1}), say verification error? The choice of focusing on a comparison with verification error will be more apparent later in the section.

%\subsubsection{Privacy Risk Score and Verification Error}

%Recently, Song et al~\cite{song2021systematic} introduced the privacy risk score, which they showed accurately captures the likelihood a data-point is a training point (i.e has a strong correlation with the likelihood a data-point is a training point). They showed this method works even when the model employs membership inference defences such as Memguard~\cite{jia2019memguard} and Adversarial Regularization~\cite{nasr2018machine}. Fundamentally, the PRS score gives a value between 0 and 1, where 0 (based on their experimental evidence) means not likely to be a training point, and 1 is very likely to be a training point. 

%\varun{you wanna describe how this score should be interpreted i.e. what is a score of 0 mean; what does a score of 1 mean} \anvith{added above}

%We test the correlation between PRS score and verification error after an approximate membership inference attack, in this case amnesiac unlearning as proposed by Graves et al~\cite{graves2020amnesiac}.

%\anvith{@gabe for you to fill once the results are back}

%Experimental Setup:

%Results:





% \varun{more details on how this is achieved} \anvith{added}



%focus on unlearning also by the second definition, however here the focus is how differential private learning (or the adapted version they propose) allows one to delete $\mathbf{x}^*$ (or more generally a number of data points less than some maximum number of delete requests) without needing to do anything under the guarantees of differential privacy. 

% \varun{could you please expand upon the last sentence? also this seems like it was explained earlier ... }
% \anvith{yep agreed again, I just changed to get to the point and say what they're doing at a high level}


%\anvith{as of now doesn't look like we'll do this}
%\subsubsection{The Pros and Cons/A Comparison}

%\anvith{feel free to give this section a better title}

%\anvith{I'll leave this for Gabriel, feel free to also add more methods to the anlysis, I just felt I should stop at one I explained above just because I felt it was a good survey and showcasing more would be for diminishing returns}


==> Contents/Unused/new_6_reducing_unlearning_error.tex <==
\section{Reducing the Unlearning Error}
\label{sec:Reducing the Unlearning Error}

%\anvith{For me: brief blurb on why we want to reduce the unlearning error, i.e to make our method of unlearning more true}

%As we now have a metric capturing the error associated with our unlearning scheme, which is simply adding back the gradient from the first sum in equation \ref{eq:approx}, the question now is whether we can possibly reduce it.

Before getting to our final proposed method at reducing unlearning error, our SD loss, we first go through several examples of methods that don't work (strawman examples) to build understanding for the possible complexities with the problem. These straw man examples are pretraining (which doesn't work for practical reasons), $\ell_2$ regularization, and a \textit{hessian regularizer} (or more properly something that \textit{tries} to regularize the singular values). \varun{introduce these methods in one or two lines.} \anvith{done}

%In section~\ref{ssec:pretraining} and~\ref{ssec:std loss}, we propose two methods to reduce the unlearning error. The following section describes our experimental setup.

\subsection{Strawmen Solutions}

\noindent{\bf 1. Pretraining} Recall that Equation~\ref{eq:error bound}, which defines our unlearning error $e$, depends on $t$, so a simple method to reduce our unlearning error would seem to be training for less steps; however this would generally come at a cost to performance, and so an alternative is to simply pretrain on some public dataset that won't need to be unlearned (there is the question of whether such a dataset is available, and we discuss this issue alongside the results in Section \ref{sec:Strawman Results}) and fine-tune on the data that might possibly need to be unlearned (and this fine-tuning will mean less steps on the part of the dataset that needs to be unlearned, so smaller $t$). However the other variables in $e$ also change with $t$, and so the fact $e$ increases with $t$ isn't completely self-evident from the formula (as it could be the other variables decrease faster than $t$ increases); nevertheless intuitively it make sense to see if training for less $t$ reduces $e$.

\vspace{1mm}
\noindent{\bf 2. $\ell_2$ Regularization} Looking at our definition of unlearning error, Equation \ref{eq:unl_err}, we see it depends on $||\weights_t - \weights_0||_2$; decreasing this (while not changing anything else) would then also decrease the unlearning error $e$. By triangle inequality we have that $||\weights_t - \weights_0||_2 \leq ||\weights_t||_2 + ||\weights_0||_2$, and so it would seem that by decreasing either of those we might be able to push a tighter bound on $||\weights_t - \weights_0||_2$ and decrease it and thus decrease unlearning error. This reasoning motivates using $\ell_2$ regularization which decreases the norm of the final weights $||\weights_t||_2$ by adding a $\lambda||w||_2$ regularization term (where $\lambda$ is a regularization constant) to the typical Cross Entropy Loss.

\vspace{1mm}
\noindent{\bf 3. Hessian Regularization} Another possible way to reduce $e$ would be to reduce $\sigma_{avg}$ while leaving everything else the same (or decreasing them too). Based on the work done by Fort et al \cite{fort2019emergent} and Papyan et al \cite{papyan2019measurements} it has been seen that the spectrum of the hessian is well modeled by the spectrum defined by another matrix which is the sum of conjugation of the hessian of the loss with respect to the logits with different non-square matrices; as the conjugation is with non-invertible matrices, saying the spectrum is left unchanged by conjugation isn't accurate, but we might still wonder if we can simply focus on the hessian of the loss with respect to the logits and try and reduce its singular value which might also reduce the singular values of the hessian with respect to the weights.

On this vein, let $\frac{\partial^2 \mathcal{L}}{\partial^2 \mathbf{z}}$ be the hessian of Cross Entropy loss with respect to the logits $\mathbf{z}$ of the model (before softmax). Note the entries of the hessian are given by $(\frac{\partial^2 \mathcal{L}}{\partial^2 \mathbf{z}})_{ij} = p_i(\delta_{ij} - p_j)$ where $p_i$ is the soft max output of $z_i$, and if the off-diagonal entries are suitably small we can then by the Greshgorin Circle Lemma approximate the spectrum by the set $\{p_1(1-p_1),p_2(1-p_2),\timess,p_c(1-p_c)\}$ where $c$ is the number of classes (i.e the number of outputs).

Building on this we can then try and reduce the magnitude of our approximation of the spectrum terms by adding an $\ell_2$ regularizing term on the approximate spectrum of the loss; in turn this would disproportionately affect the maximum eigenvalue, and thus the first singular value, and would reduce our $\sigma_avg$ and thus our unlearning error (if the approximation is good). The new hessian regularizer is then (where $\lambda$ is the regularization strength):

\begin{multline}
\label{eq:LHCE_Loss}
L_{HCE}(\model(\mathbf{x}),y) = - \sum_{i=1}^{c} y_{i}\log(\model(\mathbf{x})_{i}) + \lambda~||\mathbf{p}(1-\mathbf{p})||_2
\end{multline}




%\subsection{Experimental Setup}
%\label{ssec:experimental setup}


%\varun{1. can we make it $t$ steps instead of $T$? this will also change all the subscripts; 2. all models should be in the math environment (within 2 dollars); 3. the earlier description states that you will perform training for $t$ steps, but step 2 in the setup states that you first train for $N$ steps (make it $n$) and then train for a further $t$ steps? there's a disconnect here; 4. please use the proper subscripts for step 3 i.e. $\mathbf{w}_{n}$ and $\mathbf{w}_{n+t}$; 5. in step 2 -- remove the curly braces around the batches; 6. this setup is good, but it's unclear what you are testing. 6.1 should ideally discuss the intuition behind the strawmen approaches, and 6.2 should begin with a paragraph about the experimental setup (not a subsubsection), and proceed to discuss the results for the previously described strawmen solutions; 7. also this setup seems to be focused towards pretraining. how does it effectively handle the regularization bit?; 8. for the figures: (a) make the legends bigger, make the ticks bigger, remove the box around the legend}
%\anvith{1. yep will do, 2. yep will do, 3. will change the wording, basically we pretrain for $N$ steps (can't be $n$ as that's the variable for the size of the dataset used earlier in the paper) and then only calculate unlearning from $M_N to M_{N+t}$ 4. I believe $\mathbf{w}$ - $\weights$? 5. done 6. will be clearer once I restructure 7. yep will add some details once restructuring (will add a comment that for regularization we repeat for various strengths}

%We investigate unlearning for 2 classic computer vision models, ResNet-18 and VGG-19 on 2 vision datasets, CIFAR10 (10 classes) and CIFAR100 (100 classes). We refer to the 4 possible model and dataset combinations as 4 settings in the following section. The notation we will be using is the following: for a dataset $D$, we first train a model $\model_{0}$ on $D$ for $N$ training steps to obtain $M_N$, and then an additional $t$ training steps to obtain a model $\model_{N+t}$; we compute the unlearning error for training from $\model_N$ to $\model_{N+t}$, where the point of pretraining is generally to achieve a suitable accuracy to see any drops to performance a method may give while not converging so far as to not see any change in weights when training the additional $t$ steps.

%\begin{enumerate}
%\itemsep0em
    %\item Pretrain $\model_{0}$ by training $\model_{0}$ using all of $D$ (and not some partition) for N training steps until we reach $\model_{N}$. %\varun{what's the difference b/w steps and iterations?} \anvith{no differnce, I'm chaing anywehere interations are mentioned to mean training steps}
    %\item Train $\model_{N}$ for some number of finetuning steps $t$ on batches of data $\mathbf{x}_1,\mathbf{x}_2,\dots,\mathbf{x}_t$ to get $\model_{N+t}$. %\varun{is $T<N$?} \anvith{generally yes, but there are some cases we'll put in the appendix where N is 0. I've changed it to just say some number of finetuning steps}
    %\item Compute the unlearning error of $\model_{N+t}$ starting from $\model_N$, i.e compute eq \ref{eq:error bound} except here $\weights_t$ is the weights of $\model_{N+t}$ and $\weights_{0}$ are the weights of $M_N$ %\varun{what has been unlearned in $M_{N+T}$? can you also explain what is being calculated mathematically?} \anvith{unlearning error actually is agnostic of what were unlearning; whatever we unlearn, the metric is the same, so when we compute it we don't unlearn anything, we just preemptively know what our error will be. I've added this to final paragraph in section 3.2 on unlearning error}
%\end{enumerate}

%\varun{what is the rationale for this setup?} \anvith{added below}
%The reasoning for this setup is we want to understand how we can reduce unlearning error, but also be able to see the effect it has on performance; pretrain too much and we'll have converged and there won't be much we can change overall, pretrain too little and we won't be able to properly guage the impact a method has on performance as the performance will be poor across the board. In the appendix we've put related results to what we present in this section for different pretraining amounts for the interested reader who would like to see this relation.

%Depending on the experiment, we compute the unlearning error at regular intervals during the finetuning process or simply record the final error; what we do will be apparent in context and the figure.

\subsection{Strawman Results}
\label{sec:Strawman Results}

\varun{1. can we make it $t$ steps instead of $T$? this will also change all the subscripts; 2. all models should be in the math environment (within 2 dollars); 3. the earlier description states that you will perform training for $t$ steps, but step 2 in the setup states that you first train for $N$ steps (make it $n$) and then train for a further $t$ steps? there's a disconnect here; 4. please use the proper subscripts for step 3 i.e. $\mathbf{w}_{n}$ and $\mathbf{w}_{n+t}$; 5. in step 2 -- remove the curly braces around the batches; 6. this setup is good, but it's unclear what you are testing. 6.1 should ideally discuss the intuition behind the strawmen approaches, and 6.2 should begin with a paragraph about the experimental setup (not a subsubsection), and proceed to discuss the results for the previously described strawmen solutions; 7. also this setup seems to be focused towards pretraining. how does it effectively handle the regularization bit?; 8. for the figures: (a) make the legends bigger, make the ticks bigger, remove the box around the legend}
\anvith{1. yep will do, 2. yep will do, 3. will change the wording, basically we pretrain for $N$ steps (can't be $n$ as that's the variable for the size of the dataset used earlier in the paper) and then only calculate unlearning from $M_N to M_{N+t}$ 4. I believe $\mathbf{w}$ - $\weights$? 5. done 6. will be clearer once I restructure 7. yep will add some details once restructuring (will add a comment that for regularization we repeat for various strengths}

\paragraph{Experimental Setup} We investigate unlearning for 2 classic computer vision models, ResNet-18 and VGG-19 on 2 vision datasets, CIFAR10 (10 classes) and CIFAR100 (100 classes). We refer to the 4 possible model and dataset combinations as 4 settings in the following section. The notation we will be using is the following: for a dataset $D$, we first train a model $\model_{0}$ on $D$ for $N$ training steps to obtain $M_N$, and then an additional $t$ training steps to obtain a model $\model_{N+t}$; we compute the unlearning error for training from $\model_N$ to $\model_{N+t}$, where the point of pretraining $N$ steps is generally to achieve a suitable accuracy to see any drops to performance a method may give while not converging so far as to not see any change in weights when training the additional $t$ steps- in the specific case of checking pretraining, this setup serves the purpose of seeing $e$ increases with $t$.

\begin{enumerate}
\itemsep0em
    \item Pretrain $\model_{0}$ by training $\model_{0}$ using all of $D$ (and not some partition) for N training steps until we reach $\model_{N}$. %\varun{what's the difference b/w steps and iterations?} \anvith{no differnce, I'm chaing anywehere interations are mentioned to mean training steps}
    \item Train $\model_{N}$ for some number of finetuning steps $t$ on batches of data $\mathbf{x}_1,\mathbf{x}_2,\dots,\mathbf{x}_t$ to get $\model_{N+t}$. %\varun{is $T<N$?} \anvith{generally yes, but there are some cases we'll put in the appendix where N is 0. I've changed it to just say some number of finetuning steps}
    \item Compute the unlearning error of $\model_{N+t}$ starting from $\model_N$, i.e compute eq \ref{eq:error bound} except here $\weights_t$ is the weights of $\model_{N+t}$ and $\weights_{0}$ are the weights of $M_N$ %\varun{what has been unlearned in $M_{N+T}$? can you also explain what is being calculated mathematically?} \anvith{unlearning error actually is agnostic of what were unlearning; whatever we unlearn, the metric is the same, so when we compute it we don't unlearn anything, we just preemptively know what our error will be. I've added this to final paragraph in section 3.2 on unlearning error}
\end{enumerate}

%\varun{what is the rationale for this setup?} \anvith{added below}
%The reasoning for this setup is we want to understand how we can reduce unlearning error, but also be able to see the effect it has on performance; pretrain too much and we'll have converged and there won't be much we can change overall, pretrain too little and we won't be able to properly guage the impact a method has on performance as the performance will be poor across the board. In the appendix we've put related results to what we present in this section for different pretraining amounts for the interested reader who would like to see this relation.

Depending on the experiment, we compute the unlearning error at regular intervals during the finetuning process or simply record the final error; what we do will be apparent in context and the figure. Also for the regularizer experiments we repeat the above setup for different values of regularization strength.


\varun{1. all variables you're using should be in the math environment; 2. the first 2 paragraphs of 6.2.1 should ideally be in the revamped 6.1 (explaining the intuition behind pretraining); 3. you'll also wanna briefly explain what $\ell_2$ regularization is when you define it's use as a strawman; 4. there's a broken figure reference for the $\ell_2$ regularization bit; 5. vein not vain; 6. define the HCE loss as $\mathcal{L}_{HCE}$ to be consistent with how loss functions were defined earlier; 7. end section 6.2 with a brief note (3-4 lines) consolidating all the pitfalls you encountered, which further helps motivate the SD loss; 8. i think $M(\mathbf{x})_i$ is undefined?} \anvith{1. done (I think), 2. Moved all the inuition paragraphs for each method to 6.1, 3. done in end of paragraph for it in section 6.1, 4.fixed, 5. fixed, 6. done 7. done}

\anvith{generally speaking should these just be paragraphs? left as subsections for as I don't mind it and I think it makes the seperate sections clearer}

\subsubsection{Pretraining}
\label{ssec:pretraining}
%\anvith{For me: brief blurb on why this should theoretically work, i.e reduce the t}




%Recall that Equation~\ref{eq:error bound}, which defines our unlearning error $e$, depends on t, so a simple method to reduce our unlearning error would seem to be simply training for less steps; however this would generally come at a cost to performance, and so an alternative is to simply pretrain on some public dataset that won't need to be unlearned (there is the question of whether such a dataset is available, and we disucss this and other questions shortly) and fine-tune on the data that might possibly need to be unlearned (and this fine-tuning will mean less steps on the part of the dataset that needs to be unlearned, so smaller t). However the other variables in $e$ also change with $t$, and so the fact $e$ increases with $t$ isn't self-evident from the formula (as it could be the other variables decrease faster than $t$ increases).

To verify our hypothesis that $e$ increases with $t$ experimentally, we consider measuring the unlearning error of a model as a function of the number of SGD steps it takes; that is following the experimental setup stated earlier we record the unlearning error at regular intervals during fine-tuning. Specifically, we record the unlearning error of a model over 4000 finetuning steps (i.e $t=4000$).

As we see in Figure~\ref{fig:unl_t}, the unlearning error does increase with $t$ (practically linearly), and thus by cutting $t$ down by pre-training more, we in effect decrease $e$ almost proportionally.

\begin{figure}
    \centering
    \includegraphics[width = 3.2in]{plots/unl_t.png}
    \caption{Unlearning error for 4 different sections as a function of the number of finetuning steps. Across all 4 settings, the unlearning error increases as a function of $t$. Each model was pretrained for 10 epochs with a batch size of 32 (Hence $N = 15630$).}
    \label{fig:unl_t}
\end{figure}


There is one main issue with pretraining, which is that it might not always be possible to pretrain on a public dataset or implement it with the pipeline being used. One also has to make a big change to get a big decreases in error (i.e training for half as many steps, which could be several thousand steps less, in order to decrease the unlearning error by half). These issues will be resolved with our later SD Loss.

\subsubsection{$\ell_2$ Regularization}

%Adding $\ell_2$ regularization (also known as weight decay) to your loss function minimizes the norm of the learned parameters of your model. A stronger $\ell_2$ regularization results into the weights being less likely to have very large values. In the unlearning error framework, this translates to decreasing $||M_{T}-M_{0}||_{2}||$ as the final weights will diverge less from the original weights that are initialized to small values. To verify this experimentally, we measure unlearning error over a fixed interval of training for different $\ell_2$ regularization strengths shown in figure~\ref{fig:l2_loss}. Contrary to our intuition, although the change in weights does indeed decrease, the singular values actually increase, resulting into the overall unlearning error not decreasing with increased $\ell_2$ regularization strength.

%Looking at our definition of unlearning error, Equation \ref{eq:unl_err}, we see it depends on $||\weights_t - \weights_0||_2$; decreasing this (while not changing anything else) would then also decrease the unlearning error $e$. By simple triangle inequality we have that $||\weights_t - \weights_0||_2 \leq ||\weights_t||_2 + ||\weights_0||_2$, and so it would seem that by decreasing either of those we might be able to push a tighter bound on $||\weights_t - \weights_0||_2$ and decrease it and thus decrease unlearning error. This reasoning motivates using $\ell_2$ regularization, which decreases the norm of the final weights $||\weights_t||_2$, to try an decrease the unlearning error.

Following the setup described earlier, in Figure \ref{fig:l2_loss} we tracked the unlearning error for X\anvith{@gabe what's the # of finetuning steps for the figure} number of finetuning steps for the 4 settings, with various strengths of $\ell_2$ regularization. As can be seen there was no consistent benefit to employing the loss, and in most cases it in fact increased the unlearning error (with the exception of Resnet on CIFAR-10 that saw a modest benefit for $\lambda = 0.1$).

Fundamentally the main issue is that the bound $||\weights_t - \weights_0||_2 \leq ||\weights_t||_2 + ||\weights_0||_2$ is very loose and we can decrease the right hand side without decreasing the left hand-side (the part which we're interested in), which illustrated in Figure~\ref{fig:delta_w_sigma_ell_2} where we see for most of the regularization values we make no impact to the change in weights (or in fact increase the change in weights). So to conclude $\ell_2$-regularization doesn't reduce unlearning error.

\begin{figure}
    \centering
    \includegraphics[width = 3.2in]{plots/fig4.png}
 \caption{Change in weights and singular values during training for different strengths of $\ell_2$ regularization for ResNet18 trained on CIFAR-10}
\label{fig:delta_w_sigma_ell_2}
\end{figure}


%\anvith{@gabe to add once we get all the results- currently have results for resnet cifar10}\gabe{see new figure~\ref{fig:l2_loss}}.
\begin{figure*}[htp]
  % Fixed length
  \centering
  \includegraphics[width=7in]{plots/l2_unl_error_4_plots.png}
 \caption{Unlearning error of 4 setups trained with weight decay ($\ell_2$ regularization) with increasing strength of weight decay. As shown, weight decay does not decrease the unlearning error consistently.}
\label{fig:l2_loss}
\end{figure*}

\subsubsection{Hessian Regularization}

%Another possible way to reduce $e$ would be to reduce $\sigma_{avg}$ while leaving everything else the same (or decreasing them too). Based on the work done by Fort et al \cite{fort2019emergent} and Papyan et al \cite{papyan2019measurements} it has been that the spectrum of the hessian is well modeled by the spectrum defined by another matrix which is the sum of conjugation of the hessian of the loss with respect to the logits with different non-square matrices; as the conjugation is with non-invertible matrices, saying the spectrum is left unchanged by conjugation isn't accurate, but we might still wonder if we can simply focus on the hessian of the loss with respect to the logits and try and reduce its singular value which might also reduce the singular values of the hessian with respect to the weights.

%On this vain, let $\frac{\partial^2 \mathcal{L}}{\partial^2 \mathbf{z}}$ be the hessian of Cross Entropy loss with respect to the logits $\mathbf{z}$ of the model (before softmax). Note the entries of the hessian are given by $(\frac{\partial^2 \mathcal{L}}{\partial^2 \mathbf{z}})_{ij} = p_i(\delta_{ij} - p_j)$ where $p_i$ is the soft max output of $z_i$, and if the off-diagonal entries are suitably small we can then by the Greshgorin Circle Lemma approximate the spectrum by the set $\{p_1(1-p_1),p_2(1-p_2),\timess,p_c(1-p_c)\}$ where $c$ is the number of classes (i.e the number of outputs).

%Building on this we can then try and reduce the magnitude of our approximation of the spectrum terms by adding an $\ell_2$ regularizing term to the loss; in turn this would this would disproportionately affect the maximum eigenvalue, and thus the first singular value, and would reduce our $\sigma_avg$ and thus our unlearning error (if the approximation is good). The new hessian regularizer is then (where $\lambda$ is the regularization strength):

%\begin{multline}
%\label{eq:LHCE_Loss}
%LHCE(\model(\mathbf{x}),y) = - \sum_{i=1}^{c} y_{i}\log(\model(\mathbf{x})_{i}) + \lambda~||\mathbf{p}(1-\mathbf{p})||_2
%\end{multline}

Once again following the setup described in section \ref{ssec:experimental setup}, in Figure \ref{fig:hessian_loss} we tracked the unlearning error for X \anvith{@gabe what's # of finetuning steps- change X accordingly} number of finetuning steps for the 4 settings, with various strengths of hessian regularization. Once again we see that it had no consistent affect on the unlearning error, leaving it unchanged or larger except for ResNet18 on CIFAR-10 which for a couple setting saw a modest decrease.

The main issue here is that realistically one approximation (if not all to some degree) was too loose or not properly linked to what we're interested in, the largest singular value; the fact the regularizer does not in fact reduce the singular values is illustrated in Figure~\ref{fig:delta_w_sigma_hessian} where we see changing the strength of the regularizer has no consistent affect. Future work might be able to improve this line of reasoning to reduce the singular values, however we conclude that our hessian regularizer does not consistently affect unlearning error \footnote{The fact that both $\ell_2$ Regularization and the hessian regularizer were able to reduce unlearning error for ResNet18 on Cifar-10 for a couple setting perhaps indicates that there might be something special about this setting worth being investigated more}.

\begin{figure}
    \centering
    \includegraphics[width = 3.2in]{plots/fig6.png}
    \caption{Change in weights and singular values during training for different strengths of hessian regularization for ResNet18 trained on CIFAR-10}
\label{fig:delta_w_sigma_hessian}
\end{figure}


%\gabe{I know we have written in the past the intution behind Hessian regularization. Do we want to use that or a shorter (less mathematical version?}\anvith{I'm going to explain the main is about a paragraph, shouldn't be too bad}
%\anvith{@gabe to add once we get all the results- currently have results for resnet cifar10}\gabe{see new figure~\ref{fig:hessian_loss}}.
\begin{figure*}[htp]
  % Fixed length
  \centering
  \includegraphics[width=7in]{plots/hessian_loss_unl_results.png}
 \caption{Unlearning error of 4 setups trained with the Hessian loss with increasing levels of hessian regularization. As shown, despite the hessian loss function aims to decrease the largest singular value, the unlearning error does not decrease, in certain scenarios it even increases.}
\label{fig:hessian_loss}
\end{figure*}

%So what follows is our primary contribution to the problem of decreasing unlearning error, a novel loss function that reduces the unlearning error significantly; the benefit of simply having a loss function is it's non-invasive to the pipeline (i.e can be used in practically all scenarios), as it just requires training on it.

%There is one main issue with pretraining, which is that it might not always be possible to pretrain on a public dataset or implement it with the pipeline being used. You also seemingly have to make a big change to get a big decreases in error (i.e training for half as many steps, which could be several thousand steps less, in order to decrease the unlearning error by half). So what follows is our primary contribution to the problem of decreasing unlearning error, a novel loss function that reduces the unlearning error significantly; the benefit of simply having a loss function is it's non-invasive to the pipeline (i.e can be used in practically all scenarios), as it just requires training on it.

\subsubsection{Conclusions from Strawman Examples}

To summarize, one thing we want a proposed method to reduce unlearning error to be is non-invasive to the training pipeline (this is where pretraining fails). Looking at a loss function solves the issue of being non-invasive as all it requires is an entity to train with it, however as we saw a common regularizer ($\ell_2$ regularization), despite being able to reduce bounds on the change in weights, doesn't in fact reduce the change in weights (as this bound can be very loose) and thus doesn't make any difference to $e$. Similarly our attempt to try and reduce singular values to reduce $e$ was not fruitful, despite having some intuition behind it.

This motivates our main contribution to this problem, a loss function that does in fact reduce the unlearning error (our SD Loss).

%some of the highlighted issues with the previous examples: we'd like a method that doesn't require access to public datasets and generally is non-invasive to the training procedure, and general bounds and approximations don't always work (either because they're too loose or the approximation/justification, though intuitive, is wrong). The 

\subsection{Our Proposal: Standard Deviation Loss}
\label{ssec:std loss}

\varun{1. ensure that the terminology used is consistent -- weights have a different variable here; 2. highlight that this subsection is one of your main contributions in this work}
\anvith{1. I've changed it so $\weights$ refers to the whole matrix and $\weights_1$ and $\weights_2$ are as before- row vectors, 2. I think done in the last sentence of the conclusion for 6.2 (section 6.2.4); reiterated that our solution below is our main contribution to this problem}


Our solution to reducing the unlearning error, which is our main contribution to this problem, is to introduce a standard deviation regularizer on the logits outputted by the model, which effectively reduces the change of weights during training and thus the unlearning error. To be precise, our SD Loss is:

\begin{multline}
\label{eq:SD_Loss}
\mathcal{L}_{SD}(\model(\mathbf{x}),y) = \\
- \sum_{i=1}^{c} y_{i}\log(\model(\mathbf{x})_{i}) + \gamma~\sqrt{(\sum_{i=1}^{c}(\model(\mathbf{x})_{i}-\mu)^{2})/c}
\end{multline}

where here $c$ is the output dimension of the model $M $\varun{of what?}\anvith{done}, $\gamma$ is the regularization strength, and $\mu$ is the average value of the output logits $\model(\mathbf{x})$ for a specific datapoint $\mathbf{x}$ (note $\model(\mathbf{x})_i$ is the ith output logit). 

We first illustrate why this works by studying analytically the case of a binary linear classifier (i.e a linear model with just two outputs) training to minimize its loss on a single datapoint; we show how it reduces the minimum distance (in the weight space) to the minimum of the loss (which is where the final weights end up), and so assuming SD Loss doesn't increase singular values, it should reduce unlearning error as we have a smaller $||w_t - w_0||_{\ell_2}$ . We then empirically show how this result generalizes to the 4 settings stated in Section \ref{sec:Strawman Results}.


%\varun{what is $\model(\mathbf{x})_i$?, how is $\mu$ calculated? is it the running average or the average for that particular batch of data? $\gamma$ undefined} \anvith{added now to the sentence}.

%\label{ssec:std loss}
%\anvith{For me: brief blurb on motivation for the loss, i.e the paper which links it to singular values, introdue the exact formula}


%\varun{re-iterate what the downsides were with pre-training; also re-iterate that this is the primary contribution of your work (i.e. new loss function)} \anvith{added to the end of the previous section on pretraining}

\subsubsection{A Simple Binary classifier}
\label{sec:A Simple Binary Classifer}

Let us consider the specific setup where $\mathbf{x}$ is a vector of length $k$ representing a datapoint, $\weights = \begin{bmatrix} \weights_1 \\ \weights_2 \end{bmatrix}$ is a $2{\times}k$ weight matrix, and $M$ is a linear model with two outputs defined by $M(\mathbf{x}) = W\mathbf{x}$. For the sake of simplicity (and without loss of generality) let us assume the label of $\mathbf{x}$ is $0$ (i.e is the first output). Then the SD loss of our model, where $a = \model(\mathbf{x})_1$ and $b = \model(\mathbf{x})_2$ (i.e the first and second output), is:

\begin{multline}
\label{eq:sd_loss_binary}
    \mathcal{L}_{SD}\model(\mathbf{x}),0) = -\log(\frac{e^a}{e^a + e^b}) + \gamma~\sqrt{\frac{a^2+b^2-0.5(a+b)^2}{2}}
\end{multline}

Where the second term is just a simplified version of the standard deviation.

The main empirical observation is the following: increasing the strength of $\gamma$ moves the minimum of this loss (a function of the two outputs $a$ and $b$) closer to the line defined by $a=b$. This is illustrated in Figure \ref{fig:SD_loss_landscape_1} and Figure \ref{fig:SD_loss_neg_grads} which both illustrate how the minimum of the loss approaches the line $a=b$ (black in both figures), and generally how the minimum is defined by a line $a=b + \epsilon$ where $\epsilon$ decreases with the strength of $\gamma$.

We now proceed to analytically show how SD Loss reduces the minimum change in weights required to reach a minimum of the loss. In particular we focus on the initialization of $\weights$ by a constant (that is all the entries are the same), and thus $a_0=b_0$. More generally starting at any state such that $a_0 = b_0$ works for the below, and the analysis has implications for just being close to such a state (i.e starting with low logit standard deviation which is typical in training) as we show that the minimum is found somewhere on a sphere around the initial weights whose radius decreases with $\gamma$.

\varun{what happens to $a_0$ and $b_0$ in the equations below?}\anvith{they cancel, added a line stating this}

To find the minimum distance to a minimum  we need to solve the constrained optimization problem 

\begin{equation}\label{eq1}
  \begin{gathered}
    \min_{\mathbf{u}_1,\mathbf{u}_2} ||\mathbf{u}_1||_2^2 + ||\mathbf{u}_2||_2^2    \\
    \text{subject to} \\
    a_0 + \mathbf{u}_1 \times \mathbf{x} = b_0 + \mathbf{u}_2 \times \mathbf{x} + \epsilon \\
    \implies (\mathbf{u}_1 - \mathbf{u}_2) \cdot \mathbf{x} - \epsilon = 0
  \end{gathered}
\end{equation}

where $\mathbf{u}_1$ and $\mathbf{u}_2$ are the updates to $\weights_1$ and $\weights_2$ respectively to reach the minimum; note that in the equation defining the constraint (which is the equation defining the minimum), $a_0$ and $b_0$ cancelled as we assume they are equal.

The solution, given by minimizing the lagrangian $\mathfrak{L} = \mathbf{u}_1 \times \mathbf{u}_1 + \mathbf{u}_2 \times \mathbf{u}_2 + \lamda((\mathbf{u}_1 - \mathbf{u}_2) \times \mathbf{x} - \epsilon)$, is $\mathbf{u}_1 = \frac{\epsilon}{2||\mathbf{x}||_2^2}\mathbf{x}$ and $\mathbf{u}_2 = \frac{-\epsilon}{2||\mathbf{x}||_2^2}\mathbf{x}$. 

Note that $||\mathbf{u}_1||_2^2 + ||\mathbf{u}_2||_2^2 = \frac{\epsilon^2}{2} ||\mathbf{x}||_2^2$ and thus by reducing $\epsilon$ we reduce the magnitude of the change of weights needed to reach a minimum. As increasing the strength of our SD Loss regularization $\gamma$ does just that, we see that increasing $\gamma$ means decreasing the minimum change in weights needed to reach a minimum (which is what the path following negative gradients approximates).

So if the SD Loss doesn't also increase the singular values (something we'll see shortly), we see that for this model the SD Loss decreases unlearning error.




\begin{figure*}[htp]
  % Fixed length
  \centering
 \subcaptionbox{SD Loss reg=0.01 \label{fig2:a}}{\includegraphics[width=1.63in]{plots/SD_Loss_landscape/SD_landscape_0.01.png}}\hspace{1em}%
   \subcaptionbox{SD Loss reg=0.1 \label{fig2:a}}{\includegraphics[width=1.63in]{plots/SD_Loss_landscape/SD_landscape_0.1.png}}\hspace{1em}%
   \subcaptionbox{SD Loss reg=1 \label{fig2:a}}{\includegraphics[width=1.63in]{plots/SD_Loss_landscape/SD_landscape_1.png}}\hspace{1em}%
   \subcaptionbox{SD Loss reg=5 \label{fig2:a}}{\includegraphics[width=1.63in]{plots/SD_Loss_landscape/SD_landscape_5.png}}\hspace{1em}%
 \caption{Plots of the SD Loss landscape with respect to the two outputs ($a = out 1$, $b= out 2$). Note the black dot represents where $a=b$, and observe how the minimum of the loss landscape approaches the black dot}
\label{fig:SD_loss_landscape_1}
\end{figure*}

\begin{figure*}[htp]
  % Fixed length
  \centering
 \subcaptionbox{SD Loss reg=0.01 \label{fig2:a}}{\includegraphics[width=1.63in]{plots/SD_Loss_landscape/neg_grads_sd_0.01.png}}\hspace{1em}%
   \subcaptionbox{SD Loss reg=0.1 \label{fig2:a}}{\includegraphics[width=1.63in]{plots/SD_Loss_landscape/neg_grads_sd_0.1.png}}\hspace{1em}%
   \subcaptionbox{SD Loss reg=1 \label{fig2:a}}{\includegraphics[width=1.63in]{plots/SD_Loss_landscape/neg_grads_sd_1.png}}\hspace{1em}%
   \subcaptionbox{SD Loss reg=5 \label{fig2:a}}{\includegraphics[width=1.63in]{plots/SD_Loss_landscape/neg_grads_sd_5.png}}\hspace{1em}%
 \caption{Plots of the negative gradients of SD Loss with respect to the two outputs ($a = out 1$, $b= out 2$). Note the black line represents where $a=b$, and observe how the minimum of the loss landscape (where the arrows switch direction) approaches the black dot}
\label{fig:SD_loss_neg_grads}
\end{figure*}

%\subsubsection{Experimental Verification}

%\varun{1. compare this with your prior approaches to highlight how good/bad it is?; 2. when you're referring to a figure, use the word "Figure" and not just the wreference; 3. } \anvith{1. done (added a brief paragraph to the end of 6.3.2, and the first line is simply that this actually reduces unlearning error compared to the strawman examples), 2. done}

%To see how SD Loss generalizes for the settings stated in Section~\ref{sec:Strawman Results}, we computed the unlearning error over 8000 finetuning steps (5 epochs) after pretraining 10 epochs (as to reach a suitable accuracy to understand drops to performance though not so much as to have already converged) for different regularization strengths, which are plotted in Figure~\ref{fig:SD_loss}. The final unlearning error and accuracies of the models trained on Cifar-10 for the various regularization values at the end of the finetuning are listed in Table \ref{tb:SD_loss_unl_err}, and the percent drops are listed in Table \ref{tb:SD_loss_unl_percent}. 

%As we see from Figure \ref{fig:SD_loss} strengthening the regularization of SD Loss consistently drops the unlearning error for ResNet-18 and VGG-19 on both Cifar-10 and cifar-100, and we see from Table \ref{tb:SD_loss_unl_percent} incurring a $5\%$ drop to accuracy one can drop the unlearning error by roughly $25\%$, and allowing for larger drops to accuracy one can keep dropping the unlearning error; it should be noted that this drop in accuracy is after 5 epochs of finetuning (with 15 epochs of total training), and continuing to train we see the effect on performance becomes less \anvith{@gabe for us to reference once we add results for different amounts of pretraining}. Lastly note the regularization strengths in \ref{fig:SD_loss} were chosen after some hyper parameter tuning (mainly that we need to work on a scale of $5-25$ for CIFAR10 and $50-250$ for CIFAR100), and generally, if you scale the output dimension by say $10$ (i.e from having $10$ outputs to $100$ outputs) you need to also scale the regularization strength accordingly; this makes sense as we divide by c (the output dimension) in eq \ref{eq:SD_Loss}. %\varun{why did you choose these particular values?} \anvith{added sentence above}

%However based on \ref{fig:SD_loss} we see for Cifar-100 the SD Loss wasn't able to make a difference; we hypothesize that the large output dimension makes it hard for the SD Loss to optimize, and it's an interesting direction for future work to adapt to build loss functions that work for high dimensional outputs.

%Lastly, in attempt to understand what variables our SD Loss is decreasing in order to decrease the unlearning error, we separately computed the singular values \ref{fig:std_sigma} and change in weights \ref{fig:std_delta_weights} for over 16000 finetuning steps for ResNet-18 on CIFAR-10. As seen in Figure \ref{fig:SD_loss} the SD regularization barely affects the largest singular value, and in fact for large regularization values increases it slightly. 

%Nevertheless as seen in \ref{fig:std_delta_weights} increasing the regularization strength decreases the change in weights significantly, which is what we predicted in our previous analysis of a binary linear classifer in Section~\ref{sec:A Simple Binary Classifer} and now see generalizes to deep neural networks. This is ultimately how it is able to reduce the unlearning error. This loss function may be of interest for other applications where reducing the change in weights is of interest.  

%\paragraph{Conclusion of SD Loss} Thus, compared to the strawman examples considered in Section \ref{sec:Strawman Results}, we have that SD Loss actually reduces $e$. The reason is that it decreases the change in weights, with stronger $\gamma$ meaning a stronger drop in change in weights, just as we predicted. \anvith{@varun or @gabe, anyone know how to fix the big gap that appears in the pdf before the paragraph?}


%In the appendix we added similar experimental results for ResNet-18 when trained with $\ell_2$-regularization, and note though it's goal is to reduce the overall magnitude of the weights, it doesn't have a significant impact on the change in weights nor the unlearning error (and in fact increases it).

%that this new loss does significantly decrease the unlearning error as $\gamma$ increases across all 4 settings. Evidently, $\gamma$ must not be too large to not hinder actual learning of the models. Across all 4 settings, we see that we are able to decrease the unlearning error by on average 47.6\% at $\gamma=5.0$ while only decreasing in testing accuracy by X\% (from X\% to X\%). Changes in testing accuracy and unlearning error as a function of $\gamma$ for all 4 settings is shown in table~\ref{table:SD_loss} in appendix~\ref{appendix:A}. These results show that the standard deviation loss is an effective way to decrease the unlearning error while having limited effect on the performance of models.

%\begin{figure*}[htp]
  % Fixed length
  %\centering
  %\includegraphics[width=7in]{plots/fig10.png}
 %\caption{Unlearning error of 4 setups trained with the standard deviation loss with increasing levels of SD regularization. Across all 4 setups, a stronger regularization decreases the unlearning error at a (minimal) cost of the performance of the model.}
%\label{fig:SD_loss}
%\end{figure*}

%Looking specifically at the singular values, we see in figure~\ref{fig:std_sigma} it seems that the largest singular value blows up at the very beginning of training and increases as a function of of the regularization strength. Although this should increase the unlearning error, we see in figure~\ref{fig:std_delta_weights} that the change in weights decreases as a function of the regularization strength. As supported by the values on the y-axis of figure~\ref{fig:std_sigma} and~\ref{fig:std_delta_weights}, the decrease in the change in weights outweights the increase in the largest singular value which results into the net decrease in unlearning error shown in figure~\ref{fig:SD_loss}. This is counterintuivite to our theoertical justification regarding the SD loss which aims at decreasing the largest singular value. However, these results are understandable: sigma is a function of the loss function which means that if we modify the loss function to decrease sigma,sigma will change accordingly. \gabe{I might have worded this wrong. basically this phenomenon appears in physics where the moment you read a measurement from a system, you break the system. In the same vein, if we try to optimize for sigma by changing the loss function, since sigma is a function of the loss function, you have this nested definition which will lead to unintended results}. \anvith{going to go over this once the figures are updated a bit}

%\begin{figure}
    %\centering
    %\includegraphics[width = 3.3in]{plots/sigma_resnet_cifar10.png}
    %\caption{Largest Singular value over training for different regularization strengths for ResNet-18 on CIFAR-10}
    %\label{fig:std_sigma}
%\end{figure}
%\begin{figure}
    %\centering
    %\includegraphics[width = 3.3in]{plots/delta weights_resnet_cifar10.png}
    %\caption{Change in weights over training for different regularization strengths for ResNet-18 on CIFAR-10}
    %\label{fig:std_delta_weights}
%\end{figure}



%subsection{Evaluating Methods}

%\subsubsection{Pretraining}

    %\anvith{for gabe: basically just show the finetuning results for different models and datasets, i.e that unlearning error increases with t, so clearly having the finetune less steps works}
    
%\anvith{I'll move the discussion for change in weights to the above, ideally here is where you present/explain the experiments and the main takeaways (assuming we are going to present this aspect), for now I've commented it out}

%As the derived unlearning error in equation~\ref{eq:error bound} is a function of the number of SGD steps $t$ and the change in weights $||\mathbf{w}_{t} - \mathbf{w}_{0}||_{2}$, if a model is pretrained for a certain number of steps $N$ on a dataset that is never unlearned, both of these terms will be decreased. It is important that this dataset represents data that will be never be unlearned (ie: could be publicly available data). Pretraining effectively changes the intial weights $\mathbf{w}_{0}$ in  $||\mathbf{w}_{t} - \mathbf{w}_{0}||_{2}$ to $\mathbf{w}_{N}$ if the model was pretrained for $N$ steps. This is because after $N$ steps of pretraining, the pretrained model is much close to it's final minima than the originally initialized weights $\mathbf{w}_{0}$. Additionally, instead of training for a total number of steps $t = T$ and hence needing to consider $T$ steps in the derivation of the unlearning error, pretraining for $N$ steps means that we only need to consider $t = T - N$ steps in the derivation of the unlearning error (ie: $N-T$ is the number of finetuning steps). 

%\gabe{Should I have a paragraph of how pretraining is actually an incredibly common thing in NLP and CV and effectively reduces the individual effect of your small set of private data points by having trained on millions/billions of public data points?}
%\subsubsection{Standard Deviation Loss}

%\anvith{for gabe: basically show the results for SD loss for the different model and datasets, and different settings}

%\anvith{for me and gabe: add some figures showing it does indeed reduce the standard deviation, and if true, show it reduces singular values, and thus supports our hypothetical reasoning}


==> Contents/_10_harm.tex <==
\section*{Proactive Prevention of Harm}

As noted in several prior works (as stated in the paper), unlearning has the potential to leak private information about the data point being unlearnt. If an adversarial entity considers a model before unlearning (say at time $t_0$) and after unlearning (say at time $t_1$), the difference in states leaks information about the data point being unlearnt. Unlearning also has the potential to degrade model performance (depending on the importance of the point towards model functionality).

==> Contents/applications.tex <==

\section{Unlearning Approach} 
\label{section: Unlearning Approach}
The first thing we felt this decomposition led to was a way to unlearn, similar to that proposed in Cao and Yang. Here we simply approximate further that $w_{t} = w_0 - \eta \sum_{i=0}^{t-1} \frac{\partial L}{\partial w}|_{w_0,x_i}$ with the error term simply being  ~\ref{eq: error}, thus to unlearn we'd simply have to add back these gradient updates with respect to $w_{0}$.

However, we can take this further by realizing that error depends on $t^2$, and so can decrease the error by check-pointing the weights regularly, say at a period $\phi$ so that, $w_{n}$, our final weights, is simply:

\begin{equation}
w_{n} = \sum_{i=0}^{\frac{n}{\phi}} (w_{i+1} - w_{i}) + w_{0}
\end{equation}

and so if we unlearn between each $w_{i+1}$ and $w_{i}$ independently, our error is roughly order $n \phi < n^2$.

\section{Applications}

\subsection{Applying the Framework}
Having now set up the classification of unlearning approaches and how we will go about measuring approximate unlearning methods, we now apply this to compare various prior approaches to unlearning; in this sense one of our main contributions is being able to directly compare approaches.

\subsubsection{SISA}
We first define what a proof of learning in this setup looks like, which is an individual proof $P_i$ for every shard. Unlearning then follows by locating the earliest slice the datapoint to be unlearned $x^*$ is seen for the given shard it's in, and retraining from there.

We can the characterize the modified proof obtained as a proof of unlearning as $P_i'$ where $P_i' = P_i$ upto the slice $x^*$ is found, and then changes according to the retraining from there onwards; note all other $P_j$ where $j \neq i$ are left unchanged as they're still constitute a valid proof of unlearning as they do not have $x^*$ as a datapoint used.

It is then clear that from the process of unlearning in SISA one immediately obtains a valid proof of unlearning, and thus this method falls in the category of proper unlearning, with 0 verification error.

\subsubsection{Amnesiac Unlearning}
The proof of learning in this setup is the one originally obtained when training the model, which we'll denote as $P$. Applying Amnesiac Unlearning only changes the final weights, say $w$ to some provably good state $w''$; in the original paper the justification for why the method was effective was given as mitigating membership inference, however membership inference, though intuitively promising, doesn't give proper guarantees constituting a proof (however if mitigating membership inference is all one wishes then this is may be a sufficient justification, however we are focused on the proof aspect). We'll discuss in a later section the correlation between membership inference and our approximate unlearning error (which we note and verify is correlated to verification error), however it's not necessary to focus on membership inference further for Amnesiac unlearning as we can characterize it as a particular realization of our approximate unlearning approach.

By the previous description of our unlearning method \ref{section: Unlearning Approach} (based on our analysis of SGD), if we define our intervals such that each starts at $x^*$ the batch containing the point we want to unlearn, and ends with the batch just before $x^*$ appears again, then in fact our approach is exactly amnesiac unlearning. This is of great consequence as we can now analyze amnesiac unlearning with our approximate error, which we'll see is correlated with verification error (so measures closeness of $w'$ to be coming from the valid proof discussed in \ref{sec: Basis for Approximation}: Basis for Unlearning). In this sense we see that amnesiac unlearning is errorless if batch size equals dataset size, and if the loss landscape is completely linear; the former was suggested by the original authors, but note in their system this would mean removing all updates, however for us we can simply remove the contribution of the specific datapoint, thus this is may actually be practical. Furthermore we see in general, as we can reasonably assume the batch containing $x*$ appears 1 epoch apart in training, the error is equivalent to what our method gets with checkpointing every epoch, which we ran experiments for and found the error to comparatively low (\anvith{will cite these experimental results when added, but it was around a magnitude drop from no checkpointing}) .

\subsubsection{}

\subsection{Issue with including hessian terms}
Until now, we've simply considered unlearning by changed the order independent part. However, there is a more thorough approach to unlearning where you systematically remove all terms including $x^*$ in the order dependent part in ~\eqref{eq: aprox}. However, this would require computing the expected number of hessian vector products on average, which is at least as expensice as training (discussed in \ref{Counting Hessians} classifier to show how this might work in practice.

\section{Optimizing Unlearning}
\subsubsection{Loss functions}
Above we discussed in greater detail the effect of interval lengths on unlearning, here we focus on how we can further reduce the error by modifying the loss function.

As mentioned, the error ~\eqref{eq: aprox} depends on the singular values (i.e the magnitude of the hessian vector products), and so an approach to decrease the error would be to decrease the singular values.

Based on work done in understanding the hessian of the loss function of neural networks, ~\cite{fort2019emergent}, we know the hessian is dominated by the gradient of the softmax, and we can efficiently compute the sum of its eigenvalues by taking the trace of it, which is simply $\sum_{i=0}^{n} p_{i}(1-p_{i})$, where $p_{i}$ denotes the i'th logit, for a classifier with n outputs. We can thus introduce this to a loss function, and have sgd follow a path of lower singular values (the extent of this depends on the weight we give to this new term). We'll call this new loss function the hessian cross-entropy loss, and it is:

\begin{equation}
LHCE(p,y) = - \sum_{i=0}^{n} y_{i} \log(p_{i}) + c*p_{i}(1-p_{i})
\end{equation}

where c is the weighting on the additional term.

\subsubsection{Pretraining}
Another method to further reduce the error is focusing on the number of updates $t$ and the change in weights. If we consider the original model is pre-trained on a dataset that would never be unlearned, the number of updates and accordingly the change in weights to achieve satisfactory performance is significantly decreased. This setting is very common in many tasks in natural language processing and computer vision where models trained on incredibly large datasets and then finetuned for the specific problem at hand. In fact, in NLP, state of the art models such as BERT or GTP-2 have the vast majority of their weights frozen and only the last layer or an additional small classification layer is added on and trained for a small number of updates for a specific task. The pre-trained datasets are usually available to the public or collected from public data and would never be unlearned. \gabe{reminder: its actually very possible that the pretrained dataset is what you want to unlearn (ie: remember Jagielski's paper/blog post about GTP2 knowing your phone number? you might want to unlearn that). Furthermore, if we are going to take about pretraining alot, there is actually a paper that specifically gives an algorithm in the unlearning setting when you can assume that your dataset is divided into a non-unlearning and unlearning dataset so that could be the a compairason}.

\subsubsection{Batch Size}
In the ML literature, the batch size over which you perform a mini-batch update is an important hyperparameter to consider. A large batch size is a less noisy gradient and converges faster but smaller batches results in more updates per second. An additional factor of the batch size is that previous work has shown that larger batch size have shown to lead to sharper minima i.e., the hessian is characterized by many large positive eigenvalues. On the other hand, smaller batch sizes lead to flatter minima with many small eigenvalues. This result is bittersweet in our case. On one end, smaller batch sizes may lead to smaller positive eigenvalues of the hessian which may decrease the largest positive singular value of the hessian. This would decrease the error to unlearn. \gabe{ idk if this is true: Furthermore, to unlearn a single data point, we cannot remove only that data point's gradient update but rather the entire batch it was averaged over. This would mean that we are unintentionally removing $B-1$ updates that we do not wish to unlearn. If $B$ is decreased, this mishap is less important.} On the other end, smaller batch size require more updates to reach adequate performance. Hence understanding which of these effects dominates can help us understand how batch size affects our unlearning error.






==> Contents/comments.tex <==
\begin{comment}

\section{Nicolas Comments}
I guess just address each of Nicolas's comments here (i.e relevant papers, what's been done, issues, good points)
\begin{enumerate}
    \item \textbf{How to define unlearning}. Some papers define unlearning differently. \textit{Linear Filtration for Logit-based Classifiers} ~\cite{baumhauer2020machine} define it as having small difference in the final logit predictions. Other papers are defining unlearning as similar weights to the gold standard. Others want similar accuracy on the points to unlearn of the gold standard retrained model. Some even consider information theory metrics like the mutual information gain ~\cite{golatkar2020eternal}.
    \item \textbf{Group vs. individual guarantee (as in DP):} Can you make any guarantee on individual versus group unlearning? For example does unlearning 1 point from a class K, make it easier for later unlearning requests from the same class? It will also be meaningful to see if we can think of the error bound from SGD as a DP bound 
    \item \textbf{Combine slicing + grad diff estimation:} To improve on amnesiac unlearning, would slicing help to reduce t? There has been no prior work on this
    \item \textbf{higher order terms of error} Considering higher order terms will take as much time or more time to compute then re-training. Although its a shame, we can construct this as a negative result as an upper bound on unlearning while still being effecient.
    \item Taxanomy: 
    The main unlearning methods so far are:
    \begin{enumerate}
        \item SISA (and coded machine unlearning)
        \item Linear Filtration for Logit-based Classifiers
        \item deltagrad
        \item selective forgetting (ie: scrubbing)
        \item amnesiac unlearning
        \item Forgetting Outside the Box: Scrubbing Deep Networks of Information Accessible from Input-Output Observations 
        \item muddying techniques (amensiac unlearning other proposal, Class Clown paper
    \end{enumerate}
\end{enumerate}


\section*{Varun}

\begin{enumerate}
\item Begin discussion by introducing the problem of unlearning and a bunch of relevant related work -- including unlearning using influence functions, amnesiac unlearning, unlearning using SQ learning etc.
\item Motivate the generic approach i.e. how you obtain equation 5.
\item Motivate how prior works actually approximate equation 5 + error term leads to a score that measures "goodness of unlearning"
\item Motivate how prior works fall short in unlearning based on this score. 
\item Motivate how new loss function (with regularization) can enable minimization of this metric (i.e., helps minimize said unlearning metric); can other regularization methods work?
\item Talk about how "unlearning score" is analogous to epsilon in DP -- in practice, does the score actually mean anything? For example, can we formulate some MI attack and verify if the proposed method actually does unlearn better in practice in comparison to prior work?
\item Finally, why should the S\&P community care when most of this work is published in ML venues? 
\end{enumerate}

\end{comment}

==> Contents/contribution.tex <==
\section{Basis for Approximation} \label{section: Basis for Approximation}

The goal of $T$ in the approximate POL scenario is to modify the end state of the model such that it is "close' to the end state of some possible $P'$ that doesn't use $x*$.

For the following work we'll be interested in the specific $P$ described now; consider the model trained by the following sequence of batches $B = {x_0, x_1, \cdot , x_i, \cdot, x_t}$ starting with weights $w_0$ and the associated proof $P$ obtained by training with it. Let $x_i$ be the batch we want to unlearn, then the modified proof $P'$ we submit to $V$ is given by training with the same initial weights $w_0$ but with the batches $B' = {x_0, x_1, \cdot , x_{i-1}, x_{i+1}, \cdot, x_t}$. Our goal then is to get as close to the final state given by $P'$ as possible, as we are less interested in actually computing the proof $P'$, but rather the plausibility of our modified model $f'$ coming from $P'$ which doesn't have $x*$.

A plausible way of understanding this error and modifying $f$ accordingly is modeling the training dynamics approximately by a taylor series approximation over the steps SGD takes, and thus "approximating" the end state of $P'$ which we'll denote as $w'_t$. In particular we're in interested in the differnce between that end state and the current end state $w_t$, which is what we'll proceed to do and analyze. We expect that future work will be able to use more sophisticated models for training, and extend it to training algorithms beyond simple SGD with constant learning rate (which is what we focus on), however there is still plenty of insight to be gained by this approximation.

\footnote{There is vast field devoted to understanding and approximating SGD behaviour \cite{hu2017diffusion,feng2017semi,li2017stochastic}. Using taylor series seems to be a standard approach in other work \cite{smith2021origin}, and is what we proceed to do, however our framework for unlearning is heavily related to this question of understanding sgd, and so it's our opinion that future work will benefit from more sophisticated approximations.}

\section{Introducing The SGD approximation}

What follows in this section is essentially the standard SGD approximation used in other papers for error analysis, as seen in equation 13 in \cite{smith2021origin} (though we keep a few more of the higher order terms, though not all), however we go through the steps of deriving it here to frame it in the problem we're using it for and to be consistent with notation used here and related work, primarily \cite{jia2021proof}. We later deviate from the above mentioned paper as we take a different approach to approximating the second order term more relevant to the approaches we propose later.

Our notation here is that $w_t$ stands for the weights after t steps, $L$ is a generic loss function (i.e what gradient descent acts on), and $x_t$ is the batch of data at the $t+1$ step, i.e $x_0$ is the first batch of data.

We start with the following statement for a single SGD learning update:

\begin{equation}
w_{1} = w_0 - \eta \frac{\partial L}{\partial w}|_{w_0,x_0}
\end{equation}

Then we have that $w_{2}$ is:
\begin{equation}
w_{2} = w_0 - \eta \frac{\partial L}{\partial w}|_{w_0,x_0} - \eta \frac{\partial L}{\partial w}|_{w_0-\eta \frac{\partial L}{\partial w}|_{w_0,x_0},x_1}
\end{equation}

At this point we wish to approximate $\eta \frac{\partial L}{\partial w}|_{w_0-\eta \frac{\partial L}{\partial w}|_{w_0,x_0},x_1}$ so that it only depends on $w_{0}$ and not on the previous gradient computation. We can do this by using a first order taylor series approximation on the partial derivative under the assumption that $\eta \frac{\partial L}{\partial w}|_{w_0,x_0}$ is small (i.e $L_{\infty}<1$), which, as we'll later discuss, is a fair assumption for machine learning models. The result is the following:

\begin{equation}
w_{2} = w_0 - \eta (\frac{\partial L}{\partial w}|_{w_0,x_0} + \frac{\partial L}{\partial w}|_{w_0,x_1} + \frac{\partial^2 L}{\partial^2 w}|_{w_0,x_1} (- \eta \frac{\partial L}{\partial w}|_{w_0,x_0}))
\end{equation}

This is all nice and good, but the true question is how to scale this for an arbitrary t updates. Though it may not be completely obvious at first, the hessian terms from the taylor expansion recursively depend on each other, and we can thus write an arbitrary t update as:

\begin{equation}
w_{t} = w_0 - \eta \sum_{i=0}^{t-1} \frac{\partial L}{\partial w}|_{w_0,x_i} + \sum_{i=1}^{t} f(i) \label{eq: aprox}
\end{equation}

where $f(i)$ is defined recursively as:
\begin{equation}
f(i) = -\eta \frac{\partial^2 L}{\partial^2 w}|_{w_0,x_i} (- \eta \sum_{j=0}^{i-1} \frac{\partial L}{\partial w}|_{w_0,x_j} + \sum_{j=0}^{i-1} f(j))
\end{equation}

with $f(0) = 0$.


==> Contents/detail.tex <==


\section{Understanding The Approximation}

The first important detail to note is that the first sum is commutative with respect to the indices; that is, any permutation of $x_{i}$ results in the same value. Thus, we will continue call this the order independent part.

The recursive component is not invariant to permutations, and so we will call it the order dependent part.

Though we leave it to later sections to further elaborate, the error we're interested between $w'_t$ and $w_t$ is approximated by the magnitude of the order dependent part averaged over the size of the dataset, i.e the contribution of a given datapoint to that term; this is simply as the modified state $f'$ we can feasibly achieve undoes the effect of a given $x*$ on the first part, but not the second, and thus the approximate associated error is the contribution of $x*$ to the second term.

\subsection{Understanding Order Independent Component}

There is not much to say now other than this introduces an ideal scenario in order to remove updates, i.e unlearn. This is also analogous to the update rule in distributed learning and batch SGD.

\subsection{Understanding Order Dependent Component}
$\eta^2 c_{t} + \eta^3 c_{t-1} + ... +\eta^{2+t-1} c_{1}$
\\
The sum of recursive sums is seemingly less digestible, but we can remark that it's global structure follows $\eta^2 c_{t} + \eta^3 c_{t-1} + ... +\eta^{2+t-1} c_{1}$, where $c_{i}$ represent vectors. Thus we can focus primarily on the $\eta^2$ dependent term, noting then that:

\begin{equation}
\label{eq: error}
\eta^2 c_{t} = \sum_{i=1}^{t} \eta^{2} \frac{\partial^2 L}{\partial^2 w}|_{w_0,x_i}  \sum_{j=0}^{i-1} \frac{\partial L}{\partial w}|_{w_0,x_j} 
\end{equation}

now in general we can approximate $\sum_{j=0}^{i-1} \frac{\partial L}{\partial w}|_{w_0,x_j}$ by its expectation, which is $\frac{i(w_{t}-w_{0})}{t}$. We further normalize the vector, and thus have:

\begin{equation}
\label{eq: Detailed_Aprox}
\eta^2 c_{t} \approx \eta^{2} \frac{||w_{t}-w_{0}||}{t} \sum_{i=1}^{t} \frac{\partial^2 L}{\partial^2 w}|_{w_0,x_i} \frac{w_{t}-w_{0}}{||w_{t}-w_{0}||} i
\end{equation}

We can take a further step by focusing on $||c_{t}||$ and noting $||\frac{\partial^2 L}{\partial^2 w}|_{w_0,x_i} \frac{w_{t}-w_{0}}{||w_{t}-w_{0}||}|| \leq ||\frac{\partial^2 L}{\partial^2 w}|_{w_0,x_i}||$ by definition of the induced $L_{2}$ norm, which is simply the largest eigenvalue of the hessian square rooted, i.e $\sigma_{1,i}$ the first singular value of the hessian on $x_{i}$. For sake of simplicity we consider $\sigma = max(\sigma_{1,i})$, and thus have:

\begin{equation}
||\eta^{2} c_{t}|| \leq \eta^{2} \frac{||w_{t}-w_{0}||}{t} \sigma \frac{t^{2} - t}{2} \label{eq: error bound}
\end{equation}

This is far more informative as we thus see the term depends linearly on $||w_{t}-w_{0}||$, $\sigma$, and $t$. The $\sigma$ captures the non-linearity of the loss landscape from the hessian, and thus we see that the more linear the loss landscape, the lower the value. We also see from this that in the scenario $t=1$ or $\sigma = 0$, this bound, and thus the term, is 0. We will later further elaborate on all these properties and how they relate to unlearning. However for later experiments we will stick to approximating \ref{eq: Detailed_Aprox} by taking the average singular values over epochs as mentioned in the previous paragraph.

%\todo{np: this is cool for intuition. you should illustrate the intuition we discussed on our call for each of the terms of the bound on a linear model where you know that everything will hold exactly. you could also consider a deep linear network (look up on internet there is long line of work started by andrew saxe) to make things more interesting with non-linear learning dynamics}

%\anvith{That sounds interesting, I'm taking a look into it. What's actually weird is that the non-linearity of the loss, i.e value of the hessian, is actually dominated by the contribution from the final softmax (see equation 10 and the discussion above it from "Emergent properties of the local geometry of neural loss landscapes"), but I guess those deep linear networks wouldn't have a softmax (or at least those that don't are the ones we'd look at to see extremely low to no error)}

%Perhaps most importantly, this quantity is seemingly the same units as the loss, as we expect $||w_{t}-w_{0}|| \propto t$, and units of $\sigma$ are $\frac{loss}{w^2} = \frac{loss}{t^2}$, thus all together we have  $\frac{loss * t^3}{t^3} = loss$. This helps justify the universality of our $d(A,A')$ if indeed the loss is a universal metric (i.e comparable between models and datasets).

%However in general we expect $||w_{t}-w_{0}|| \propto t$, and so we expect a quadratic growth with $t$ (or at least a faster growth than simply linear) but interestingly, experimentally we found that the error grows linearly with t, suggesting that $||w_{t}-w_{0}||* \sigma = constant$.


\subsection{Noteworthy Properties}
So far in our analysis we have set $w_{0}$ and $w_{t}$ to be arbitrary, though perhaps implied that they are the starting and end point in training. In general we can consider any $w_{0}$ and $w_{n}$, and split this further into smaller arbitrary intervals $w_{0},w_{t},w_{2t}, ... w_{n}$. Thus we see that we can simply approximate any $w_{i*t}$ with respect to $w_{(i-1)t}$ rather than needing to approximate $w_{n}$ with respect to $w_{0}$. We emphasize this now as this will be particularly relevant in our analysis of amnesiac unlearning and how pretraining is beneficial.

\subsection{Counting Hessians} \label{Counting Hessians}

We focus now on the expression in \ref{eq: error}, and consider what terms on average would contain a particular $x_{i}$.

Consider that we focus on a uniform distribution over datapoints $x_i$ so that our expectation of i is $t/2$. In this case, every indexed term $j$ where $(t/2) \leq j$ will thus contain an $x_i$ in the second sum. Furthermore, the term $j=t/2$ would have $x_i$ in the hessian, meaning every term in the second sum for $i=t/2$ would have a coefficient with $x_i$. Thus on average we'd expect to compute $t$ gradients and $t/2$ hessian.

To be more specific, we'd need to compute $t$ hessian vector products. In general it is possible to implement hessian products in O(n) ~\cite{adams1995hitchhiker}.

So noting that the hessian vector product is at least as expensive (or of the same order as) gradient computation, we have that the computational requirement to compute all these terms is at least as expensive as training. However we can easily approximate the sum of the eigenvalues of the hessian, and as we'll see, we are to able to introduce this into the loss in order to decrease the singular values (and thus the magnitude of our error).

\todo{np you should expand discussion here to say whether there are valuable uses to computing an approximation of the hessian instead}


==> Contents/motivation.tex <==
\section{Update: Motivation and Focus}
From literature review on unlearning methods, most work on machine unlearning can roughly be divided into two methods: manipulation/approximation of SGD and statistical methods. The former leverages checking pointing gradient updates throughout the whole training procedure of SGD and undoing certain updates to unlearning. The latter methods use different methods to effectively unlearn from the final weights, where unlearning manifests itself in different ways (on the weights, on the predictions, on accuracy etc).\todo{np: i have no idea what you are talking about here in the latter methods} We will be focusing solely on the former class and provide a theoretical framework to understand the effectiveness and the limitations associated with SGD based unlearning methods. Our contributions will be as follows. In italics is not set in stone, rather things we think can be interesting
\begin{enumerate}
    \item Provide a theoretical framework from Amnesiac Unlearning \todo{np: i think it is a bit limiting to say you provide a theoretical framework for amnesiac unlearning. i would suggest saying that you analyze the broad class of methods that seek to compute inverse SGD gradients. amnesiac unlearning is just one approach to achieve this effect }
    \item Provide bounds on the error of SGD based unlearning methods
    \item \textit{Investigate how SGD based unlearning methods are affected by architecture and model complexity}
    \item \textit{Provide a simply taxonomy of the 2 classes of unlearning}
\end{enumerate}



==> Contents/new_7_Unl_Err_is_Good.tex <==
\section{Comparing Unlearning Error and Verification Error}
\label{sec:Comparing Unlearning Error and Verification Error}

%\anvith{for me: brief blurb on reasoning to just check that we're actually achieving what we want to (reducing true discrepency), i.e our approximation is justified, but it is an approximation, and it is worth checking we are indeed accomplishing what we want to}

At this point, with our SD Loss, we see we can significantly reduce $e$, and similarly we see changing $t$ (i.e by pretraining) is also a viable option though not ideal. Together these two give us an option to vary the unlearning error and see if reducing unlearning error also reduces verification error (i.e that they are correlated under these methods). The main takeaway from this section will be that they are indeed strongly correlated, and that when we reduce unlearning error with the methods we've considered we in fact also reduce verification error. This shows unlearning error is a viable alternative to verification error.

%However it is reasonable to wonder whether in fact decreasing $e$ as we've done with the two methods does in fact decrease the true discrepancy, i.e whether our approximation are justified and good (i.e are we doing what we want to), which is what we verify in this section.

%Note the main point for computing $e$ instead of the true discrepancy is simply that, as you'll see with our experimental setup described in \ref{ssec:verifying experimental setup}, the true discrepancy requires computing the properly retrained model $M'$, and so in practice having to compute $M'$ to assess error would negate the computational benefit of the approximate unlearning method. It is also not clear what exactly one needs to change to reduce the verification error, however it is more apparent with unlearning error.

%However, as will be the main takeaway from this section, decreasing $e$ with the methods we've described earlier does in fact decrease the true discrepancy and the correlation between $e$ and the true discrepancy is very strong; thus one can reasonably only work with $e$ to compare how effectively one has unlearned.

\subsection{Experimental Setup}
\label{ssec:verifying experimental setup}
We are interested in determining what is the relationship between our proposed unlearning error in Equation~\ref{eq:unl_err} with the actual verification error, measured simply as $||\weights' - \weights''||_{2}$ where $\weights'$ are the weights of $M'$ (the ideal retrained model) and $M''$ the weights after our unlearning method. 

%Using the taxonomy defined in section~\ref{sec:define_unlearning}, we are interested in the relationship between the difference of our unlearned model compared to the gold standard of retraining ($||\model^{'} - \model^{''}||_{2}$) and our unlearning error. 

%From now on we'll also refer to $||\model^{'} - \model^{''}||_{2}$ (the true discrepancy) as verification error, for reasons more apparent when we make the connection to proof of learning. 

The experiments in this section will be for the same models and datasets introduced in section~\ref{ssec:experimental setup}, and we modify the experimental procedure from section~\ref{ssec:experimental setup} as follows:
\begin{enumerate}
    \item Pretrain $\model_{0}$ by training $\model_{0}$ on the entirety of $D$ for N steps until we reach $\model_{N}$.
    \item Train $\model_{N}$ for a small number of steps $T$ on batches of data $\{x_1,x_2,\dots,x_T\}$ to get $\model_{N+T}$ and its weights $\weights_{N+T}$. We will consider $\model_{N+T}$ the model we wish to unlearn and WLOG the point we wish to unlearn is in batch $x_{1}$.
    \item Train $\model_{N}$ for $T-1$ steps on batches $\{x_2,\dots,x_T\}$. The resulting model is the naively retrained model $M'$ without batch $x_{1}$, with weights $\weights'$.
    \item Get $M''$, in particular $\weights''$, by our unlearning method:
    $$ \weights'' = \weights_{N+T} + \eta  \frac{\partial L}{\partial w}|_{\weights_{N+T},x_1}$$
    \item Compute the unlearning error of $M_{N+T}$ and the verification error ($||\weights' -\weights''||_{2}$).
\end{enumerate}
Again, depending on the experiment we compute the unlearning error and verification error at regular intervals during the finetuning process.

\varun{what are the datasets used? what are the model architectures used?}\anvith{same as last time, added/modifed the sentence just before the enumeration}




\subsection{Experimental evidence}
%\anvith{for gabe: present here the experimental evidence showing that the methods we considered earlier for decreasing unlearning error are indeed decreasing the true discrepency}

\varun{i find the section on pretraining distracting as in 4.1 and 4.2 -- you've established why you'd not want to do it; the discussion in this section is also very thin -- you basically conclude with "there's strong correlation". no discussion on "why". }
\anvith{I think showing pretraining is still important, as the underlying phenomenon is the correlation with t, which strictly speaking we have no justification for why verification error should increase with unlearning error when increasing t}
\anvith{I'm adding more discussion, but the main "why" is that unlearning error is a good metric for verification error, this is to just prove this- tying back to the opening paragraphs to section 5}


\subsubsection{Changing t}

%The main underlying assumption for pretraining is that varying t varies the unlearning error $e$ proportionally; thus, with $t$ being our only variable, we'd like to see that the true discrepency and unlearning error are positively correlated, meaning that with pretraining we are in fact reducing the true discrepency when we are reducing the unlearning error (which is what we can relatively cheaply measure).

What we saw from Figure~\ref{fig:unl_t} is that unlearning error increases with t; the follow up question is now whether verification error does in fact increase with t, or more generally, with t as our only variable, is unlearning error and verification error correlated.

Figure~\ref{fig:pretrain} shows the relationship between the verification error and the unlearning error as a function of the number of SGD steps taken (i.e $t$). The model is a ResNet-18 pretrained for 80 epochs on CIFAR10 and then performs steps 1-5 in section~\ref{ssec:experimental setup} for $T=14000$ steps or approximately 5 epochs of training. The main takeaway here is that the verification error and unlearning error have a strong correlation of $0.9668$, and thus when we reduce the unlearning error with pretraining, we reduce the true discrpency.

%Furthermore, We also see that both verification and unlearning error are a similar function of $t$, and so we can conclude that when varying $t$, if we decrease unlearning error, we also decrease the true discrepancy; thus our assumption for pretraining . 

%\gabe{does this make sense? I think it's poorly worded, need to fix IMO} \anvith{I've reworded it a bit, basically the point is we want to state first the assumption for pretraining was varying t proportionally affect unlearning error, and we want to show that with this as our only variable, we have a strong correlation between verification error and unlearning error, which is what that figure shows; thus we conclude that our assumption for pretraining was correct, and thus pretraining is applicable}.

\anvith{Slight issue with the below statement is that verification error is the difference between $M''$ and $M$, and so increasing verification error does necessarily mean increasing difference of $M$ and $M'$}
As another takeaway, these results also agree with the intuition behind why unlearning deep neural networks trained with iterative methods such as SGD are difficult. Even though $\model$ and $\model^{'}$ differ by a single batch, once the differing batch occurs during training, $\model$ and $\model^{'}$ begin to take two different sequences of updates and begin to diverge. As you increase the number of steps a model learns for, the model is left to continue to diverge further and further, which is shown by the verification error increasing as a function of $t$.



\begin{figure}
    \centering
    \includegraphics[width = 3.2in]{plots/VER_VS_UNL_61.png}
    \caption{Unlearning error and verification error as a function of the finetuning steps (indicated by the color gradient) for ResNet-18 on CIFAR-10. Unlearning error and verification error are measured every 100 SGD updates for a total of 14000 SGD updates. The correlation between unlearning error and verification error as a function of $T$ is 0.9668. Both unlearning error and verification error increase as a function of the number of finetuning steps}
    \label{fig:pretrain}
\end{figure}

\subsubsection{SD Loss}


\varun{could you explain, with the pearson coefficient values, why the correlation is strong in the text description as well?} \anvith{added}

As seen in figure~\ref{fig:corr_std_loss} when varying the strength of our SD regularization we have a strong correlation between unlearning error and the verification error for ResNet-18 and VGG-19 on CIFAR10 of 0.96 and 0.81 respectively; in fact for VGG-19 we see the relation between verification error and the regularization is stronger than that for unlearning error (note the y-axis in \ref{fig:corr_std_loss} (b) continually decreases with the strength of the regularization where as the x-axis has some noise).

%Thus the main takeaway here is that only changing the SD regularization, when we decrease the unlearning error we also decrease the verification error, and so we were justified in looking solely at the unlearning error (which is easier to compute).

This is a strong result, as only reasoning with the verification error, it is not clear how one might've come to the SD Loss to reduce it. This also shows more generally that the unlearning error accurately proxies the verification error when varying our loss function.

\begin{figure}
    \centering
    \includegraphics[width = 3.2in]{plots/std_loss_correlation-2.png}
 \caption{Correlation between unlearning error and verification error for ResNet-18 and VGG-19 on CIFAR10 as a function of the regularization strength. The correlations are both high at 0.96 and 0.81 for ResNet-18 and VGG-19, respectively. Notice that the stronger the regularization (more blue) the more the verification and unlearning error decrease in both settings.}
\label{fig:corr_std_loss}
\end{figure}


\subsubsection{Considering all Models}


\varun{what are the parameters you vary in fig~\ref{fig:big_final_corr}?} \anvith{@gabe can you add it somewhere in the text: I believe it was just loss, regularization strength, finetuning steps, pretraining amount, model, and datasets}\gabe{Added in the text below, we can be more specific in the appendix if need be}.

Lastly as seen in figure~\ref{fig:big_final_corr} where we consider 160 different training setups (ie: different batch sizes, training amounts, regularization strength(s) etc), we see that in general, regardless of architecture, when a model with a specific setup (one of the ones we've been considering) has lower unlearning error, it has lower verification error, as we see by the strong positive correlation between unlearning error and the verification error across the different settings and architecture considered.

This result is highly non-trivial, as simply using the number of training steps as a proxy for verification error (with the rather intuitive reasoning behind pretraining that error increases with steps), we would not be able to tell if one model had a higher error than another when trained the same number of steps, nor how a loss function might change this error.

\anvith{@varun added this to reiterate why this works, going back to the opening paragraphs for section 5}
In the end the reason why unlearning error does in fact serve as a good proxy for the verification is simply the mathematical basis for it presented in section \ref{sec:approximation}, which relied on several approximations but as we've seen in this section the metric still works (at least for all the scenarios we've considered).

\begin{figure*}
    \centering
    \includegraphics[width = 7in]{plots/final_fig.png}
 \caption{Unlearning and verification error for 160 settings across CIFAR10 and CIFAR100. The correlation between unlearning error and verification error for CIFAR10 and CIFAR100 are \textbf{0.9028} and  \textbf{0.8813}, respecively. Settings trained with SD loss (green) for both datasets have lower unlearning and verification error then those trained with regular cross entropy (red).}
\label{fig:big_final_corr}
\end{figure*}

==> usenix2019_v3.1.tex <==
% usenix.sty - to be used with latex2e for USENIX.
% To use this style file, look at the template usenix2019_v3.1.tex
%
% $Id: usenix.sty,v 1.2 2005/02/16 22:30:47 maniatis Exp $
%
% The following definitions are modifications of standard article.sty
% definitions, arranged to do a better job of matching the USENIX
% guidelines.
% It will automatically select two-column mode and the Times-Roman
% font.
%
% 2018-12-19 [for ATC'19]: add packages to help embed all fonts in
%   pdf; to improve appearance (hopefully); to make refs and citations
%   clickable in pdf
%
% 2020-09-21 file updated to comment out flushend and make it optional

%
% USENIX papers are two-column.
% Times-Roman font is nice if you can get it (requires NFSS,
% which is in latex2e.

\if@twocolumn\else\input twocolumn.sty\fi
\usepackage{mathptmx}  % times roman, including math (where possible)

% hopefully embeds all fonts in pdf
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{pslatex}

% appearance
\usepackage[kerning,spacing]{microtype} % more compact and arguably nicer

% Uncomment the following line if you want the columns of the last page 
% equal in size. But note that doing so may cause issues with some 
% document-generating tools.
% \usepackage{flushend}

% refs and bib
\usepackage{cite}               % order multiple entries in \cite{...}
\usepackage{breakurl}           % break too-long urls in refs
\usepackage{url}                % allow \url in bibtex for clickable links
\usepackage{xcolor}             % color definitions, to be use for...
\usepackage[]{hyperref}         % ...clickable refs within pdf...
\hypersetup{                    % ...like so
  colorlinks,
  linkcolor={green!80!black},
  citecolor={red!70!black},
  urlcolor={blue!70!black}
}

%
% USENIX wants margins of: 0.75" sides, 1" bottom, and 1" top.
% 0.33" gutter between columns.
% Gives active areas of 7" x 9"
%
\setlength{\textheight}{9.0in}
\setlength{\columnsep}{0.33in}
\setlength{\textwidth}{7.00in}

\setlength{\topmargin}{0.0in}

\setlength{\headheight}{0.0in}

\setlength{\headsep}{0.0in}

\addtolength{\oddsidemargin}{-0.25in}
\addtolength{\evensidemargin}{-0.25in}

% USENIX wants no page numbers for camera-ready papers, so that they can
% number them themselves.  But submitted papers should have page numbers
% for the reviewers' convenience.
% 
%
% \pagestyle{empty}

%
% USENIX titles are in 14-point bold type, with no date, and with no
% change in the empty page headers.  The whole author section is 12 point
% italic--- you must use {\rm } around the actual author names to get
% them in roman.
%
\def\maketitle{\par
 \begingroup
   \renewcommand\thefootnote{\fnsymbol{footnote}}%
   \def\@makefnmark{\hbox to\z@{$\m@th^{\@thefnmark}$\hss}}%
    \long\def\@makefntext##1{\parindent 1em\noindent
            \hbox to1.8em{\hss$\m@th^{\@thefnmark}$}##1}%
   \if@twocolumn
     \twocolumn[\@maketitle]%
     \else \newpage
     \global\@topnum\z@
     \@maketitle \fi\@thanks
 \endgroup
 \setcounter{footnote}{0}%
 \let\maketitle\relax
 \let\@maketitle\relax
 \gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}

\def\@maketitle{\newpage
 \vbox to 2.5in{
 \vspace*{\fill}
 \vskip 2em
 \begin{center}%
  {\Large\bf \@title \par}%
  \vskip 0.375in minus 0.300in
  {\large\it
   \lineskip .5em
   \begin{tabular}[t]{c}\@author
   \end{tabular}\par}%
 \end{center}%
 \par
 \vspace*{\fill}
% \vskip 1.5em
 }
}

%
% The abstract is preceded by a 12-pt bold centered heading
\def\abstract{\begin{center}%
{\large\bf \abstractname\vspace{-.5em}\vspace{\z@}}%
\end{center}}
\def\endabstract{}

%
% Main section titles are 12-pt bold.  Others can be same or smaller.
%
\def\section{\@startsection {section}{1}{\z@}{-3.5ex plus-1ex minus
    -.2ex}{2.3ex plus.2ex}{\reset@font\large\bf}}
